Learning-Assisted Optimization for Transmission Switching

The design of new strategies that exploit methods from Machine Learning to facilitate the resolution of challenging and large-scale mathematical optimization problems has recently become an avenue of prolific and promising research. In this paper, we propose a novel learning procedure to assist in the solution of a well-known computationally difficult optimization problem in power systems: The Direct Current Optimal Transmission Switching (DC-OTS) problem. The DC-OTS problem consists in finding the configuration of the power network that results in the cheapest dispatch of the power generating units. With the increasing variability in the operating conditions of power grids, the DC-OTS problem has lately sparked renewed interest, because operational strategies that include topological network changes have proved to be effective and efficient in helping maintain the balance between generation and demand. The DC-OTS problem includes a set of binaries that determine the on/off status of the switchable transmission lines. Therefore, it takes the form of a mixed-integer program, which is NP-hard in general. In this paper, we propose an approach to tackle the DC-OTS problem that leverages known solutions to past instances of the problem to speed up the mixed-integer optimization of a new unseen model. Although our approach does not offer optimality guarantees, a series of numerical experiments run on a real-life power system dataset show that it features a very high success rate in identifying the optimal grid topology (especially when compared to alternative competing heuristics), while rendering remarkable speed-up factors.

==> times.tex <==
count,BEN,ANG-BA5,ANG-BK5,ANG-K5,KNN5,LP5,MIP_B5,MIP_BM5,MIP_M5,ANG-BA10,ANG-BK10,ANG-K10,KNN10,LP10,MIP_B10,MIP_BM10,MIP_M10,ANG-BA20,ANG-BK20,ANG-K20,KNN20,LP20,MIP_B20,MIP_BM20,MIP_M20,ANG-BA50,ANG-BK50,ANG-K50,KNN50,LP50,MIP_B50,MIP_BM50,MIP_M50,ANG-BA100,ANG-BK100,ANG-K100,KNN100,LP100,MIP_B100,MIP_BM100,MIP_M100,ANG-BA200,ANG-BK200,ANG-K200,KNN200,LP200,MIP_B200,MIP_BM200,MIP_M200,ANG-BA500,ANG-BK500,ANG-K500,KNN500,LP500,MIP_B500,MIP_BM500,MIP_M500
0.0,0.59,0.03,0.04,0.03,0.0,0.0,0.04,0.02,0.69,0.04,0.04,0.07,0.0,0.01,0.07,0.06,0.86,0.04,0.05,0.06,0.0,0.02,0.09,0.07,0.71,0.05,0.05,0.07,0.0,0.04,0.18,0.08,0.81,0.06,0.05,0.07,0.0,0.07,0.2,0.11,0.52,0.06,0.05,0.06,0.0,0.13,0.24,0.21,0.53,0.07,0.07,0.35,0.0,0.19,0.46,0.42,0.53
1.0,0.82,0.03,0.04,0.06,0.0,0.0,0.04,0.04,0.74,0.04,0.05,0.07,0.0,0.01,0.08,0.07,0.94,0.05,0.05,0.06,0.0,0.02,0.11,0.08,0.81,0.05,0.05,0.07,0.0,0.04,0.21,0.11,0.86,0.06,0.05,0.07,0.0,0.08,0.24,0.21,0.72,0.08,0.06,0.07,0.0,0.15,0.32,0.23,0.72,0.11,0.11,0.35,0.0,0.24,0.47,0.44,0.61
2.0,0.89,0.03,0.04,0.06,0.0,0.0,0.05,0.04,0.75,0.05,0.05,0.08,0.0,0.01,0.09,0.07,0.96,0.05,0.05,0.07,0.0,0.02,0.12,0.09,0.85,0.05,0.05,0.07,0.0,0.04,0.25,0.14,0.87,0.06,0.06,0.08,0.0,0.08,0.26,0.23,0.72,0.09,0.06,0.08,0.0,0.16,0.33,0.28,0.73,0.13,0.13,0.35,0.0,0.24,0.58,0.44,0.62
3.0,0.92,0.03,0.04,0.06,0.0,0.0,0.06,0.04,0.89,0.05,0.05,0.08,0.0,0.01,0.1,0.07,0.99,0.05,0.05,0.08,0.0,0.02,0.15,0.09,0.92,0.06,0.06,0.07,0.0,0.04,0.27,0.17,0.88,0.06,0.06,0.08,0.0,0.08,0.27,0.27,0.73,0.09,0.06,0.08,0.0,0.16,0.33,0.32,0.77,0.13,0.13,0.35,0.0,0.24,0.62,0.47,0.63
4.0,0.96,0.03,0.05,0.06,0.0,0.0,0.06,0.05,0.9,0.05,0.06,0.08,0.0,0.01,0.1,0.07,1.0,0.05,0.05,0.08,0.0,0.02,0.17,0.1,0.95,0.07,0.06,0.07,0.0,0.04,0.3,0.18,0.89,0.07,0.06,0.09,0.0,0.08,0.28,0.29,0.83,0.1,0.07,0.09,0.0,0.16,0.33,0.33,0.81,0.18,0.18,0.36,0.0,0.26,0.63,0.47,0.77
5.0,0.99,0.04,0.05,0.06,0.0,0.0,0.06,0.06,0.92,0.05,0.06,0.09,0.0,0.01,0.1,0.08,1.01,0.05,0.05,0.08,0.0,0.02,0.19,0.11,0.96,0.07,0.06,0.07,0.0,0.04,0.32,0.2,0.91,0.07,0.07,0.09,0.0,0.08,0.31,0.32,0.86,0.1,0.08,0.1,0.0,0.16,0.43,0.34,0.85,0.18,0.18,0.36,0.0,0.26,0.66,0.5,0.78
6.0,0.99,0.04,0.05,0.06,0.0,0.0,0.07,0.06,0.93,0.05,0.06,0.09,0.0,0.01,0.1,0.08,1.01,0.05,0.05,0.08,0.0,0.02,0.21,0.12,0.96,0.07,0.06,0.07,0.0,0.04,0.32,0.2,0.92,0.07,0.07,0.1,0.0,0.08,0.31,0.32,0.89,0.1,0.08,0.1,0.0,0.16,0.44,0.35,0.86,0.19,0.19,0.36,0.0,0.26,0.68,0.5,0.8
7.0,1.0,0.04,0.05,0.06,0.0,0.0,0.07,0.06,0.94,0.05,0.06,0.09,0.0,0.01,0.1,0.08,1.07,0.06,0.05,0.09,0.0,0.02,0.24,0.12,1.0,0.07,0.06,0.08,0.0,0.04,0.32,0.2,0.96,0.08,0.07,0.1,0.0,0.08,0.32,0.33,0.9,0.1,0.08,0.11,0.0,0.16,0.45,0.39,0.88,0.2,0.2,0.36,0.0,0.26,0.69,0.51,0.81
8.0,1.01,0.04,0.05,0.06,0.0,0.0,0.07,0.06,0.98,0.05,0.06,0.09,0.0,0.01,0.1,0.09,1.08,0.06,0.06,0.09,0.0,0.02,0.25,0.12,1.0,0.07,0.06,0.08,0.0,0.04,0.33,0.22,0.97,0.08,0.07,0.11,0.0,0.08,0.33,0.33,0.96,0.1,0.09,0.11,0.0,0.16,0.45,0.4,0.93,0.21,0.21,0.37,0.0,0.26,0.7,0.51,0.87
9.0,1.02,0.04,0.05,0.06,0.0,0.0,0.07,0.06,0.98,0.05,0.06,0.09,0.0,0.01,0.11,0.09,1.11,0.06,0.06,0.09,0.0,0.02,0.26,0.15,1.01,0.07,0.06,0.09,0.0,0.04,0.33,0.23,0.97,0.08,0.07,0.11,0.0,0.08,0.33,0.34,0.96,0.1,0.09,0.11,0.0,0.16,0.46,0.41,0.95,0.21,0.21,0.37,0.0,0.26,0.72,0.51,0.89
10.0,1.06,0.04,0.05,0.07,0.0,0.0,0.07,0.06,1.0,0.05,0.06,0.1,0.0,0.01,0.11,0.09,1.13,0.06,0.06,0.1,0.0,0.02,0.26,0.15,1.04,0.07,0.07,0.09,0.0,0.04,0.34,0.23,0.98,0.09,0.07,0.11,0.0,0.08,0.33,0.34,0.97,0.1,0.09,0.12,0.0,0.16,0.48,0.42,0.96,0.22,0.22,0.38,0.0,0.26,0.74,0.51,0.9
11.0,1.07,0.05,0.05,0.07,0.0,0.0,0.07,0.06,1.01,0.05,0.06,0.1,0.0,0.01,0.12,0.09,1.13,0.06,0.06,0.1,0.0,0.02,0.26,0.15,1.04,0.08,0.07,0.1,0.0,0.04,0.35,0.25,1.06,0.09,0.07,0.11,0.0,0.08,0.33,0.35,0.97,0.11,0.09,0.12,0.0,0.16,0.48,0.42,0.97,0.23,0.23,0.38,0.0,0.26,0.74,0.52,0.9
12.0,1.09,0.05,0.05,0.07,0.0,0.0,0.07,0.06,1.07,0.06,0.06,0.1,0.0,0.01,0.12,0.09,1.15,0.06,0.06,0.11,0.0,0.02,0.27,0.16,1.06,0.08,0.07,0.11,0.0,0.04,0.35,0.27,1.08,0.09,0.07,0.12,0.0,0.08,0.33,0.35,0.98,0.11,0.09,0.14,0.0,0.16,0.49,0.42,0.97,0.24,0.24,0.38,0.0,0.26,0.78,0.52,0.91
13.0,1.1,0.05,0.05,0.07,0.0,0.0,0.08,0.06,1.12,0.06,0.06,0.1,0.0,0.01,0.14,0.09,1.18,0.06,0.06,0.11,0.0,0.02,0.28,0.16,1.07,0.08,0.07,0.11,0.0,0.04,0.36,0.28,1.1,0.09,0.08,0.13,0.0,0.08,0.36,0.36,0.98,0.11,0.09,0.15,0.0,0.16,0.5,0.44,0.98,0.26,0.26,0.38,0.0,0.26,0.79,0.54,0.92
14.0,1.1,0.05,0.05,0.07,0.0,0.0,0.09,0.07,1.13,0.06,0.06,0.1,0.0,0.01,0.14,0.1,1.19,0.06,0.06,0.11,0.0,0.02,0.29,0.16,1.11,0.08,0.07,0.11,0.0,0.04,0.37,0.29,1.11,0.1,0.08,0.13,0.0,0.08,0.37,0.36,0.98,0.12,0.1,0.16,0.0,0.16,0.5,0.44,0.98,0.27,0.27,0.38,0.0,0.26,0.8,0.55,0.93
15.0,1.11,0.05,0.05,0.07,0.0,0.0,0.09,0.07,1.13,0.06,0.06,0.1,0.0,0.01,0.14,0.1,1.23,0.06,0.06,0.12,0.0,0.02,0.3,0.17,1.13,0.08,0.07,0.11,0.0,0.04,0.37,0.29,1.12,0.1,0.08,0.13,0.0,0.08,0.38,0.37,0.99,0.12,0.1,0.17,0.0,0.16,0.51,0.45,1.01,0.27,0.27,0.38,0.0,0.26,0.8,0.55,0.94
16.0,1.15,0.05,0.05,0.07,0.0,0.0,0.09,0.07,1.13,0.06,0.06,0.1,0.0,0.01,0.14,0.1,1.23,0.06,0.06,0.12,0.0,0.02,0.3,0.17,1.15,0.08,0.08,0.11,0.0,0.04,0.37,0.3,1.15,0.1,0.08,0.14,0.0,0.08,0.4,0.37,0.99,0.12,0.1,0.19,0.0,0.16,0.53,0.45,1.02,0.27,0.27,0.38,0.0,0.26,0.8,0.56,1.0
17.0,1.16,0.05,0.05,0.07,0.0,0.0,0.1,0.07,1.13,0.06,0.06,0.11,0.0,0.01,0.14,0.1,1.24,0.06,0.06,0.12,0.0,0.02,0.3,0.17,1.16,0.08,0.08,0.12,0.0,0.04,0.37,0.3,1.17,0.1,0.08,0.14,0.0,0.08,0.41,0.37,1.02,0.13,0.1,0.19,0.0,0.16,0.54,0.45,1.03,0.29,0.29,0.39,0.0,0.26,0.82,0.56,1.0
18.0,1.2,0.05,0.05,0.07,0.0,0.0,0.1,0.07,1.15,0.06,0.07,0.11,0.0,0.01,0.15,0.11,1.24,0.07,0.07,0.12,0.0,0.02,0.3,0.18,1.2,0.08,0.08,0.12,0.0,0.04,0.38,0.31,1.18,0.1,0.08,0.15,0.0,0.08,0.42,0.38,1.03,0.13,0.1,0.21,0.0,0.16,0.55,0.46,1.05,0.29,0.29,0.39,0.0,0.26,0.82,0.57,1.01
19.0,1.2,0.05,0.05,0.07,0.0,0.0,0.11,0.07,1.16,0.06,0.07,0.11,0.0,0.01,0.16,0.12,1.25,0.07,0.07,0.12,0.0,0.02,0.3,0.19,1.21,0.09,0.08,0.12,0.0,0.04,0.38,0.31,1.21,0.1,0.09,0.15,0.0,0.08,0.42,0.38,1.05,0.13,0.1,0.22,0.0,0.16,0.55,0.46,1.08,0.29,0.29,0.39,0.0,0.26,0.83,0.58,1.01
20.0,1.2,0.05,0.05,0.07,0.0,0.0,0.11,0.07,1.27,0.06,0.07,0.11,0.0,0.01,0.17,0.12,1.26,0.07,0.07,0.13,0.0,0.02,0.31,0.19,1.22,0.09,0.08,0.12,0.0,0.04,0.4,0.32,1.23,0.1,0.09,0.16,0.0,0.08,0.43,0.38,1.08,0.13,0.1,0.22,0.0,0.16,0.57,0.47,1.09,0.29,0.29,0.39,0.0,0.26,0.85,0.58,1.03
21.0,1.22,0.05,0.05,0.08,0.0,0.0,0.11,0.07,1.29,0.06,0.07,0.11,0.0,0.01,0.18,0.13,1.28,0.07,0.07,0.13,0.0,0.02,0.31,0.2,1.24,0.09,0.08,0.12,0.0,0.04,0.41,0.33,1.24,0.11,0.09,0.16,0.0,0.08,0.43,0.39,1.08,0.13,0.11,0.22,0.0,0.16,0.61,0.47,1.12,0.29,0.29,0.39,0.0,0.26,0.86,0.59,1.03
22.0,1.24,0.05,0.05,0.08,0.0,0.0,0.12,0.07,1.33,0.06,0.07,0.12,0.0,0.01,0.19,0.15,1.3,0.07,0.07,0.13,0.0,0.02,0.33,0.2,1.29,0.09,0.08,0.13,0.0,0.04,0.42,0.33,1.25,0.11,0.09,0.16,0.0,0.08,0.43,0.39,1.1,0.13,0.11,0.23,0.0,0.16,0.62,0.48,1.14,0.29,0.29,0.39,0.0,0.26,0.86,0.59,1.06
23.0,1.24,0.05,0.05,0.08,0.0,0.0,0.12,0.07,1.34,0.06,0.07,0.12,0.0,0.01,0.2,0.15,1.3,0.07,0.07,0.13,0.0,0.02,0.34,0.2,1.34,0.09,0.08,0.13,0.0,0.04,0.42,0.34,1.28,0.12,0.09,0.17,0.0,0.08,0.44,0.39,1.12,0.13,0.11,0.23,0.0,0.16,0.62,0.48,1.15,0.29,0.29,0.4,0.0,0.26,0.87,0.6,1.06
24.0,1.25,0.05,0.05,0.08,0.0,0.0,0.12,0.07,1.36,0.06,0.07,0.12,0.0,0.01,0.21,0.16,1.3,0.07,0.07,0.13,0.0,0.02,0.34,0.21,1.35,0.09,0.08,0.13,0.0,0.04,0.43,0.34,1.31,0.12,0.09,0.17,0.0,0.08,0.44,0.4,1.14,0.15,0.12,0.23,0.0,0.16,0.64,0.49,1.15,0.3,0.3,0.4,0.0,0.26,0.88,0.6,1.06
25.0,1.26,0.05,0.05,0.08,0.0,0.0,0.13,0.07,1.36,0.07,0.07,0.12,0.0,0.01,0.21,0.16,1.33,0.07,0.07,0.14,0.0,0.02,0.34,0.21,1.36,0.09,0.08,0.13,0.0,0.04,0.43,0.34,1.31,0.12,0.09,0.17,0.0,0.08,0.44,0.4,1.15,0.15,0.12,0.24,0.0,0.16,0.65,0.5,1.16,0.3,0.3,0.4,0.0,0.26,0.89,0.6,1.07
26.0,1.27,0.05,0.05,0.08,0.0,0.0,0.13,0.07,1.37,0.07,0.07,0.12,0.0,0.01,0.22,0.16,1.34,0.07,0.07,0.14,0.0,0.02,0.35,0.22,1.41,0.1,0.09,0.13,0.0,0.04,0.43,0.34,1.32,0.12,0.1,0.18,0.0,0.08,0.44,0.4,1.16,0.16,0.12,0.24,0.0,0.16,0.66,0.5,1.17,0.3,0.3,0.4,0.0,0.26,0.9,0.61,1.07
27.0,1.28,0.06,0.05,0.08,0.0,0.0,0.13,0.08,1.41,0.07,0.07,0.12,0.0,0.01,0.23,0.16,1.34,0.07,0.07,0.15,0.0,0.02,0.36,0.22,1.42,0.1,0.09,0.13,0.0,0.04,0.43,0.35,1.33,0.12,0.1,0.18,0.0,0.08,0.45,0.4,1.16,0.17,0.12,0.25,0.0,0.16,0.67,0.5,1.17,0.3,0.3,0.4,0.0,0.26,0.95,0.61,1.08
28.0,1.28,0.06,0.05,0.08,0.0,0.0,0.14,0.08,1.42,0.07,0.07,0.13,0.0,0.01,0.23,0.16,1.35,0.07,0.07,0.15,0.0,0.02,0.36,0.23,1.43,0.1,0.09,0.14,0.0,0.04,0.43,0.35,1.33,0.12,0.1,0.18,0.0,0.08,0.45,0.4,1.17,0.17,0.12,0.25,0.0,0.16,0.68,0.51,1.18,0.31,0.31,0.4,0.0,0.26,0.96,0.62,1.08
29.0,1.28,0.06,0.05,0.09,0.0,0.0,0.15,0.08,1.43,0.07,0.07,0.13,0.0,0.01,0.24,0.16,1.36,0.08,0.07,0.15,0.0,0.02,0.36,0.23,1.44,0.1,0.09,0.15,0.0,0.04,0.43,0.36,1.35,0.13,0.1,0.19,0.0,0.08,0.46,0.41,1.19,0.17,0.12,0.27,0.0,0.16,0.69,0.51,1.2,0.31,0.31,0.4,0.0,0.26,0.99,0.64,1.09
30.0,1.29,0.06,0.06,0.09,0.0,0.0,0.16,0.08,1.44,0.07,0.07,0.13,0.0,0.01,0.24,0.17,1.38,0.08,0.07,0.15,0.0,0.02,0.36,0.25,1.47,0.1,0.09,0.15,0.0,0.04,0.44,0.36,1.35,0.14,0.1,0.2,0.0,0.08,0.46,0.41,1.2,0.17,0.14,0.27,0.0,0.16,0.69,0.52,1.21,0.31,0.31,0.41,0.0,0.26,1.0,0.64,1.11
31.0,1.31,0.06,0.06,0.09,0.0,0.0,0.16,0.08,1.46,0.07,0.07,0.13,0.0,0.01,0.26,0.17,1.4,0.08,0.07,0.15,0.0,0.02,0.37,0.25,1.5,0.11,0.09,0.15,0.0,0.04,0.44,0.36,1.36,0.14,0.1,0.2,0.0,0.08,0.47,0.41,1.22,0.19,0.14,0.3,0.0,0.16,0.7,0.52,1.22,0.31,0.31,0.41,0.0,0.26,1.02,0.64,1.11
32.0,1.35,0.06,0.06,0.09,0.0,0.0,0.17,0.09,1.46,0.07,0.07,0.13,0.0,0.01,0.26,0.18,1.4,0.08,0.07,0.15,0.0,0.02,0.37,0.25,1.5,0.11,0.09,0.16,0.0,0.04,0.45,0.36,1.37,0.14,0.1,0.21,0.0,0.08,0.47,0.42,1.24,0.19,0.14,0.3,0.0,0.16,0.71,0.53,1.24,0.32,0.32,0.41,0.0,0.26,1.03,0.65,1.14
33.0,1.36,0.06,0.06,0.09,0.0,0.0,0.17,0.09,1.48,0.07,0.08,0.13,0.0,0.01,0.26,0.18,1.43,0.08,0.07,0.15,0.0,0.02,0.37,0.26,1.51,0.11,0.09,0.16,0.0,0.04,0.45,0.37,1.39,0.15,0.1,0.22,0.0,0.08,0.47,0.42,1.24,0.19,0.15,0.3,0.0,0.16,0.71,0.53,1.27,0.32,0.32,0.41,0.0,0.26,1.04,0.67,1.15
34.0,1.36,0.06,0.06,0.09,0.0,0.0,0.18,0.09,1.5,0.07,0.08,0.14,0.0,0.01,0.26,0.18,1.44,0.08,0.07,0.15,0.0,0.02,0.38,0.27,1.51,0.11,0.09,0.16,0.0,0.04,0.45,0.37,1.4,0.15,0.11,0.22,0.0,0.08,0.48,0.42,1.25,0.2,0.15,0.31,0.0,0.16,0.72,0.54,1.27,0.32,0.32,0.41,0.0,0.27,1.04,0.67,1.15
35.0,1.36,0.06,0.06,0.09,0.0,0.0,0.19,0.1,1.58,0.07,0.08,0.14,0.0,0.01,0.27,0.18,1.45,0.08,0.07,0.16,0.0,0.02,0.38,0.27,1.53,0.11,0.09,0.17,0.0,0.04,0.46,0.37,1.41,0.16,0.11,0.22,0.0,0.08,0.48,0.43,1.25,0.2,0.15,0.31,0.0,0.16,0.72,0.55,1.28,0.32,0.32,0.41,0.0,0.27,1.05,0.67,1.17
36.0,1.38,0.06,0.06,0.1,0.0,0.0,0.19,0.1,1.58,0.07,0.08,0.14,0.0,0.01,0.27,0.19,1.45,0.08,0.07,0.16,0.0,0.02,0.4,0.27,1.54,0.11,0.09,0.17,0.0,0.04,0.46,0.38,1.42,0.16,0.11,0.22,0.0,0.08,0.48,0.44,1.26,0.2,0.15,0.31,0.0,0.16,0.73,0.55,1.29,0.32,0.32,0.41,0.0,0.27,1.09,0.68,1.21
37.0,1.38,0.06,0.06,0.1,0.0,0.0,0.19,0.1,1.59,0.07,0.08,0.14,0.0,0.01,0.29,0.19,1.48,0.09,0.07,0.16,0.0,0.02,0.4,0.27,1.57,0.11,0.09,0.18,0.0,0.04,0.46,0.38,1.43,0.16,0.11,0.23,0.0,0.08,0.48,0.44,1.26,0.2,0.16,0.31,0.0,0.16,0.73,0.55,1.32,0.32,0.32,0.41,0.0,0.27,1.1,0.69,1.24
38.0,1.4,0.06,0.06,0.1,0.0,0.0,0.19,0.1,1.59,0.07,0.08,0.14,0.0,0.01,0.29,0.19,1.48,0.09,0.08,0.16,0.0,0.02,0.4,0.28,1.59,0.12,0.09,0.18,0.0,0.04,0.47,0.39,1.45,0.17,0.11,0.23,0.0,0.08,0.49,0.45,1.26,0.21,0.16,0.32,0.0,0.16,0.74,0.56,1.32,0.32,0.32,0.41,0.0,0.27,1.1,0.69,1.25
39.0,1.4,0.06,0.06,0.1,0.0,0.0,0.2,0.1,1.59,0.07,0.08,0.15,0.0,0.01,0.29,0.2,1.49,0.09,0.08,0.16,0.0,0.02,0.4,0.29,1.62,0.12,0.1,0.18,0.0,0.04,0.47,0.39,1.46,0.17,0.11,0.23,0.0,0.08,0.49,0.45,1.26,0.21,0.16,0.32,0.0,0.16,0.75,0.57,1.33,0.32,0.32,0.41,0.0,0.28,1.11,0.7,1.25
40.0,1.42,0.06,0.06,0.1,0.0,0.0,0.2,0.1,1.61,0.07,0.08,0.15,0.0,0.01,0.3,0.21,1.51,0.09,0.08,0.16,0.0,0.02,0.41,0.3,1.63,0.12,0.1,0.18,0.0,0.04,0.48,0.39,1.46,0.17,0.11,0.23,0.0,0.08,0.49,0.46,1.26,0.21,0.16,0.32,0.0,0.16,0.75,0.57,1.35,0.33,0.33,0.42,0.0,0.28,1.12,0.71,1.27
41.0,1.42,0.06,0.06,0.1,0.0,0.0,0.2,0.1,1.62,0.07,0.08,0.15,0.0,0.01,0.3,0.21,1.51,0.09,0.08,0.17,0.0,0.02,0.41,0.3,1.64,0.12,0.1,0.19,0.0,0.04,0.48,0.39,1.47,0.18,0.11,0.24,0.0,0.08,0.49,0.47,1.28,0.22,0.16,0.32,0.0,0.16,0.76,0.57,1.36,0.33,0.33,0.42,0.0,0.28,1.13,0.71,1.28
42.0,1.43,0.06,0.06,0.1,0.0,0.0,0.21,0.11,1.66,0.07,0.08,0.15,0.0,0.01,0.31,0.21,1.56,0.09,0.08,0.17,0.0,0.02,0.41,0.3,1.64,0.13,0.1,0.19,0.0,0.04,0.48,0.4,1.48,0.18,0.11,0.24,0.0,0.08,0.5,0.47,1.29,0.22,0.16,0.32,0.0,0.16,0.77,0.61,1.37,0.33,0.33,0.42,0.0,0.29,1.13,0.71,1.28
43.0,1.43,0.07,0.06,0.1,0.0,0.0,0.21,0.11,1.66,0.07,0.08,0.16,0.0,0.01,0.31,0.21,1.59,0.09,0.08,0.18,0.0,0.02,0.41,0.31,1.65,0.13,0.1,0.2,0.0,0.04,0.49,0.41,1.48,0.18,0.12,0.25,0.0,0.08,0.51,0.47,1.33,0.23,0.17,0.33,0.0,0.16,0.77,0.62,1.37,0.33,0.33,0.42,0.0,0.3,1.15,0.72,1.28
44.0,1.43,0.07,0.06,0.1,0.0,0.0,0.21,0.11,1.66,0.08,0.08,0.16,0.0,0.01,0.31,0.22,1.63,0.09,0.08,0.18,0.0,0.02,0.41,0.31,1.65,0.13,0.1,0.2,0.0,0.04,0.49,0.41,1.48,0.18,0.12,0.25,0.0,0.08,0.52,0.47,1.33,0.23,0.17,0.33,0.0,0.16,0.77,0.62,1.38,0.33,0.33,0.42,0.0,0.3,1.16,0.73,1.29
45.0,1.44,0.07,0.06,0.1,0.0,0.0,0.21,0.11,1.69,0.08,0.08,0.16,0.0,0.01,0.32,0.22,1.64,0.09,0.08,0.18,0.0,0.02,0.42,0.31,1.66,0.13,0.1,0.2,0.0,0.04,0.49,0.41,1.48,0.19,0.12,0.25,0.0,0.08,0.54,0.48,1.34,0.23,0.17,0.33,0.0,0.16,0.79,0.62,1.39,0.33,0.33,0.42,0.0,0.3,1.17,0.73,1.29
46.0,1.44,0.07,0.06,0.1,0.0,0.0,0.21,0.11,1.69,0.08,0.08,0.16,0.0,0.01,0.32,0.22,1.64,0.09,0.08,0.18,0.0,0.02,0.42,0.32,1.66,0.14,0.1,0.21,0.0,0.04,0.49,0.41,1.49,0.19,0.12,0.26,0.0,0.08,0.54,0.48,1.35,0.24,0.17,0.33,0.0,0.16,0.79,0.63,1.39,0.34,0.34,0.42,0.0,0.3,1.17,0.74,1.3
47.0,1.46,0.07,0.06,0.1,0.0,0.0,0.22,0.11,1.71,0.08,0.08,0.16,0.0,0.01,0.32,0.23,1.65,0.1,0.08,0.18,0.0,0.02,0.42,0.32,1.67,0.14,0.1,0.21,0.0,0.04,0.5,0.41,1.51,0.19,0.12,0.27,0.0,0.08,0.54,0.48,1.36,0.25,0.17,0.33,0.0,0.16,0.8,0.63,1.4,0.34,0.34,0.42,0.0,0.31,1.18,0.75,1.3
48.0,1.46,0.07,0.06,0.1,0.0,0.0,0.22,0.11,1.71,0.08,0.08,0.17,0.0,0.01,0.32,0.23,1.68,0.1,0.09,0.19,0.0,0.02,0.42,0.32,1.67,0.14,0.1,0.21,0.0,0.04,0.5,0.42,1.51,0.2,0.12,0.27,0.0,0.08,0.54,0.48,1.36,0.26,0.18,0.33,0.0,0.16,0.82,0.63,1.41,0.34,0.34,0.42,0.0,0.32,1.18,0.76,1.32
49.0,1.46,0.07,0.06,0.11,0.0,0.0,0.23,0.12,1.72,0.08,0.08,0.17,0.0,0.01,0.32,0.23,1.69,0.1,0.09,0.2,0.0,0.02,0.43,0.32,1.69,0.14,0.1,0.21,0.0,0.04,0.5,0.42,1.52,0.2,0.12,0.27,0.0,0.08,0.54,0.49,1.37,0.26,0.19,0.33,0.0,0.16,0.82,0.64,1.43,0.34,0.34,0.43,0.0,0.33,1.19,0.76,1.33
50.0,1.47,0.07,0.06,0.11,0.0,0.0,0.23,0.12,1.79,0.08,0.08,0.17,0.0,0.01,0.32,0.24,1.72,0.1,0.09,0.2,0.0,0.02,0.43,0.32,1.69,0.15,0.1,0.22,0.0,0.04,0.51,0.42,1.55,0.2,0.12,0.28,0.0,0.08,0.55,0.49,1.37,0.26,0.19,0.34,0.0,0.16,0.82,0.65,1.44,0.34,0.34,0.43,0.0,0.33,1.19,0.77,1.33
51.0,1.5,0.07,0.06,0.11,0.0,0.0,0.23,0.12,1.79,0.08,0.08,0.17,0.0,0.01,0.32,0.24,1.72,0.1,0.09,0.21,0.0,0.02,0.44,0.32,1.7,0.15,0.1,0.22,0.0,0.04,0.51,0.42,1.55,0.21,0.13,0.29,0.0,0.08,0.56,0.49,1.39,0.27,0.19,0.34,0.0,0.16,0.85,0.65,1.44,0.34,0.34,0.43,0.0,0.33,1.2,0.77,1.33
52.0,1.54,0.07,0.06,0.11,0.0,0.0,0.24,0.12,1.8,0.08,0.08,0.17,0.0,0.01,0.32,0.25,1.72,0.1,0.09,0.21,0.0,0.02,0.44,0.32,1.7,0.16,0.11,0.22,0.0,0.04,0.51,0.42,1.57,0.21,0.13,0.29,0.0,0.08,0.57,0.5,1.41,0.27,0.19,0.34,0.0,0.16,0.88,0.65,1.46,0.35,0.35,0.43,0.0,0.33,1.2,0.78,1.33
53.0,1.56,0.07,0.06,0.11,0.0,0.0,0.24,0.13,1.81,0.08,0.08,0.18,0.0,0.01,0.33,0.25,1.74,0.1,0.09,0.21,0.0,0.02,0.45,0.33,1.75,0.16,0.11,0.23,0.0,0.04,0.53,0.42,1.6,0.21,0.13,0.29,0.0,0.08,0.57,0.51,1.41,0.28,0.19,0.34,0.0,0.16,0.89,0.65,1.47,0.35,0.35,0.43,0.0,0.33,1.21,0.79,1.34
54.0,1.57,0.07,0.06,0.11,0.0,0.0,0.25,0.13,1.81,0.08,0.08,0.18,0.0,0.01,0.33,0.26,1.78,0.1,0.09,0.21,0.0,0.02,0.45,0.33,1.75,0.16,0.11,0.23,0.0,0.04,0.54,0.43,1.62,0.21,0.14,0.3,0.0,0.08,0.58,0.51,1.42,0.28,0.19,0.35,0.0,0.16,0.89,0.65,1.48,0.35,0.35,0.43,0.0,0.34,1.21,0.79,1.34
55.0,1.59,0.07,0.06,0.11,0.0,0.0,0.25,0.13,1.82,0.08,0.08,0.18,0.0,0.01,0.34,0.27,1.79,0.1,0.09,0.21,0.0,0.02,0.45,0.33,1.76,0.16,0.11,0.23,0.0,0.04,0.54,0.43,1.62,0.21,0.14,0.3,0.0,0.08,0.59,0.51,1.42,0.29,0.2,0.35,0.0,0.16,0.89,0.66,1.48,0.35,0.35,0.43,0.0,0.34,1.23,0.79,1.35
56.0,1.59,0.07,0.06,0.12,0.0,0.0,0.25,0.13,1.83,0.08,0.08,0.19,0.0,0.01,0.36,0.27,1.8,0.1,0.09,0.21,0.0,0.02,0.45,0.34,1.77,0.17,0.11,0.23,0.0,0.04,0.54,0.44,1.63,0.21,0.14,0.3,0.0,0.08,0.59,0.51,1.44,0.29,0.2,0.35,0.0,0.16,0.9,0.67,1.51,0.35,0.35,0.43,0.0,0.34,1.23,0.8,1.36
57.0,1.59,0.07,0.06,0.12,0.0,0.0,0.26,0.13,1.84,0.09,0.08,0.19,0.0,0.01,0.37,0.27,1.81,0.1,0.09,0.22,0.0,0.02,0.45,0.34,1.78,0.17,0.11,0.23,0.0,0.04,0.56,0.44,1.63,0.22,0.15,0.3,0.0,0.08,0.6,0.52,1.45,0.29,0.2,0.35,0.0,0.16,0.9,0.67,1.52,0.35,0.35,0.43,0.0,0.34,1.26,0.8,1.36
58.0,1.6,0.07,0.06,0.12,0.0,0.0,0.26,0.14,1.9,0.09,0.08,0.19,0.0,0.01,0.37,0.27,1.83,0.11,0.1,0.22,0.0,0.02,0.45,0.34,1.79,0.17,0.11,0.24,0.0,0.04,0.56,0.44,1.64,0.22,0.15,0.3,0.0,0.08,0.6,0.52,1.45,0.29,0.21,0.35,0.0,0.16,0.91,0.68,1.52,0.35,0.35,0.43,0.0,0.35,1.26,0.8,1.36
59.0,1.63,0.07,0.06,0.12,0.0,0.0,0.26,0.14,1.9,0.09,0.08,0.19,0.0,0.01,0.37,0.27,1.83,0.11,0.1,0.22,0.0,0.02,0.45,0.35,1.8,0.17,0.12,0.25,0.0,0.04,0.57,0.44,1.65,0.22,0.15,0.3,0.0,0.08,0.61,0.52,1.47,0.29,0.21,0.35,0.0,0.16,0.93,0.68,1.52,0.35,0.35,0.43,0.0,0.35,1.28,0.81,1.39
60.0,1.64,0.07,0.06,0.12,0.0,0.0,0.26,0.15,1.91,0.09,0.09,0.19,0.0,0.01,0.37,0.28,1.83,0.11,0.1,0.22,0.0,0.02,0.46,0.35,1.82,0.18,0.12,0.25,0.0,0.04,0.57,0.45,1.65,0.22,0.16,0.3,0.0,0.08,0.62,0.52,1.47,0.3,0.21,0.35,0.0,0.16,0.94,0.68,1.53,0.35,0.35,0.43,0.0,0.36,1.29,0.81,1.4
61.0,1.64,0.07,0.06,0.12,0.0,0.0,0.26,0.15,1.94,0.09,0.09,0.19,0.0,0.01,0.37,0.29,1.84,0.11,0.1,0.22,0.0,0.02,0.46,0.35,1.83,0.18,0.12,0.25,0.0,0.04,0.58,0.45,1.67,0.22,0.16,0.31,0.0,0.08,0.64,0.52,1.48,0.3,0.22,0.36,0.0,0.16,0.94,0.69,1.53,0.35,0.35,0.43,0.0,0.36,1.3,0.82,1.42
62.0,1.64,0.07,0.06,0.12,0.0,0.0,0.26,0.15,1.98,0.09,0.09,0.2,0.0,0.01,0.38,0.29,1.85,0.11,0.1,0.22,0.0,0.02,0.46,0.35,1.83,0.19,0.12,0.25,0.0,0.04,0.58,0.45,1.67,0.22,0.16,0.31,0.0,0.08,0.64,0.53,1.49,0.3,0.22,0.36,0.0,0.16,0.94,0.7,1.54,0.35,0.35,0.43,0.0,0.36,1.32,0.82,1.42
63.0,1.64,0.07,0.07,0.12,0.0,0.0,0.26,0.16,1.98,0.09,0.09,0.2,0.0,0.01,0.38,0.29,1.87,0.11,0.1,0.23,0.0,0.02,0.47,0.35,1.85,0.19,0.13,0.25,0.0,0.04,0.58,0.45,1.67,0.22,0.17,0.32,0.0,0.08,0.65,0.54,1.52,0.3,0.23,0.36,0.0,0.16,0.94,0.71,1.55,0.36,0.36,0.43,0.0,0.36,1.32,0.82,1.42
64.0,1.64,0.07,0.07,0.12,0.0,0.0,0.26,0.16,2.0,0.09,0.09,0.2,0.0,0.01,0.38,0.3,1.87,0.11,0.1,0.23,0.0,0.02,0.47,0.35,1.9,0.19,0.13,0.25,0.0,0.04,0.6,0.46,1.69,0.23,0.17,0.32,0.0,0.08,0.65,0.54,1.54,0.31,0.23,0.36,0.0,0.16,0.95,0.71,1.55,0.36,0.36,0.43,0.0,0.36,1.35,0.83,1.43
65.0,1.67,0.07,0.07,0.13,0.0,0.0,0.27,0.17,2.0,0.09,0.09,0.2,0.0,0.01,0.38,0.31,1.88,0.11,0.1,0.23,0.0,0.02,0.47,0.35,1.9,0.19,0.13,0.25,0.0,0.04,0.6,0.46,1.7,0.23,0.17,0.32,0.0,0.08,0.66,0.56,1.55,0.31,0.23,0.36,0.0,0.16,0.96,0.72,1.55,0.36,0.36,0.44,0.0,0.36,1.38,0.83,1.44
66.0,1.7,0.07,0.07,0.13,0.0,0.0,0.27,0.18,2.02,0.1,0.09,0.2,0.0,0.01,0.39,0.31,1.89,0.11,0.1,0.23,0.0,0.02,0.48,0.35,1.94,0.19,0.14,0.26,0.0,0.04,0.6,0.46,1.7,0.23,0.17,0.32,0.0,0.08,0.67,0.57,1.55,0.31,0.23,0.36,0.0,0.16,0.96,0.72,1.55,0.36,0.36,0.44,0.0,0.37,1.38,0.84,1.44
67.0,1.71,0.07,0.07,0.13,0.0,0.0,0.27,0.19,2.02,0.1,0.09,0.2,0.0,0.01,0.39,0.31,1.96,0.11,0.1,0.23,0.0,0.02,0.48,0.36,1.98,0.2,0.14,0.26,0.0,0.04,0.6,0.46,1.72,0.23,0.17,0.32,0.0,0.08,0.67,0.57,1.56,0.31,0.23,0.36,0.0,0.16,0.97,0.73,1.55,0.36,0.36,0.44,0.0,0.37,1.39,0.85,1.45
68.0,1.71,0.07,0.07,0.13,0.0,0.0,0.27,0.19,2.06,0.1,0.09,0.2,0.0,0.01,0.39,0.32,1.98,0.11,0.1,0.23,0.0,0.02,0.48,0.36,1.99,0.2,0.14,0.27,0.0,0.04,0.61,0.46,1.72,0.23,0.18,0.32,0.0,0.08,0.67,0.57,1.57,0.31,0.23,0.36,0.0,0.16,0.98,0.74,1.55,0.36,0.36,0.44,0.0,0.37,1.39,0.85,1.47
69.0,1.71,0.07,0.07,0.13,0.0,0.0,0.27,0.19,2.08,0.1,0.09,0.21,0.0,0.01,0.39,0.32,2.04,0.12,0.1,0.23,0.0,0.02,0.49,0.37,2.01,0.2,0.14,0.27,0.0,0.04,0.62,0.46,1.74,0.24,0.18,0.32,0.0,0.08,0.68,0.57,1.58,0.31,0.23,0.37,0.0,0.16,0.99,0.75,1.56,0.36,0.36,0.44,0.0,0.37,1.39,0.85,1.48
70.0,1.72,0.07,0.07,0.13,0.0,0.0,0.27,0.19,2.08,0.1,0.09,0.21,0.0,0.01,0.39,0.32,2.04,0.12,0.1,0.23,0.0,0.02,0.49,0.37,2.03,0.2,0.14,0.27,0.0,0.04,0.63,0.46,1.76,0.24,0.18,0.32,0.0,0.08,0.68,0.58,1.61,0.31,0.23,0.37,0.0,0.16,1.02,0.75,1.56,0.36,0.36,0.44,0.0,0.37,1.4,0.86,1.5
71.0,1.73,0.07,0.07,0.13,0.0,0.0,0.27,0.19,2.12,0.1,0.09,0.21,0.0,0.01,0.39,0.32,2.05,0.12,0.1,0.23,0.0,0.02,0.49,0.37,2.03,0.2,0.14,0.27,0.0,0.04,0.64,0.47,1.77,0.25,0.19,0.33,0.0,0.08,0.7,0.58,1.63,0.31,0.23,0.37,0.0,0.16,1.04,0.76,1.56,0.36,0.36,0.44,0.0,0.38,1.41,0.86,1.51
72.0,1.74,0.07,0.07,0.14,0.0,0.0,0.27,0.2,2.16,0.1,0.09,0.21,0.0,0.01,0.39,0.32,2.06,0.13,0.1,0.24,0.0,0.02,0.5,0.37,2.04,0.2,0.14,0.27,0.0,0.04,0.64,0.47,1.77,0.25,0.19,0.33,0.0,0.08,0.7,0.58,1.63,0.32,0.24,0.37,0.0,0.16,1.07,0.77,1.57,0.36,0.36,0.44,0.0,0.38,1.41,0.87,1.52
73.0,1.77,0.08,0.07,0.14,0.0,0.0,0.28,0.2,2.17,0.1,0.09,0.21,0.0,0.01,0.39,0.33,2.07,0.13,0.1,0.24,0.0,0.02,0.5,0.37,2.06,0.21,0.14,0.27,0.0,0.04,0.65,0.47,1.79,0.25,0.19,0.33,0.0,0.08,0.71,0.58,1.65,0.32,0.24,0.37,0.0,0.16,1.07,0.77,1.58,0.36,0.36,0.45,0.0,0.38,1.43,0.88,1.55
74.0,1.8,0.08,0.07,0.14,0.0,0.0,0.28,0.2,2.19,0.1,0.09,0.21,0.0,0.01,0.4,0.33,2.08,0.13,0.1,0.24,0.0,0.02,0.5,0.38,2.08,0.21,0.15,0.28,0.0,0.04,0.65,0.47,1.8,0.25,0.2,0.33,0.0,0.08,0.72,0.59,1.65,0.32,0.24,0.37,0.0,0.16,1.08,0.78,1.59,0.36,0.36,0.45,0.0,0.39,1.43,0.89,1.55
75.0,1.8,0.08,0.07,0.15,0.0,0.0,0.28,0.2,2.23,0.1,0.09,0.21,0.0,0.01,0.4,0.34,2.09,0.13,0.1,0.24,0.0,0.02,0.5,0.38,2.08,0.21,0.15,0.28,0.0,0.04,0.65,0.47,1.81,0.26,0.2,0.33,0.0,0.08,0.74,0.59,1.66,0.32,0.24,0.37,0.0,0.16,1.09,0.78,1.62,0.36,0.36,0.45,0.0,0.39,1.43,0.9,1.58
76.0,1.8,0.08,0.07,0.16,0.0,0.0,0.29,0.21,2.24,0.1,0.1,0.21,0.0,0.01,0.4,0.34,2.14,0.13,0.11,0.24,0.0,0.02,0.51,0.38,2.11,0.21,0.15,0.28,0.0,0.04,0.65,0.47,1.83,0.26,0.2,0.33,0.0,0.08,0.74,0.59,1.68,0.32,0.24,0.38,0.0,0.16,1.09,0.78,1.63,0.36,0.36,0.45,0.0,0.39,1.44,0.91,1.61
77.0,1.8,0.08,0.07,0.16,0.0,0.0,0.29,0.22,2.26,0.1,0.1,0.21,0.0,0.01,0.4,0.34,2.15,0.13,0.11,0.24,0.0,0.02,0.51,0.39,2.14,0.22,0.15,0.28,0.0,0.04,0.66,0.47,1.83,0.26,0.2,0.33,0.0,0.08,0.75,0.6,1.68,0.32,0.25,0.38,0.0,0.16,1.1,0.78,1.64,0.36,0.36,0.45,0.0,0.39,1.45,0.92,1.63
78.0,1.81,0.08,0.08,0.16,0.0,0.0,0.29,0.22,2.26,0.1,0.1,0.21,0.0,0.01,0.4,0.35,2.16,0.14,0.11,0.24,0.0,0.02,0.51,0.39,2.14,0.22,0.15,0.29,0.0,0.04,0.68,0.47,1.86,0.26,0.2,0.34,0.0,0.08,0.75,0.6,1.68,0.32,0.25,0.38,0.0,0.16,1.1,0.79,1.65,0.36,0.36,0.45,0.0,0.39,1.46,0.94,1.63
79.0,1.82,0.08,0.08,0.16,0.0,0.0,0.29,0.22,2.27,0.1,0.1,0.22,0.0,0.01,0.4,0.35,2.19,0.14,0.11,0.24,0.0,0.02,0.51,0.39,2.16,0.22,0.15,0.29,0.0,0.04,0.68,0.48,1.88,0.26,0.2,0.34,0.0,0.08,0.76,0.6,1.69,0.32,0.26,0.38,0.0,0.16,1.1,0.79,1.65,0.37,0.37,0.45,0.0,0.39,1.46,0.94,1.64
80.0,1.82,0.08,0.08,0.16,0.0,0.0,0.29,0.23,2.27,0.1,0.1,0.22,0.0,0.01,0.4,0.35,2.19,0.14,0.11,0.25,0.0,0.02,0.51,0.4,2.16,0.22,0.15,0.29,0.0,0.04,0.68,0.48,1.89,0.27,0.2,0.34,0.0,0.08,0.77,0.6,1.69,0.32,0.26,0.38,0.0,0.16,1.1,0.79,1.66,0.37,0.37,0.45,0.0,0.39,1.47,0.95,1.65
81.0,1.83,0.08,0.08,0.16,0.0,0.0,0.3,0.23,2.28,0.1,0.1,0.22,0.0,0.01,0.41,0.36,2.2,0.14,0.11,0.25,0.0,0.02,0.51,0.4,2.2,0.23,0.15,0.3,0.0,0.04,0.69,0.48,1.9,0.27,0.2,0.34,0.0,0.08,0.78,0.61,1.7,0.32,0.27,0.38,0.0,0.16,1.11,0.81,1.67,0.37,0.37,0.45,0.0,0.39,1.47,0.96,1.66
82.0,1.84,0.08,0.08,0.17,0.0,0.0,0.3,0.23,2.29,0.1,0.1,0.22,0.0,0.01,0.41,0.36,2.21,0.14,0.11,0.25,0.0,0.02,0.51,0.4,2.21,0.23,0.15,0.3,0.0,0.04,0.7,0.49,1.9,0.27,0.2,0.34,0.0,0.08,0.78,0.61,1.72,0.33,0.27,0.38,0.0,0.16,1.12,0.81,1.69,0.37,0.37,0.45,0.0,0.39,1.47,0.96,1.68
83.0,1.85,0.08,0.08,0.17,0.0,0.0,0.3,0.23,2.3,0.1,0.1,0.22,0.0,0.01,0.41,0.37,2.22,0.14,0.11,0.25,0.0,0.02,0.53,0.42,2.23,0.23,0.15,0.3,0.0,0.04,0.7,0.49,1.93,0.28,0.2,0.34,0.0,0.08,0.79,0.62,1.72,0.33,0.27,0.39,0.0,0.16,1.12,0.81,1.69,0.37,0.37,0.45,0.0,0.39,1.48,0.97,1.68
84.0,1.86,0.08,0.08,0.17,0.0,0.0,0.3,0.24,2.32,0.1,0.1,0.22,0.0,0.01,0.41,0.37,2.23,0.14,0.12,0.25,0.0,0.02,0.53,0.42,2.24,0.23,0.15,0.3,0.0,0.04,0.7,0.49,1.94,0.28,0.21,0.34,0.0,0.08,0.81,0.63,1.72,0.33,0.27,0.39,0.0,0.16,1.13,0.81,1.69,0.37,0.37,0.46,0.0,0.39,1.49,0.97,1.7
85.0,1.88,0.08,0.08,0.17,0.0,0.0,0.3,0.24,2.34,0.1,0.1,0.22,0.0,0.01,0.41,0.37,2.24,0.15,0.12,0.26,0.0,0.02,0.53,0.42,2.24,0.23,0.15,0.3,0.0,0.04,0.71,0.5,1.95,0.28,0.21,0.34,0.0,0.08,0.81,0.64,1.74,0.33,0.27,0.39,0.0,0.16,1.13,0.82,1.7,0.37,0.37,0.46,0.0,0.39,1.49,0.98,1.71
86.0,1.88,0.08,0.08,0.17,0.0,0.0,0.31,0.24,2.37,0.1,0.1,0.23,0.0,0.01,0.41,0.37,2.24,0.15,0.12,0.26,0.0,0.02,0.53,0.43,2.24,0.23,0.15,0.3,0.0,0.04,0.71,0.51,1.98,0.28,0.21,0.34,0.0,0.08,0.82,0.65,1.76,0.33,0.27,0.39,0.0,0.16,1.13,0.82,1.7,0.37,0.37,0.46,0.0,0.39,1.5,0.98,1.72
87.0,1.89,0.08,0.08,0.17,0.0,0.0,0.31,0.24,2.41,0.1,0.1,0.23,0.0,0.01,0.42,0.37,2.25,0.15,0.12,0.26,0.0,0.02,0.54,0.43,2.25,0.24,0.16,0.31,0.0,0.04,0.75,0.51,1.99,0.29,0.21,0.34,0.0,0.08,0.82,0.65,1.78,0.33,0.28,0.39,0.0,0.16,1.14,0.82,1.71,0.37,0.37,0.46,0.0,0.39,1.53,0.98,1.73
88.0,1.89,0.08,0.08,0.17,0.0,0.0,0.31,0.24,2.41,0.1,0.1,0.23,0.0,0.01,0.42,0.37,2.28,0.15,0.12,0.26,0.0,0.02,0.54,0.43,2.26,0.24,0.16,0.31,0.0,0.04,0.75,0.51,2.01,0.29,0.21,0.34,0.0,0.08,0.82,0.66,1.79,0.34,0.28,0.39,0.0,0.16,1.15,0.82,1.75,0.37,0.37,0.46,0.0,0.39,1.54,1.0,1.73
89.0,1.9,0.08,0.08,0.18,0.0,0.0,0.31,0.24,2.42,0.1,0.1,0.23,0.0,0.01,0.42,0.37,2.28,0.15,0.12,0.26,0.0,0.02,0.54,0.43,2.27,0.24,0.16,0.32,0.0,0.04,0.75,0.51,2.03,0.29,0.22,0.35,0.0,0.08,0.83,0.67,1.8,0.34,0.28,0.39,0.0,0.16,1.17,0.83,1.75,0.37,0.37,0.46,0.0,0.39,1.54,1.0,1.74
90.0,1.91,0.08,0.08,0.18,0.0,0.0,0.31,0.25,2.44,0.11,0.1,0.23,0.0,0.01,0.42,0.37,2.28,0.15,0.12,0.26,0.0,0.02,0.54,0.43,2.32,0.24,0.16,0.32,0.0,0.04,0.75,0.52,2.05,0.29,0.22,0.35,0.0,0.08,0.84,0.67,1.8,0.34,0.28,0.39,0.0,0.16,1.18,0.83,1.75,0.38,0.38,0.46,0.0,0.39,1.55,1.01,1.74
91.0,1.93,0.08,0.08,0.18,0.0,0.0,0.31,0.25,2.46,0.11,0.1,0.23,0.0,0.01,0.42,0.38,2.28,0.15,0.12,0.26,0.0,0.02,0.54,0.43,2.34,0.25,0.16,0.32,0.0,0.04,0.76,0.52,2.06,0.29,0.22,0.35,0.0,0.08,0.84,0.67,1.81,0.34,0.28,0.39,0.0,0.16,1.19,0.84,1.76,0.38,0.38,0.46,0.0,0.39,1.55,1.04,1.74
92.0,1.95,0.08,0.08,0.18,0.0,0.0,0.32,0.25,2.5,0.11,0.11,0.23,0.0,0.01,0.43,0.38,2.3,0.16,0.12,0.26,0.0,0.02,0.55,0.44,2.36,0.25,0.16,0.32,0.0,0.04,0.76,0.52,2.08,0.29,0.22,0.35,0.0,0.08,0.84,0.68,1.83,0.34,0.28,0.39,0.0,0.16,1.19,0.85,1.77,0.38,0.38,0.46,0.0,0.39,1.56,1.05,1.75
93.0,2.0,0.09,0.08,0.19,0.0,0.0,0.32,0.25,2.52,0.11,0.11,0.23,0.0,0.01,0.43,0.38,2.31,0.16,0.12,0.26,0.0,0.02,0.56,0.44,2.39,0.25,0.16,0.32,0.0,0.04,0.76,0.52,2.13,0.29,0.22,0.35,0.0,0.08,0.85,0.68,1.85,0.34,0.29,0.39,0.0,0.16,1.19,0.85,1.78,0.38,0.38,0.47,0.0,0.39,1.58,1.05,1.75
94.0,2.02,0.09,0.08,0.19,0.0,0.0,0.32,0.25,2.52,0.11,0.11,0.24,0.0,0.01,0.44,0.38,2.32,0.16,0.12,0.27,0.0,0.02,0.57,0.44,2.43,0.25,0.16,0.32,0.0,0.04,0.76,0.52,2.14,0.29,0.22,0.36,0.0,0.08,0.85,0.68,1.87,0.34,0.29,0.39,0.0,0.16,1.19,0.85,1.8,0.38,0.38,0.47,0.0,0.39,1.58,1.06,1.76
95.0,2.02,0.09,0.08,0.19,0.0,0.0,0.32,0.25,2.54,0.11,0.11,0.24,0.0,0.01,0.45,0.38,2.35,0.16,0.12,0.27,0.0,0.02,0.57,0.45,2.46,0.25,0.16,0.32,0.0,0.04,0.76,0.52,2.2,0.29,0.22,0.36,0.0,0.08,0.86,0.68,1.87,0.34,0.29,0.4,0.0,0.16,1.2,0.85,1.83,0.38,0.38,0.47,0.0,0.39,1.59,1.08,1.77
96.0,2.05,0.09,0.08,0.19,0.0,0.0,0.32,0.25,2.54,0.11,0.11,0.24,0.0,0.01,0.45,0.39,2.4,0.16,0.13,0.27,0.0,0.02,0.58,0.45,2.48,0.25,0.17,0.32,0.0,0.04,0.77,0.54,2.2,0.3,0.23,0.36,0.0,0.08,0.86,0.69,1.88,0.34,0.29,0.4,0.0,0.16,1.22,0.86,1.84,0.38,0.38,0.47,0.0,0.39,1.59,1.08,1.82
97.0,2.05,0.09,0.08,0.19,0.0,0.0,0.32,0.25,2.58,0.11,0.11,0.24,0.0,0.01,0.45,0.39,2.41,0.16,0.13,0.28,0.0,0.02,0.58,0.45,2.49,0.25,0.17,0.32,0.0,0.04,0.77,0.54,2.23,0.3,0.23,0.36,0.0,0.08,0.88,0.69,1.88,0.35,0.29,0.4,0.0,0.16,1.22,0.86,1.85,0.38,0.38,0.47,0.0,0.39,1.59,1.08,1.83
98.0,2.05,0.09,0.08,0.19,0.0,0.0,0.33,0.26,2.58,0.11,0.11,0.24,0.0,0.01,0.45,0.39,2.41,0.16,0.13,0.28,0.0,0.02,0.58,0.45,2.49,0.25,0.17,0.32,0.0,0.04,0.78,0.55,2.25,0.3,0.23,0.36,0.0,0.08,0.89,0.69,1.88,0.35,0.29,0.4,0.0,0.16,1.24,0.86,1.88,0.38,0.38,0.47,0.0,0.39,1.59,1.08,1.83
99.0,2.06,0.09,0.08,0.19,0.0,0.0,0.33,0.26,2.59,0.11,0.11,0.25,0.0,0.01,0.45,0.39,2.42,0.16,0.13,0.28,0.0,0.02,0.58,0.46,2.51,0.25,0.17,0.32,0.0,0.04,0.78,0.55,2.27,0.3,0.23,0.36,0.0,0.08,0.89,0.7,1.93,0.35,0.29,0.4,0.0,0.16,1.27,0.87,1.95,0.39,0.39,0.47,0.0,0.39,1.59,1.08,1.83
100.0,2.06,0.09,0.08,0.19,0.0,0.0,0.33,0.26,2.59,0.12,0.11,0.25,0.0,0.01,0.46,0.39,2.43,0.16,0.13,0.28,0.0,0.02,0.58,0.46,2.55,0.26,0.17,0.33,0.0,0.04,0.78,0.55,2.28,0.3,0.23,0.36,0.0,0.08,0.89,0.7,1.95,0.35,0.29,0.4,0.0,0.16,1.27,0.88,1.95,0.39,0.39,0.47,0.0,0.39,1.59,1.09,1.84
101.0,2.08,0.09,0.08,0.19,0.0,0.0,0.33,0.26,2.6,0.12,0.12,0.25,0.0,0.01,0.46,0.39,2.48,0.16,0.13,0.28,0.0,0.02,0.59,0.46,2.55,0.26,0.17,0.33,0.0,0.04,0.78,0.55,2.29,0.3,0.23,0.36,0.0,0.08,0.9,0.71,1.95,0.35,0.3,0.4,0.0,0.16,1.28,0.88,1.96,0.39,0.39,0.47,0.0,0.39,1.64,1.11,1.86
102.0,2.08,0.09,0.08,0.2,0.0,0.0,0.34,0.27,2.62,0.12,0.12,0.25,0.0,0.01,0.46,0.4,2.49,0.16,0.14,0.28,0.0,0.02,0.59,0.46,2.57,0.26,0.17,0.33,0.0,0.04,0.81,0.56,2.32,0.3,0.24,0.36,0.0,0.08,0.91,0.71,1.96,0.35,0.3,0.4,0.0,0.16,1.3,0.88,1.96,0.39,0.39,0.48,0.0,0.39,1.64,1.11,1.87
103.0,2.09,0.09,0.08,0.2,0.0,0.0,0.34,0.27,2.62,0.12,0.12,0.25,0.0,0.01,0.47,0.4,2.51,0.16,0.14,0.28,0.0,0.02,0.59,0.46,2.59,0.26,0.18,0.33,0.0,0.04,0.81,0.56,2.32,0.3,0.24,0.36,0.0,0.08,0.91,0.71,1.98,0.35,0.3,0.4,0.0,0.16,1.32,0.89,1.98,0.39,0.39,0.48,0.0,0.4,1.67,1.11,1.89
104.0,2.1,0.09,0.09,0.2,0.0,0.0,0.35,0.27,2.62,0.12,0.12,0.25,0.0,0.01,0.47,0.4,2.52,0.16,0.14,0.28,0.0,0.02,0.6,0.46,2.6,0.26,0.18,0.33,0.0,0.04,0.81,0.57,2.33,0.3,0.25,0.36,0.0,0.08,0.92,0.72,2.0,0.35,0.3,0.4,0.0,0.16,1.33,0.89,2.02,0.39,0.39,0.48,0.0,0.4,1.67,1.12,1.9
105.0,2.1,0.09,0.09,0.2,0.0,0.0,0.35,0.27,2.64,0.12,0.12,0.26,0.0,0.01,0.47,0.41,2.52,0.17,0.14,0.29,0.0,0.02,0.61,0.46,2.65,0.26,0.18,0.33,0.0,0.04,0.82,0.57,2.35,0.3,0.25,0.37,0.0,0.08,0.92,0.72,2.0,0.35,0.3,0.4,0.0,0.16,1.33,0.9,2.03,0.39,0.39,0.48,0.0,0.4,1.67,1.12,1.92
106.0,2.1,0.09,0.09,0.21,0.0,0.0,0.35,0.27,2.66,0.13,0.12,0.26,0.0,0.01,0.47,0.41,2.53,0.17,0.14,0.29,0.0,0.02,0.61,0.46,2.67,0.27,0.18,0.34,0.0,0.04,0.83,0.57,2.37,0.3,0.25,0.37,0.0,0.08,0.93,0.72,2.01,0.36,0.3,0.41,0.0,0.16,1.33,0.9,2.04,0.39,0.39,0.48,0.0,0.4,1.68,1.12,1.93
107.0,2.13,0.09,0.09,0.21,0.0,0.0,0.35,0.27,2.66,0.13,0.12,0.26,0.0,0.01,0.47,0.41,2.54,0.17,0.14,0.29,0.0,0.02,0.61,0.46,2.71,0.27,0.18,0.34,0.0,0.04,0.84,0.57,2.38,0.3,0.25,0.37,0.0,0.08,0.94,0.72,2.01,0.36,0.3,0.41,0.0,0.16,1.34,0.9,2.04,0.39,0.39,0.48,0.0,0.4,1.69,1.12,1.93
108.0,2.15,0.09,0.09,0.21,0.0,0.0,0.36,0.27,2.67,0.13,0.12,0.26,0.0,0.01,0.47,0.42,2.54,0.17,0.14,0.29,0.0,0.02,0.62,0.46,2.73,0.28,0.18,0.35,0.0,0.04,0.86,0.58,2.38,0.3,0.25,0.37,0.0,0.08,0.94,0.72,2.02,0.36,0.3,0.41,0.0,0.16,1.34,0.9,2.05,0.39,0.39,0.48,0.0,0.4,1.7,1.13,1.94
109.0,2.16,0.09,0.09,0.21,0.0,0.0,0.36,0.27,2.67,0.13,0.12,0.26,0.0,0.01,0.48,0.42,2.55,0.17,0.14,0.29,0.0,0.02,0.62,0.46,2.73,0.28,0.18,0.35,0.0,0.04,0.87,0.58,2.38,0.31,0.26,0.37,0.0,0.08,0.94,0.72,2.03,0.36,0.3,0.41,0.0,0.16,1.35,0.91,2.06,0.39,0.39,0.48,0.0,0.4,1.7,1.13,1.94
110.0,2.18,0.09,0.09,0.21,0.0,0.0,0.36,0.27,2.67,0.13,0.12,0.27,0.0,0.01,0.49,0.42,2.56,0.17,0.14,0.29,0.0,0.02,0.62,0.46,2.73,0.28,0.18,0.35,0.0,0.04,0.88,0.59,2.39,0.31,0.26,0.37,0.0,0.08,0.95,0.73,2.03,0.36,0.31,0.41,0.0,0.16,1.36,0.92,2.06,0.4,0.4,0.48,0.0,0.4,1.72,1.14,1.96
111.0,2.18,0.09,0.09,0.21,0.0,0.0,0.36,0.28,2.7,0.13,0.12,0.27,0.0,0.01,0.49,0.43,2.58,0.18,0.14,0.3,0.0,0.02,0.63,0.47,2.74,0.28,0.18,0.35,0.0,0.04,0.89,0.59,2.41,0.31,0.26,0.37,0.0,0.08,0.96,0.73,2.04,0.36,0.31,0.41,0.0,0.16,1.37,0.92,2.08,0.4,0.4,0.48,0.0,0.4,1.73,1.14,2.03
112.0,2.2,0.09,0.09,0.21,0.0,0.0,0.37,0.28,2.71,0.13,0.12,0.27,0.0,0.01,0.49,0.43,2.59,0.18,0.14,0.3,0.0,0.02,0.63,0.47,2.74,0.28,0.19,0.35,0.0,0.04,0.89,0.59,2.41,0.31,0.26,0.37,0.0,0.08,0.96,0.73,2.04,0.36,0.31,0.41,0.0,0.16,1.38,0.93,2.09,0.4,0.4,0.49,0.0,0.4,1.73,1.14,2.04
113.0,2.2,0.09,0.09,0.22,0.0,0.0,0.37,0.28,2.71,0.13,0.12,0.28,0.0,0.01,0.49,0.43,2.62,0.18,0.14,0.3,0.0,0.02,0.63,0.47,2.75,0.29,0.19,0.35,0.0,0.04,0.89,0.59,2.42,0.31,0.26,0.37,0.0,0.08,0.96,0.73,2.05,0.36,0.31,0.41,0.0,0.16,1.39,0.94,2.1,0.4,0.4,0.49,0.0,0.4,1.75,1.15,2.06
114.0,2.21,0.1,0.09,0.22,0.0,0.0,0.37,0.28,2.71,0.13,0.12,0.28,0.0,0.01,0.49,0.43,2.64,0.18,0.14,0.3,0.0,0.02,0.64,0.47,2.8,0.29,0.19,0.35,0.0,0.04,0.9,0.59,2.44,0.32,0.26,0.37,0.0,0.08,0.97,0.73,2.06,0.37,0.31,0.41,0.0,0.16,1.39,0.94,2.1,0.4,0.4,0.49,0.0,0.4,1.75,1.16,2.08
115.0,2.22,0.1,0.09,0.22,0.0,0.0,0.37,0.29,2.72,0.13,0.12,0.29,0.0,0.01,0.49,0.43,2.69,0.18,0.15,0.3,0.0,0.02,0.65,0.47,2.83,0.29,0.19,0.35,0.0,0.04,0.91,0.6,2.45,0.32,0.27,0.37,0.0,0.08,0.97,0.74,2.1,0.37,0.32,0.42,0.0,0.16,1.44,0.95,2.1,0.4,0.4,0.49,0.0,0.4,1.75,1.18,2.11
116.0,2.24,0.1,0.09,0.22,0.0,0.0,0.37,0.29,2.74,0.13,0.12,0.29,0.0,0.01,0.5,0.44,2.71,0.19,0.15,0.3,0.0,0.02,0.65,0.47,2.84,0.29,0.19,0.35,0.0,0.04,0.92,0.6,2.47,0.32,0.27,0.37,0.0,0.08,0.97,0.74,2.12,0.37,0.32,0.42,0.0,0.16,1.45,0.95,2.11,0.4,0.4,0.49,0.0,0.4,1.76,1.18,2.13
117.0,2.25,0.1,0.09,0.22,0.0,0.0,0.37,0.29,2.75,0.14,0.12,0.29,0.0,0.01,0.5,0.44,2.77,0.2,0.15,0.3,0.0,0.02,0.65,0.47,2.85,0.3,0.2,0.35,0.0,0.04,0.92,0.6,2.47,0.32,0.27,0.37,0.0,0.08,0.98,0.75,2.14,0.37,0.32,0.42,0.0,0.16,1.45,0.96,2.12,0.4,0.4,0.49,0.0,0.4,1.79,1.19,2.13
118.0,2.27,0.1,0.09,0.22,0.0,0.0,0.38,0.29,2.77,0.14,0.12,0.3,0.0,0.01,0.51,0.44,2.79,0.2,0.15,0.31,0.0,0.02,0.65,0.47,2.9,0.3,0.2,0.35,0.0,0.04,0.93,0.61,2.47,0.32,0.27,0.37,0.0,0.08,0.99,0.75,2.15,0.37,0.32,0.42,0.0,0.16,1.47,0.96,2.13,0.4,0.4,0.49,0.0,0.4,1.79,1.2,2.13
119.0,2.28,0.1,0.09,0.23,0.0,0.0,0.38,0.3,2.79,0.14,0.12,0.3,0.0,0.01,0.51,0.44,2.82,0.2,0.15,0.31,0.0,0.02,0.66,0.48,2.93,0.3,0.2,0.35,0.0,0.04,0.93,0.61,2.49,0.32,0.27,0.37,0.0,0.08,0.99,0.75,2.16,0.37,0.32,0.42,0.0,0.16,1.47,0.96,2.13,0.4,0.4,0.49,0.0,0.4,1.8,1.2,2.14
120.0,2.36,0.1,0.09,0.23,0.0,0.0,0.38,0.3,2.87,0.14,0.13,0.31,0.0,0.01,0.52,0.44,2.85,0.2,0.15,0.31,0.0,0.02,0.66,0.49,2.94,0.3,0.2,0.35,0.0,0.04,0.93,0.61,2.49,0.33,0.27,0.37,0.0,0.08,1.0,0.75,2.17,0.37,0.32,0.42,0.0,0.16,1.48,0.96,2.17,0.41,0.41,0.49,0.0,0.4,1.82,1.2,2.15
121.0,2.37,0.1,0.09,0.23,0.0,0.0,0.38,0.3,2.9,0.14,0.13,0.31,0.0,0.01,0.53,0.45,2.86,0.2,0.15,0.31,0.0,0.02,0.66,0.49,2.95,0.3,0.2,0.36,0.0,0.04,0.94,0.62,2.49,0.33,0.28,0.38,0.0,0.08,1.0,0.77,2.18,0.37,0.32,0.42,0.0,0.16,1.48,0.97,2.17,0.41,0.41,0.49,0.0,0.4,1.82,1.2,2.17
122.0,2.38,0.1,0.09,0.23,0.0,0.0,0.38,0.3,2.93,0.14,0.13,0.31,0.0,0.01,0.53,0.45,2.88,0.2,0.16,0.31,0.0,0.02,0.66,0.49,2.98,0.3,0.21,0.36,0.0,0.04,0.94,0.62,2.51,0.33,0.28,0.38,0.0,0.08,1.0,0.77,2.19,0.37,0.32,0.42,0.0,0.16,1.5,0.97,2.22,0.41,0.41,0.5,0.0,0.4,1.82,1.21,2.17
123.0,2.4,0.1,0.09,0.23,0.0,0.0,0.38,0.3,2.95,0.14,0.13,0.32,0.0,0.01,0.53,0.45,2.89,0.21,0.16,0.32,0.0,0.02,0.67,0.49,2.98,0.3,0.21,0.36,0.0,0.04,0.94,0.62,2.51,0.33,0.28,0.38,0.0,0.08,1.0,0.77,2.21,0.37,0.32,0.42,0.0,0.16,1.5,0.98,2.22,0.41,0.41,0.5,0.0,0.4,1.83,1.21,2.18
124.0,2.4,0.1,0.1,0.23,0.0,0.0,0.39,0.3,2.97,0.14,0.13,0.32,0.0,0.01,0.53,0.45,2.92,0.21,0.16,0.32,0.0,0.02,0.68,0.49,2.99,0.3,0.21,0.36,0.0,0.04,0.96,0.62,2.54,0.33,0.28,0.38,0.0,0.08,1.01,0.77,2.25,0.38,0.33,0.42,0.0,0.16,1.51,0.98,2.24,0.42,0.42,0.5,0.0,0.4,1.83,1.22,2.18
125.0,2.4,0.1,0.1,0.24,0.0,0.0,0.39,0.3,2.99,0.14,0.13,0.32,0.0,0.01,0.53,0.46,2.97,0.21,0.16,0.32,0.0,0.02,0.68,0.51,3.0,0.3,0.21,0.36,0.0,0.04,0.96,0.62,2.55,0.33,0.28,0.38,0.0,0.08,1.01,0.78,2.25,0.38,0.33,0.42,0.0,0.16,1.52,0.98,2.26,0.42,0.42,0.5,0.0,0.4,1.83,1.22,2.19
126.0,2.42,0.1,0.1,0.25,0.0,0.0,0.39,0.3,3.01,0.15,0.13,0.32,0.0,0.01,0.53,0.46,2.99,0.21,0.16,0.32,0.0,0.02,0.68,0.52,3.02,0.3,0.21,0.36,0.0,0.04,0.97,0.62,2.56,0.33,0.29,0.38,0.0,0.08,1.01,0.78,2.25,0.38,0.33,0.42,0.0,0.16,1.53,0.99,2.27,0.42,0.42,0.5,0.0,0.4,1.84,1.22,2.2
127.0,2.43,0.1,0.1,0.25,0.0,0.0,0.39,0.31,3.01,0.15,0.13,0.32,0.0,0.01,0.53,0.46,2.99,0.22,0.16,0.32,0.0,0.02,0.69,0.52,3.02,0.3,0.22,0.37,0.0,0.04,0.97,0.62,2.57,0.33,0.29,0.38,0.0,0.08,1.04,0.78,2.28,0.38,0.33,0.42,0.0,0.16,1.54,0.99,2.28,0.42,0.42,0.5,0.0,0.4,1.85,1.23,2.2
128.0,2.44,0.1,0.1,0.25,0.0,0.0,0.39,0.31,3.02,0.15,0.13,0.32,0.0,0.01,0.54,0.46,3.02,0.22,0.16,0.32,0.0,0.02,0.69,0.53,3.04,0.3,0.22,0.37,0.0,0.04,0.97,0.63,2.59,0.33,0.29,0.38,0.0,0.08,1.04,0.79,2.28,0.38,0.33,0.42,0.0,0.16,1.54,0.99,2.29,0.42,0.42,0.5,0.0,0.4,1.86,1.25,2.21
129.0,2.45,0.11,0.1,0.26,0.0,0.0,0.39,0.31,3.05,0.15,0.14,0.32,0.0,0.01,0.54,0.46,3.04,0.22,0.16,0.32,0.0,0.02,0.69,0.53,3.06,0.31,0.22,0.37,0.0,0.04,0.98,0.64,2.6,0.34,0.29,0.38,0.0,0.08,1.05,0.79,2.29,0.38,0.33,0.42,0.0,0.16,1.55,1.0,2.29,0.42,0.42,0.5,0.0,0.4,1.9,1.25,2.21
130.0,2.47,0.11,0.1,0.26,0.0,0.0,0.39,0.31,3.06,0.15,0.14,0.32,0.0,0.01,0.54,0.47,3.08,0.22,0.16,0.32,0.0,0.02,0.71,0.53,3.06,0.31,0.22,0.37,0.0,0.04,0.99,0.64,2.68,0.34,0.29,0.38,0.0,0.08,1.06,0.79,2.36,0.38,0.33,0.42,0.0,0.16,1.55,1.0,2.34,0.42,0.42,0.5,0.0,0.4,1.91,1.25,2.22
131.0,2.5,0.11,0.1,0.26,0.0,0.0,0.39,0.31,3.06,0.15,0.14,0.33,0.0,0.01,0.55,0.47,3.09,0.23,0.16,0.32,0.0,0.02,0.72,0.53,3.08,0.31,0.22,0.37,0.0,0.04,0.99,0.64,2.69,0.34,0.29,0.38,0.0,0.08,1.06,0.8,2.37,0.38,0.33,0.43,0.0,0.16,1.56,1.0,2.36,0.42,0.42,0.5,0.0,0.4,1.92,1.26,2.23
132.0,2.51,0.11,0.1,0.27,0.0,0.0,0.39,0.31,3.08,0.15,0.14,0.33,0.0,0.01,0.55,0.47,3.12,0.23,0.17,0.33,0.0,0.02,0.73,0.53,3.08,0.31,0.22,0.37,0.0,0.04,1.0,0.64,2.74,0.34,0.29,0.38,0.0,0.08,1.07,0.81,2.38,0.38,0.33,0.43,0.0,0.16,1.56,1.01,2.36,0.42,0.42,0.5,0.0,0.4,1.94,1.28,2.24
133.0,2.55,0.11,0.1,0.27,0.0,0.0,0.39,0.32,3.09,0.15,0.14,0.33,0.0,0.01,0.55,0.47,3.14,0.23,0.17,0.33,0.0,0.02,0.73,0.54,3.1,0.31,0.23,0.37,0.0,0.04,1.0,0.64,2.74,0.34,0.29,0.39,0.0,0.08,1.07,0.81,2.38,0.39,0.33,0.43,0.0,0.16,1.57,1.01,2.36,0.42,0.42,0.5,0.0,0.4,1.95,1.28,2.25
134.0,2.57,0.11,0.1,0.27,0.0,0.0,0.39,0.32,3.18,0.16,0.14,0.33,0.0,0.01,0.56,0.47,3.15,0.23,0.17,0.33,0.0,0.02,0.73,0.54,3.11,0.31,0.23,0.37,0.0,0.04,1.01,0.65,2.74,0.34,0.29,0.39,0.0,0.08,1.07,0.81,2.39,0.39,0.34,0.43,0.0,0.16,1.58,1.01,2.37,0.42,0.42,0.5,0.0,0.4,1.95,1.3,2.25
135.0,2.6,0.11,0.1,0.27,0.0,0.0,0.39,0.32,3.25,0.16,0.14,0.33,0.0,0.01,0.56,0.47,3.15,0.24,0.17,0.33,0.0,0.02,0.73,0.54,3.15,0.31,0.23,0.37,0.0,0.04,1.02,0.65,2.75,0.34,0.3,0.39,0.0,0.08,1.08,0.82,2.41,0.39,0.34,0.43,0.0,0.16,1.59,1.01,2.39,0.42,0.42,0.5,0.0,0.4,1.99,1.3,2.27
136.0,2.61,0.11,0.1,0.27,0.0,0.0,0.4,0.32,3.26,0.16,0.15,0.33,0.0,0.01,0.56,0.48,3.15,0.24,0.17,0.33,0.0,0.02,0.73,0.55,3.15,0.31,0.23,0.38,0.0,0.04,1.02,0.66,2.75,0.34,0.3,0.39,0.0,0.08,1.08,0.82,2.41,0.39,0.34,0.43,0.0,0.16,1.59,1.02,2.39,0.42,0.42,0.51,0.0,0.4,2.0,1.31,2.28
137.0,2.67,0.11,0.1,0.27,0.0,0.0,0.4,0.32,3.28,0.16,0.15,0.33,0.0,0.01,0.56,0.48,3.15,0.24,0.17,0.33,0.0,0.02,0.74,0.55,3.16,0.31,0.23,0.38,0.0,0.04,1.02,0.66,2.78,0.34,0.3,0.39,0.0,0.08,1.09,0.82,2.44,0.39,0.34,0.43,0.0,0.16,1.64,1.05,2.4,0.42,0.42,0.51,0.0,0.4,2.0,1.32,2.34
138.0,2.67,0.11,0.1,0.28,0.0,0.0,0.4,0.33,3.33,0.16,0.15,0.33,0.0,0.01,0.57,0.48,3.16,0.24,0.17,0.33,0.0,0.02,0.75,0.55,3.17,0.31,0.23,0.38,0.0,0.04,1.03,0.66,2.79,0.34,0.3,0.39,0.0,0.08,1.09,0.83,2.46,0.39,0.34,0.44,0.0,0.16,1.64,1.05,2.41,0.43,0.43,0.51,0.0,0.4,2.0,1.32,2.34
139.0,2.68,0.11,0.1,0.28,0.0,0.0,0.41,0.33,3.33,0.17,0.15,0.33,0.0,0.01,0.58,0.48,3.17,0.24,0.17,0.34,0.0,0.02,0.75,0.56,3.23,0.31,0.24,0.38,0.0,0.04,1.03,0.66,2.87,0.34,0.3,0.39,0.0,0.08,1.09,0.83,2.47,0.39,0.34,0.44,0.0,0.16,1.65,1.06,2.42,0.43,0.43,0.51,0.0,0.4,2.01,1.32,2.36
140.0,2.69,0.11,0.1,0.28,0.0,0.0,0.41,0.33,3.34,0.17,0.15,0.34,0.0,0.01,0.58,0.48,3.17,0.24,0.17,0.34,0.0,0.02,0.75,0.56,3.25,0.31,0.24,0.38,0.0,0.04,1.04,0.67,2.87,0.34,0.31,0.39,0.0,0.08,1.1,0.83,2.49,0.39,0.34,0.44,0.0,0.16,1.67,1.06,2.43,0.43,0.43,0.51,0.0,0.4,2.02,1.33,2.37
141.0,2.7,0.11,0.1,0.28,0.0,0.0,0.41,0.33,3.39,0.17,0.15,0.34,0.0,0.01,0.58,0.48,3.19,0.24,0.17,0.34,0.0,0.02,0.75,0.56,3.27,0.31,0.24,0.38,0.0,0.04,1.04,0.67,2.9,0.34,0.31,0.39,0.0,0.08,1.1,0.83,2.49,0.39,0.34,0.44,0.0,0.16,1.68,1.06,2.44,0.43,0.43,0.51,0.0,0.4,2.06,1.34,2.37
142.0,2.7,0.11,0.11,0.28,0.0,0.0,0.41,0.33,3.42,0.17,0.15,0.34,0.0,0.01,0.59,0.48,3.2,0.24,0.17,0.34,0.0,0.02,0.75,0.56,3.31,0.31,0.24,0.38,0.0,0.04,1.05,0.67,2.9,0.35,0.31,0.39,0.0,0.08,1.1,0.83,2.5,0.39,0.34,0.44,0.0,0.16,1.69,1.07,2.46,0.43,0.43,0.51,0.0,0.4,2.08,1.35,2.37
143.0,2.73,0.11,0.11,0.28,0.0,0.0,0.41,0.33,3.48,0.17,0.15,0.34,0.0,0.01,0.6,0.48,3.22,0.24,0.18,0.34,0.0,0.02,0.76,0.57,3.32,0.31,0.24,0.38,0.0,0.04,1.05,0.67,2.9,0.35,0.32,0.4,0.0,0.08,1.11,0.84,2.52,0.39,0.34,0.44,0.0,0.16,1.69,1.07,2.46,0.43,0.43,0.51,0.0,0.4,2.1,1.37,2.38
144.0,2.73,0.11,0.11,0.28,0.0,0.0,0.41,0.34,3.48,0.17,0.15,0.34,0.0,0.01,0.61,0.49,3.24,0.25,0.18,0.34,0.0,0.02,0.76,0.58,3.38,0.31,0.24,0.38,0.0,0.04,1.05,0.67,2.91,0.35,0.32,0.4,0.0,0.08,1.11,0.84,2.52,0.39,0.34,0.44,0.0,0.16,1.7,1.07,2.47,0.43,0.43,0.51,0.0,0.41,2.11,1.39,2.38
145.0,2.74,0.11,0.11,0.28,0.0,0.0,0.42,0.34,3.5,0.18,0.15,0.35,0.0,0.01,0.61,0.49,3.26,0.25,0.18,0.35,0.0,0.02,0.76,0.58,3.39,0.32,0.24,0.39,0.0,0.04,1.06,0.68,2.91,0.35,0.32,0.4,0.0,0.08,1.12,0.85,2.54,0.39,0.35,0.44,0.0,0.16,1.72,1.07,2.48,0.43,0.43,0.51,0.0,0.41,2.12,1.4,2.39
146.0,2.74,0.11,0.11,0.28,0.0,0.0,0.42,0.34,3.51,0.18,0.15,0.35,0.0,0.01,0.61,0.49,3.29,0.25,0.18,0.35,0.0,0.02,0.77,0.58,3.43,0.32,0.25,0.39,0.0,0.04,1.06,0.68,2.92,0.35,0.32,0.4,0.0,0.08,1.13,0.85,2.55,0.39,0.35,0.44,0.0,0.16,1.74,1.08,2.5,0.43,0.43,0.51,0.0,0.41,2.12,1.4,2.39
147.0,2.76,0.12,0.11,0.29,0.0,0.0,0.42,0.34,3.53,0.18,0.15,0.35,0.0,0.01,0.61,0.49,3.32,0.26,0.18,0.35,0.0,0.02,0.77,0.58,3.47,0.32,0.25,0.39,0.0,0.04,1.07,0.68,2.94,0.35,0.32,0.4,0.0,0.08,1.13,0.86,2.57,0.39,0.35,0.44,0.0,0.16,1.74,1.08,2.54,0.43,0.43,0.51,0.0,0.41,2.12,1.4,2.4
148.0,2.76,0.12,0.11,0.29,0.0,0.0,0.42,0.34,3.54,0.18,0.16,0.35,0.0,0.01,0.62,0.49,3.34,0.26,0.18,0.35,0.0,0.02,0.78,0.58,3.49,0.32,0.25,0.39,0.0,0.04,1.07,0.69,2.95,0.35,0.32,0.4,0.0,0.08,1.13,0.86,2.6,0.4,0.35,0.44,0.0,0.16,1.75,1.08,2.54,0.43,0.43,0.51,0.0,0.41,2.12,1.4,2.4
149.0,2.76,0.12,0.11,0.29,0.0,0.0,0.43,0.35,3.55,0.19,0.16,0.35,0.0,0.01,0.62,0.5,3.38,0.26,0.18,0.35,0.0,0.02,0.78,0.58,3.5,0.32,0.25,0.39,0.0,0.04,1.07,0.69,2.98,0.35,0.32,0.4,0.0,0.08,1.13,0.86,2.68,0.4,0.35,0.44,0.0,0.16,1.76,1.08,2.57,0.43,0.43,0.52,0.0,0.41,2.13,1.42,2.41
150.0,2.77,0.12,0.11,0.29,0.0,0.0,0.43,0.35,3.55,0.19,0.16,0.35,0.0,0.01,0.64,0.5,3.38,0.26,0.18,0.35,0.0,0.02,0.79,0.58,3.53,0.32,0.25,0.39,0.0,0.04,1.08,0.69,3.0,0.35,0.32,0.4,0.0,0.08,1.14,0.86,2.68,0.4,0.35,0.45,0.0,0.16,1.82,1.08,2.6,0.44,0.44,0.52,0.0,0.41,2.14,1.47,2.41
151.0,2.78,0.12,0.11,0.29,0.0,0.0,0.44,0.35,3.56,0.19,0.16,0.35,0.0,0.01,0.64,0.5,3.41,0.26,0.18,0.35,0.0,0.02,0.79,0.58,3.57,0.32,0.25,0.39,0.0,0.04,1.08,0.69,3.01,0.35,0.32,0.4,0.0,0.08,1.15,0.87,2.69,0.4,0.35,0.45,0.0,0.16,1.82,1.09,2.63,0.44,0.44,0.52,0.0,0.41,2.14,1.48,2.42
152.0,2.79,0.12,0.12,0.29,0.0,0.0,0.44,0.35,3.59,0.19,0.17,0.35,0.0,0.01,0.64,0.5,3.5,0.27,0.18,0.35,0.0,0.02,0.79,0.59,3.61,0.32,0.25,0.39,0.0,0.04,1.09,0.69,3.01,0.35,0.32,0.4,0.0,0.08,1.15,0.87,2.69,0.4,0.35,0.45,0.0,0.16,1.84,1.1,2.66,0.44,0.44,0.52,0.0,0.41,2.18,1.48,2.43
153.0,2.79,0.12,0.12,0.29,0.0,0.0,0.44,0.36,3.62,0.19,0.17,0.35,0.0,0.01,0.65,0.5,3.51,0.27,0.18,0.35,0.0,0.02,0.79,0.59,3.64,0.33,0.25,0.39,0.0,0.04,1.09,0.69,3.02,0.35,0.33,0.41,0.0,0.08,1.16,0.87,2.69,0.4,0.35,0.45,0.0,0.16,1.85,1.1,2.66,0.44,0.44,0.52,0.0,0.41,2.18,1.49,2.46
154.0,2.79,0.12,0.12,0.3,0.0,0.0,0.45,0.36,3.64,0.19,0.17,0.35,0.0,0.01,0.65,0.5,3.54,0.27,0.18,0.35,0.0,0.02,0.79,0.59,3.68,0.33,0.25,0.39,0.0,0.04,1.09,0.7,3.02,0.35,0.33,0.41,0.0,0.08,1.16,0.87,2.73,0.4,0.35,0.45,0.0,0.16,1.85,1.11,2.66,0.44,0.44,0.52,0.0,0.41,2.19,1.49,2.46
155.0,2.8,0.12,0.12,0.3,0.0,0.0,0.46,0.36,3.68,0.19,0.17,0.35,0.0,0.01,0.65,0.5,3.55,0.27,0.18,0.35,0.0,0.02,0.79,0.59,3.76,0.33,0.26,0.4,0.0,0.04,1.09,0.7,3.03,0.35,0.33,0.41,0.0,0.08,1.16,0.88,2.73,0.4,0.35,0.45,0.0,0.16,1.87,1.11,2.67,0.44,0.44,0.52,0.0,0.41,2.22,1.49,2.5
156.0,2.81,0.12,0.12,0.3,0.0,0.0,0.46,0.36,3.69,0.19,0.17,0.35,0.0,0.01,0.66,0.51,3.56,0.27,0.19,0.36,0.0,0.02,0.8,0.6,3.76,0.33,0.26,0.4,0.0,0.04,1.09,0.7,3.05,0.36,0.33,0.41,0.0,0.08,1.16,0.89,2.75,0.4,0.36,0.45,0.0,0.16,1.87,1.11,2.68,0.44,0.44,0.53,0.0,0.41,2.28,1.5,2.52
157.0,2.81,0.12,0.12,0.3,0.0,0.0,0.46,0.36,3.7,0.19,0.17,0.35,0.0,0.01,0.66,0.51,3.56,0.28,0.19,0.36,0.0,0.02,0.8,0.6,3.77,0.33,0.26,0.4,0.0,0.04,1.09,0.71,3.05,0.36,0.33,0.41,0.0,0.08,1.17,0.89,2.77,0.4,0.36,0.45,0.0,0.16,1.89,1.11,2.69,0.44,0.44,0.53,0.0,0.41,2.3,1.51,2.52
158.0,2.82,0.13,0.12,0.3,0.0,0.0,0.46,0.36,3.71,0.19,0.17,0.35,0.0,0.01,0.66,0.51,3.57,0.28,0.19,0.36,0.0,0.02,0.81,0.6,3.8,0.33,0.26,0.4,0.0,0.04,1.09,0.71,3.06,0.36,0.33,0.41,0.0,0.08,1.18,0.89,2.77,0.4,0.36,0.45,0.0,0.16,1.89,1.13,2.69,0.44,0.44,0.53,0.0,0.41,2.31,1.52,2.53
159.0,2.84,0.13,0.12,0.3,0.0,0.0,0.47,0.36,3.74,0.2,0.17,0.35,0.0,0.01,0.67,0.51,3.6,0.28,0.19,0.37,0.0,0.02,0.81,0.61,3.81,0.33,0.26,0.4,0.0,0.04,1.1,0.71,3.09,0.36,0.33,0.41,0.0,0.08,1.18,0.9,2.79,0.4,0.36,0.45,0.0,0.16,1.9,1.15,2.7,0.45,0.45,0.53,0.0,0.41,2.32,1.52,2.53
160.0,2.84,0.13,0.12,0.3,0.0,0.0,0.47,0.37,3.75,0.2,0.17,0.35,0.0,0.01,0.67,0.52,3.6,0.29,0.19,0.37,0.0,0.02,0.81,0.61,3.82,0.33,0.26,0.4,0.0,0.04,1.1,0.73,3.1,0.36,0.33,0.41,0.0,0.08,1.2,0.9,2.81,0.4,0.36,0.45,0.0,0.16,1.9,1.17,2.7,0.45,0.45,0.53,0.0,0.41,2.33,1.52,2.55
161.0,2.87,0.13,0.12,0.31,0.0,0.0,0.47,0.37,3.76,0.2,0.17,0.36,0.0,0.01,0.67,0.52,3.64,0.29,0.19,0.37,0.0,0.02,0.81,0.61,3.84,0.33,0.26,0.4,0.0,0.04,1.1,0.76,3.12,0.36,0.33,0.41,0.0,0.08,1.2,0.9,2.82,0.41,0.36,0.46,0.0,0.16,1.91,1.17,2.71,0.45,0.45,0.53,0.0,0.41,2.34,1.54,2.56
162.0,2.88,0.13,0.12,0.31,0.0,0.0,0.48,0.38,3.76,0.2,0.17,0.36,0.0,0.01,0.67,0.52,3.67,0.29,0.19,0.37,0.0,0.02,0.81,0.61,3.86,0.33,0.26,0.4,0.0,0.04,1.1,0.76,3.13,0.36,0.34,0.41,0.0,0.08,1.2,0.9,2.85,0.41,0.36,0.46,0.0,0.16,1.91,1.18,2.78,0.45,0.45,0.53,0.0,0.41,2.36,1.54,2.56
163.0,2.94,0.13,0.12,0.31,0.0,0.0,0.48,0.38,3.79,0.2,0.18,0.36,0.0,0.01,0.67,0.52,3.69,0.29,0.19,0.37,0.0,0.02,0.82,0.61,3.88,0.34,0.26,0.41,0.0,0.04,1.11,0.77,3.15,0.36,0.34,0.42,0.0,0.08,1.2,0.93,2.86,0.41,0.36,0.46,0.0,0.16,1.93,1.19,2.79,0.45,0.45,0.53,0.0,0.41,2.37,1.55,2.58
164.0,2.94,0.13,0.12,0.31,0.0,0.0,0.48,0.38,3.8,0.2,0.18,0.36,0.0,0.01,0.68,0.52,3.71,0.29,0.19,0.37,0.0,0.02,0.82,0.62,3.96,0.34,0.27,0.41,0.0,0.04,1.12,0.77,3.18,0.37,0.34,0.42,0.0,0.08,1.2,0.93,2.86,0.41,0.36,0.46,0.0,0.16,1.98,1.19,2.79,0.45,0.45,0.53,0.0,0.41,2.39,1.56,2.58
165.0,2.98,0.13,0.12,0.31,0.0,0.0,0.48,0.39,3.82,0.2,0.18,0.36,0.0,0.01,0.69,0.53,3.72,0.29,0.19,0.37,0.0,0.02,0.82,0.62,3.96,0.34,0.27,0.41,0.0,0.04,1.14,0.78,3.24,0.37,0.34,0.42,0.0,0.08,1.21,0.95,2.92,0.41,0.36,0.46,0.0,0.16,2.0,1.2,2.83,0.45,0.45,0.53,0.0,0.41,2.4,1.58,2.59
166.0,2.98,0.13,0.12,0.31,0.0,0.0,0.48,0.39,3.85,0.2,0.18,0.36,0.0,0.01,0.69,0.53,3.73,0.29,0.19,0.38,0.0,0.02,0.82,0.62,4.02,0.34,0.27,0.41,0.0,0.04,1.14,0.78,3.24,0.37,0.34,0.42,0.0,0.08,1.21,0.95,2.93,0.41,0.36,0.46,0.0,0.16,2.0,1.22,2.84,0.45,0.45,0.53,0.0,0.41,2.4,1.58,2.61
167.0,2.99,0.13,0.13,0.31,0.0,0.0,0.49,0.39,3.85,0.2,0.18,0.36,0.0,0.01,0.7,0.53,3.76,0.29,0.19,0.38,0.0,0.02,0.83,0.62,4.14,0.34,0.27,0.41,0.0,0.04,1.15,0.79,3.27,0.37,0.34,0.42,0.0,0.08,1.23,0.95,2.95,0.41,0.37,0.46,0.0,0.16,2.03,1.23,2.87,0.45,0.45,0.53,0.0,0.41,2.41,1.61,2.63
168.0,3.03,0.14,0.13,0.31,0.0,0.0,0.49,0.39,3.87,0.21,0.19,0.36,0.0,0.01,0.71,0.53,3.76,0.29,0.19,0.38,0.0,0.02,0.83,0.62,4.18,0.34,0.27,0.41,0.0,0.04,1.17,0.79,3.27,0.37,0.34,0.42,0.0,0.08,1.23,0.96,2.97,0.41,0.37,0.46,0.0,0.16,2.04,1.24,2.88,0.45,0.45,0.53,0.0,0.41,2.42,1.63,2.65
169.0,3.04,0.14,0.13,0.31,0.0,0.0,0.49,0.39,3.88,0.21,0.19,0.37,0.0,0.01,0.71,0.54,3.84,0.3,0.19,0.38,0.0,0.02,0.83,0.62,4.19,0.34,0.27,0.41,0.0,0.04,1.17,0.79,3.27,0.37,0.34,0.42,0.0,0.08,1.23,0.96,3.0,0.41,0.37,0.46,0.0,0.16,2.05,1.26,2.9,0.46,0.46,0.54,0.0,0.41,2.46,1.64,2.65
170.0,3.06,0.14,0.13,0.31,0.0,0.0,0.49,0.39,3.89,0.21,0.19,0.37,0.0,0.01,0.72,0.54,3.86,0.3,0.19,0.38,0.0,0.02,0.85,0.63,4.19,0.34,0.27,0.41,0.0,0.04,1.18,0.8,3.32,0.37,0.34,0.42,0.0,0.08,1.24,0.96,3.0,0.41,0.37,0.46,0.0,0.16,2.05,1.26,2.9,0.46,0.46,0.54,0.0,0.41,2.47,1.64,2.65
171.0,3.07,0.14,0.13,0.32,0.0,0.0,0.49,0.39,3.92,0.21,0.19,0.37,0.0,0.01,0.72,0.54,3.88,0.3,0.2,0.38,0.0,0.02,0.85,0.63,4.21,0.34,0.27,0.41,0.0,0.04,1.19,0.8,3.32,0.37,0.34,0.43,0.0,0.08,1.25,0.97,3.02,0.42,0.37,0.46,0.0,0.16,2.06,1.26,2.94,0.46,0.46,0.54,0.0,0.41,2.5,1.66,2.66
172.0,3.08,0.14,0.13,0.32,0.0,0.0,0.5,0.39,3.95,0.21,0.19,0.37,0.0,0.01,0.72,0.54,3.89,0.3,0.2,0.38,0.0,0.02,0.85,0.63,4.27,0.34,0.27,0.41,0.0,0.04,1.19,0.8,3.39,0.38,0.35,0.43,0.0,0.08,1.26,0.97,3.05,0.42,0.37,0.46,0.0,0.16,2.08,1.27,2.95,0.46,0.46,0.54,0.0,0.41,2.53,1.72,2.66
173.0,3.09,0.14,0.13,0.32,0.0,0.0,0.51,0.4,3.97,0.22,0.2,0.37,0.0,0.01,0.73,0.55,3.92,0.3,0.2,0.38,0.0,0.02,0.85,0.64,4.3,0.35,0.27,0.41,0.0,0.04,1.19,0.8,3.39,0.38,0.35,0.43,0.0,0.08,1.27,0.98,3.07,0.42,0.37,0.46,0.0,0.16,2.1,1.27,2.95,0.46,0.46,0.54,0.0,0.41,2.55,1.74,2.69
174.0,3.09,0.14,0.13,0.32,0.0,0.0,0.51,0.4,4.04,0.23,0.2,0.38,0.0,0.01,0.73,0.55,3.92,0.3,0.2,0.38,0.0,0.02,0.86,0.64,4.3,0.35,0.27,0.41,0.0,0.04,1.2,0.8,3.41,0.38,0.35,0.43,0.0,0.08,1.28,0.98,3.08,0.42,0.37,0.47,0.0,0.16,2.1,1.28,2.96,0.46,0.46,0.54,0.0,0.41,2.58,1.74,2.69
175.0,3.1,0.14,0.13,0.32,0.0,0.0,0.51,0.4,4.05,0.23,0.2,0.38,0.0,0.01,0.73,0.55,3.97,0.3,0.2,0.38,0.0,0.02,0.86,0.65,4.32,0.35,0.28,0.41,0.0,0.04,1.21,0.81,3.47,0.38,0.35,0.43,0.0,0.08,1.3,0.99,3.11,0.42,0.37,0.47,0.0,0.16,2.22,1.28,2.98,0.46,0.46,0.54,0.0,0.41,2.59,1.78,2.7
176.0,3.12,0.14,0.13,0.32,0.0,0.0,0.51,0.4,4.06,0.23,0.2,0.38,0.0,0.01,0.74,0.55,4.02,0.3,0.2,0.38,0.0,0.02,0.86,0.66,4.34,0.35,0.28,0.41,0.0,0.04,1.21,0.81,3.48,0.38,0.35,0.43,0.0,0.08,1.31,0.99,3.12,0.42,0.37,0.47,0.0,0.16,2.25,1.28,3.02,0.46,0.46,0.54,0.0,0.41,2.64,1.78,2.71
177.0,3.13,0.14,0.13,0.32,0.0,0.0,0.51,0.4,4.08,0.23,0.2,0.38,0.0,0.01,0.74,0.55,4.03,0.3,0.2,0.38,0.0,0.02,0.87,0.66,4.35,0.35,0.28,0.41,0.0,0.04,1.23,0.82,3.48,0.38,0.35,0.43,0.0,0.08,1.32,1.0,3.16,0.42,0.37,0.47,0.0,0.16,2.26,1.29,3.03,0.46,0.46,0.54,0.0,0.41,2.69,1.79,2.73
178.0,3.17,0.15,0.13,0.33,0.0,0.0,0.51,0.4,4.09,0.23,0.2,0.38,0.0,0.01,0.74,0.56,4.12,0.3,0.21,0.38,0.0,0.02,0.88,0.66,4.35,0.35,0.28,0.41,0.0,0.04,1.23,0.82,3.49,0.38,0.35,0.43,0.0,0.08,1.32,1.0,3.16,0.42,0.37,0.47,0.0,0.16,2.3,1.29,3.05,0.46,0.46,0.54,0.0,0.41,2.69,1.8,2.74
179.0,3.21,0.15,0.13,0.33,0.0,0.0,0.51,0.4,4.11,0.24,0.2,0.38,0.0,0.01,0.74,0.56,4.14,0.31,0.21,0.38,0.0,0.02,0.88,0.67,4.37,0.35,0.29,0.41,0.0,0.04,1.23,0.82,3.5,0.38,0.35,0.43,0.0,0.08,1.33,1.01,3.25,0.42,0.37,0.48,0.0,0.16,2.31,1.3,3.05,0.46,0.46,0.54,0.0,0.41,2.7,1.8,2.76
180.0,3.21,0.15,0.13,0.33,0.0,0.0,0.52,0.41,4.15,0.24,0.21,0.38,0.0,0.01,0.74,0.57,4.16,0.31,0.21,0.39,0.0,0.02,0.9,0.67,4.43,0.35,0.29,0.41,0.0,0.04,1.25,0.82,3.53,0.38,0.35,0.43,0.0,0.08,1.33,1.01,3.33,0.43,0.37,0.48,0.0,0.16,2.33,1.32,3.06,0.47,0.47,0.54,0.0,0.41,2.7,1.8,2.8
181.0,3.22,0.15,0.13,0.33,0.0,0.0,0.52,0.41,4.17,0.24,0.21,0.38,0.0,0.01,0.74,0.57,4.16,0.31,0.21,0.39,0.0,0.02,0.9,0.67,4.46,0.35,0.29,0.41,0.0,0.04,1.25,0.83,3.56,0.38,0.35,0.43,0.0,0.08,1.35,1.02,3.34,0.43,0.38,0.48,0.0,0.16,2.33,1.32,3.06,0.47,0.47,0.54,0.0,0.41,2.75,1.82,2.81
182.0,3.24,0.15,0.13,0.33,0.0,0.0,0.52,0.41,4.25,0.24,0.21,0.38,0.0,0.01,0.74,0.57,4.26,0.31,0.21,0.39,0.0,0.02,0.9,0.68,4.47,0.35,0.29,0.42,0.0,0.04,1.25,0.83,3.56,0.38,0.35,0.43,0.0,0.08,1.35,1.02,3.34,0.43,0.38,0.48,0.0,0.16,2.35,1.32,3.07,0.47,0.47,0.54,0.0,0.41,2.78,1.83,2.82
183.0,3.27,0.15,0.14,0.33,0.0,0.0,0.52,0.41,4.26,0.24,0.21,0.38,0.0,0.01,0.74,0.58,4.3,0.31,0.21,0.39,0.0,0.02,0.9,0.69,4.48,0.35,0.29,0.42,0.0,0.04,1.26,0.84,3.57,0.39,0.35,0.44,0.0,0.08,1.37,1.02,3.35,0.43,0.38,0.48,0.0,0.16,2.35,1.33,3.08,0.47,0.47,0.55,0.0,0.41,2.79,1.84,2.82
184.0,3.29,0.16,0.14,0.33,0.0,0.0,0.52,0.41,4.27,0.24,0.21,0.39,0.0,0.01,0.74,0.58,4.34,0.31,0.21,0.39,0.0,0.02,0.91,0.69,4.57,0.36,0.29,0.42,0.0,0.04,1.26,0.84,3.59,0.39,0.35,0.44,0.0,0.08,1.38,1.02,3.38,0.43,0.38,0.48,0.0,0.16,2.35,1.34,3.08,0.47,0.47,0.55,0.0,0.41,2.83,1.84,2.85
185.0,3.31,0.16,0.14,0.34,0.0,0.0,0.53,0.42,4.29,0.24,0.21,0.39,0.0,0.01,0.75,0.59,4.38,0.31,0.21,0.4,0.0,0.02,0.91,0.69,4.59,0.36,0.29,0.42,0.0,0.04,1.26,0.84,3.62,0.39,0.36,0.44,0.0,0.08,1.4,1.03,3.39,0.43,0.38,0.48,0.0,0.16,2.36,1.35,3.11,0.48,0.48,0.55,0.0,0.41,2.83,1.85,2.85
186.0,3.35,0.16,0.14,0.34,0.0,0.0,0.53,0.42,4.3,0.24,0.21,0.39,0.0,0.01,0.75,0.59,4.39,0.31,0.21,0.4,0.0,0.02,0.91,0.7,4.64,0.36,0.3,0.42,0.0,0.04,1.26,0.85,3.63,0.39,0.36,0.44,0.0,0.08,1.42,1.03,3.41,0.43,0.38,0.48,0.0,0.16,2.4,1.35,3.12,0.48,0.48,0.55,0.0,0.41,2.86,1.86,2.85
187.0,3.35,0.16,0.14,0.34,0.0,0.0,0.54,0.42,4.31,0.24,0.21,0.39,0.0,0.01,0.76,0.59,4.41,0.31,0.22,0.4,0.0,0.02,0.92,0.7,4.7,0.36,0.3,0.42,0.0,0.04,1.26,0.85,3.66,0.39,0.36,0.45,0.0,0.08,1.43,1.03,3.43,0.43,0.38,0.48,0.0,0.16,2.41,1.36,3.12,0.48,0.48,0.55,0.0,0.41,2.88,1.87,2.85
188.0,3.38,0.16,0.14,0.34,0.0,0.0,0.54,0.42,4.34,0.24,0.22,0.39,0.0,0.01,0.76,0.59,4.41,0.32,0.22,0.4,0.0,0.02,0.92,0.71,4.72,0.36,0.3,0.42,0.0,0.04,1.26,0.85,3.69,0.39,0.36,0.45,0.0,0.08,1.45,1.05,3.46,0.44,0.38,0.48,0.0,0.16,2.42,1.36,3.16,0.48,0.48,0.55,0.0,0.41,2.88,1.9,2.87
189.0,3.38,0.16,0.14,0.34,0.0,0.0,0.55,0.42,4.37,0.25,0.22,0.39,0.0,0.01,0.76,0.6,4.46,0.32,0.22,0.4,0.0,0.02,0.92,0.71,4.74,0.37,0.3,0.42,0.0,0.04,1.26,0.85,3.7,0.39,0.36,0.45,0.0,0.08,1.45,1.06,3.49,0.44,0.38,0.48,0.0,0.16,2.42,1.38,3.18,0.48,0.48,0.56,0.0,0.41,2.89,1.9,2.94
190.0,3.39,0.16,0.14,0.34,0.0,0.0,0.55,0.43,4.39,0.26,0.22,0.39,0.0,0.01,0.76,0.6,4.51,0.32,0.22,0.4,0.0,0.02,0.93,0.74,4.76,0.37,0.3,0.42,0.0,0.04,1.27,0.86,3.71,0.39,0.36,0.45,0.0,0.08,1.47,1.06,3.5,0.44,0.39,0.48,0.0,0.16,2.47,1.4,3.21,0.48,0.48,0.56,0.0,0.41,2.92,1.91,2.98
191.0,3.39,0.16,0.14,0.34,0.0,0.0,0.56,0.43,4.5,0.26,0.22,0.4,0.0,0.01,0.76,0.6,4.56,0.32,0.22,0.4,0.0,0.02,0.93,0.75,4.81,0.37,0.3,0.42,0.0,0.04,1.27,0.86,3.73,0.39,0.37,0.45,0.0,0.08,1.48,1.06,3.5,0.44,0.39,0.49,0.0,0.16,2.47,1.42,3.22,0.48,0.48,0.56,0.0,0.41,3.01,1.92,2.99
192.0,3.45,0.16,0.14,0.35,0.0,0.0,0.56,0.43,4.51,0.26,0.22,0.4,0.0,0.01,0.76,0.61,4.71,0.32,0.22,0.4,0.0,0.02,0.94,0.75,4.82,0.37,0.3,0.42,0.0,0.04,1.29,0.87,3.76,0.4,0.37,0.45,0.0,0.08,1.48,1.06,3.53,0.44,0.39,0.49,0.0,0.16,2.5,1.42,3.24,0.48,0.48,0.56,0.0,0.41,3.02,1.96,2.99
193.0,3.45,0.16,0.15,0.35,0.0,0.0,0.56,0.43,4.58,0.26,0.23,0.4,0.0,0.01,0.78,0.61,4.72,0.32,0.22,0.4,0.0,0.02,0.94,0.75,4.83,0.37,0.3,0.42,0.0,0.04,1.29,0.87,3.78,0.4,0.37,0.45,0.0,0.08,1.48,1.07,3.56,0.44,0.39,0.49,0.0,0.16,2.5,1.44,3.25,0.48,0.48,0.56,0.0,0.41,3.02,1.97,3.0
194.0,3.46,0.17,0.15,0.35,0.0,0.0,0.56,0.44,4.62,0.26,0.23,0.4,0.0,0.01,0.78,0.61,4.73,0.32,0.23,0.4,0.0,0.02,0.95,0.75,4.86,0.37,0.3,0.42,0.0,0.04,1.29,0.87,3.8,0.4,0.37,0.45,0.0,0.08,1.48,1.07,3.56,0.44,0.39,0.49,0.0,0.16,2.51,1.45,3.3,0.48,0.48,0.56,0.0,0.41,3.04,1.98,3.01
195.0,3.46,0.17,0.15,0.35,0.0,0.0,0.56,0.44,4.62,0.26,0.24,0.4,0.0,0.01,0.78,0.61,4.73,0.32,0.23,0.41,0.0,0.02,0.96,0.76,4.88,0.38,0.31,0.43,0.0,0.04,1.32,0.87,3.81,0.4,0.37,0.45,0.0,0.08,1.48,1.07,3.64,0.44,0.39,0.49,0.0,0.16,2.54,1.47,3.3,0.48,0.48,0.56,0.0,0.41,3.05,2.01,3.05
196.0,3.48,0.17,0.15,0.35,0.0,0.0,0.56,0.46,4.65,0.26,0.24,0.4,0.0,0.01,0.79,0.62,4.74,0.32,0.23,0.41,0.0,0.02,0.96,0.76,4.91,0.38,0.31,0.43,0.0,0.04,1.32,0.87,3.82,0.4,0.37,0.45,0.0,0.08,1.49,1.08,3.64,0.44,0.39,0.49,0.0,0.16,2.58,1.47,3.31,0.48,0.48,0.56,0.0,0.41,3.07,2.01,3.06
197.0,3.56,0.17,0.15,0.35,0.0,0.0,0.56,0.46,4.67,0.26,0.24,0.41,0.0,0.01,0.79,0.63,4.74,0.32,0.24,0.41,0.0,0.02,0.96,0.77,4.92,0.38,0.31,0.43,0.0,0.04,1.32,0.89,3.86,0.4,0.37,0.45,0.0,0.08,1.49,1.08,3.65,0.45,0.39,0.49,0.0,0.16,2.58,1.48,3.31,0.49,0.49,0.56,0.0,0.41,3.08,2.02,3.06
198.0,3.57,0.17,0.15,0.35,0.0,0.0,0.57,0.46,4.69,0.26,0.24,0.41,0.0,0.01,0.8,0.63,4.75,0.32,0.24,0.41,0.0,0.02,0.97,0.77,4.95,0.39,0.31,0.43,0.0,0.04,1.33,0.89,3.89,0.4,0.37,0.45,0.0,0.08,1.5,1.1,3.66,0.45,0.4,0.49,0.0,0.16,2.65,1.48,3.33,0.49,0.49,0.56,0.0,0.41,3.11,2.06,3.06
199.0,3.6,0.17,0.15,0.35,0.0,0.0,0.57,0.46,4.83,0.27,0.24,0.41,0.0,0.01,0.8,0.64,4.78,0.32,0.24,0.41,0.0,0.02,0.97,0.77,4.96,0.39,0.31,0.43,0.0,0.04,1.34,0.9,3.91,0.4,0.38,0.45,0.0,0.08,1.52,1.1,3.67,0.45,0.4,0.49,0.0,0.16,2.7,1.5,3.35,0.49,0.49,0.56,0.0,0.41,3.11,2.06,3.11
200.0,3.61,0.18,0.15,0.35,0.0,0.0,0.58,0.46,4.83,0.27,0.25,0.41,0.0,0.01,0.81,0.64,4.8,0.33,0.24,0.41,0.0,0.02,0.98,0.77,4.97,0.39,0.31,0.43,0.0,0.04,1.34,0.9,3.98,0.4,0.38,0.46,0.0,0.08,1.53,1.11,3.68,0.45,0.4,0.49,0.0,0.16,2.7,1.5,3.35,0.49,0.49,0.56,0.0,0.41,3.13,2.07,3.14
201.0,3.63,0.18,0.15,0.36,0.0,0.0,0.58,0.46,4.89,0.27,0.25,0.42,0.0,0.01,0.81,0.64,4.81,0.33,0.24,0.41,0.0,0.02,0.98,0.78,4.98,0.39,0.32,0.43,0.0,0.04,1.34,0.9,4.05,0.41,0.38,0.46,0.0,0.08,1.53,1.11,3.69,0.45,0.4,0.49,0.0,0.16,2.72,1.5,3.38,0.49,0.49,0.56,0.0,0.41,3.16,2.08,3.19
202.0,3.66,0.18,0.15,0.36,0.0,0.0,0.59,0.47,4.92,0.27,0.25,0.42,0.0,0.01,0.81,0.65,4.82,0.33,0.25,0.41,0.0,0.02,0.98,0.78,4.99,0.39,0.32,0.43,0.0,0.04,1.35,0.9,4.06,0.41,0.38,0.46,0.0,0.08,1.54,1.11,3.74,0.45,0.4,0.5,0.0,0.16,2.74,1.5,3.4,0.49,0.49,0.57,0.0,0.41,3.16,2.11,3.22
203.0,3.66,0.18,0.15,0.36,0.0,0.0,0.59,0.47,4.95,0.27,0.25,0.42,0.0,0.01,0.82,0.66,4.91,0.33,0.25,0.41,0.0,0.02,0.99,0.78,5.01,0.39,0.32,0.44,0.0,0.04,1.35,0.9,4.1,0.41,0.38,0.46,0.0,0.08,1.54,1.11,3.76,0.45,0.4,0.5,0.0,0.16,2.74,1.52,3.41,0.49,0.49,0.57,0.0,0.41,3.17,2.11,3.22
204.0,3.74,0.18,0.16,0.36,0.0,0.0,0.59,0.47,4.97,0.27,0.25,0.42,0.0,0.01,0.83,0.66,5.0,0.33,0.25,0.41,0.0,0.02,1.0,0.79,5.01,0.39,0.32,0.44,0.0,0.04,1.35,0.91,4.17,0.41,0.38,0.46,0.0,0.08,1.55,1.12,3.79,0.45,0.4,0.5,0.0,0.16,2.74,1.52,3.42,0.49,0.49,0.57,0.0,0.41,3.18,2.12,3.27
205.0,3.78,0.19,0.16,0.36,0.0,0.0,0.59,0.47,4.98,0.27,0.25,0.42,0.0,0.01,0.83,0.66,5.01,0.33,0.26,0.42,0.0,0.02,1.0,0.79,5.1,0.39,0.32,0.44,0.0,0.04,1.36,0.92,4.23,0.41,0.38,0.46,0.0,0.08,1.59,1.13,3.8,0.45,0.4,0.5,0.0,0.16,2.74,1.55,3.45,0.49,0.49,0.57,0.0,0.41,3.2,2.14,3.29
206.0,3.79,0.19,0.16,0.36,0.0,0.0,0.6,0.47,4.99,0.28,0.25,0.42,0.0,0.01,0.83,0.67,5.1,0.33,0.26,0.42,0.0,0.02,1.0,0.79,5.11,0.4,0.33,0.44,0.0,0.04,1.37,0.93,4.26,0.41,0.39,0.46,0.0,0.08,1.6,1.14,3.81,0.45,0.4,0.5,0.0,0.16,2.77,1.57,3.45,0.49,0.49,0.57,0.0,0.41,3.2,2.15,3.3
207.0,3.8,0.19,0.16,0.37,0.0,0.0,0.6,0.47,5.0,0.28,0.26,0.42,0.0,0.01,0.84,0.68,5.11,0.33,0.26,0.42,0.0,0.02,1.02,0.8,5.11,0.4,0.33,0.44,0.0,0.04,1.39,0.94,4.27,0.41,0.39,0.46,0.0,0.08,1.62,1.15,3.84,0.45,0.41,0.5,0.0,0.16,2.84,1.57,3.46,0.49,0.49,0.57,0.0,0.41,3.21,2.15,3.3
208.0,3.83,0.19,0.16,0.37,0.0,0.0,0.61,0.48,5.07,0.28,0.26,0.42,0.0,0.01,0.85,0.68,5.13,0.33,0.26,0.42,0.0,0.02,1.02,0.8,5.13,0.4,0.33,0.44,0.0,0.04,1.4,0.94,4.3,0.41,0.39,0.46,0.0,0.08,1.62,1.17,3.86,0.46,0.41,0.5,0.0,0.16,2.84,1.58,3.49,0.49,0.49,0.57,0.0,0.41,3.22,2.17,3.33
209.0,3.83,0.19,0.16,0.37,0.0,0.0,0.61,0.48,5.13,0.28,0.26,0.42,0.0,0.01,0.85,0.68,5.21,0.33,0.26,0.42,0.0,0.02,1.03,0.8,5.16,0.4,0.33,0.44,0.0,0.04,1.41,0.95,4.31,0.41,0.39,0.46,0.0,0.08,1.64,1.17,3.86,0.46,0.41,0.5,0.0,0.16,2.87,1.58,3.5,0.49,0.49,0.57,0.0,0.41,3.22,2.17,3.35
210.0,3.86,0.19,0.17,0.37,0.0,0.0,0.61,0.48,5.13,0.28,0.26,0.42,0.0,0.01,0.85,0.69,5.22,0.34,0.27,0.42,0.0,0.02,1.04,0.8,5.17,0.4,0.33,0.44,0.0,0.04,1.42,0.95,4.32,0.42,0.39,0.46,0.0,0.08,1.65,1.17,3.91,0.46,0.41,0.5,0.0,0.16,2.87,1.59,3.55,0.49,0.49,0.57,0.0,0.41,3.23,2.2,3.36
211.0,3.91,0.19,0.17,0.37,0.0,0.0,0.62,0.49,5.18,0.28,0.26,0.42,0.0,0.01,0.86,0.69,5.24,0.34,0.27,0.42,0.0,0.02,1.04,0.8,5.2,0.4,0.33,0.44,0.0,0.04,1.43,0.96,4.32,0.42,0.39,0.46,0.0,0.08,1.66,1.18,3.95,0.46,0.41,0.5,0.0,0.16,2.89,1.59,3.59,0.5,0.5,0.57,0.0,0.41,3.23,2.2,3.38
212.0,3.96,0.19,0.17,0.37,0.0,0.0,0.62,0.49,5.19,0.28,0.26,0.42,0.0,0.01,0.87,0.69,5.37,0.34,0.27,0.42,0.0,0.02,1.05,0.8,5.21,0.4,0.34,0.44,0.0,0.04,1.43,0.96,4.35,0.42,0.39,0.46,0.0,0.08,1.67,1.19,3.98,0.46,0.41,0.51,0.0,0.16,2.9,1.64,3.59,0.5,0.5,0.57,0.0,0.41,3.24,2.24,3.38
213.0,3.97,0.19,0.17,0.37,0.0,0.0,0.62,0.49,5.2,0.28,0.26,0.42,0.0,0.01,0.88,0.69,5.43,0.34,0.27,0.42,0.0,0.02,1.05,0.81,5.25,0.4,0.34,0.44,0.0,0.04,1.45,0.96,4.39,0.42,0.39,0.46,0.0,0.08,1.68,1.19,3.99,0.46,0.41,0.51,0.0,0.16,2.9,1.66,3.63,0.5,0.5,0.57,0.0,0.41,3.27,2.28,3.46
214.0,3.98,0.2,0.17,0.37,0.0,0.0,0.62,0.49,5.21,0.28,0.26,0.43,0.0,0.01,0.88,0.7,5.52,0.34,0.27,0.43,0.0,0.02,1.06,0.82,5.29,0.4,0.34,0.45,0.0,0.04,1.45,0.97,4.42,0.42,0.39,0.46,0.0,0.08,1.71,1.2,4.01,0.46,0.42,0.51,0.0,0.16,2.9,1.68,3.66,0.5,0.5,0.57,0.0,0.41,3.27,2.3,3.47
215.0,3.99,0.2,0.17,0.37,0.0,0.0,0.62,0.49,5.23,0.28,0.26,0.43,0.0,0.01,0.88,0.71,5.76,0.34,0.27,0.43,0.0,0.02,1.07,0.82,5.3,0.41,0.34,0.45,0.0,0.04,1.45,0.99,4.43,0.42,0.39,0.47,0.0,0.08,1.71,1.2,4.04,0.46,0.42,0.51,0.0,0.16,2.94,1.7,3.67,0.5,0.5,0.57,0.0,0.41,3.28,2.31,3.5
216.0,4.0,0.2,0.17,0.37,0.0,0.0,0.62,0.49,5.27,0.29,0.27,0.43,0.0,0.01,0.89,0.72,5.83,0.34,0.28,0.43,0.0,0.02,1.07,0.82,5.36,0.41,0.34,0.45,0.0,0.04,1.46,0.99,4.53,0.42,0.39,0.47,0.0,0.08,1.72,1.2,4.04,0.46,0.42,0.51,0.0,0.16,2.95,1.7,3.75,0.5,0.5,0.58,0.0,0.41,3.35,2.32,3.51
217.0,4.02,0.2,0.17,0.38,0.0,0.0,0.63,0.5,5.28,0.29,0.27,0.43,0.0,0.01,0.89,0.72,5.85,0.34,0.28,0.43,0.0,0.02,1.07,0.83,5.4,0.41,0.34,0.45,0.0,0.04,1.46,1.01,4.54,0.43,0.4,0.47,0.0,0.08,1.73,1.21,4.05,0.47,0.42,0.51,0.0,0.16,2.97,1.7,3.78,0.5,0.5,0.58,0.0,0.41,3.36,2.32,3.52
218.0,4.03,0.2,0.17,0.38,0.0,0.0,0.63,0.5,5.35,0.29,0.27,0.43,0.0,0.01,0.89,0.72,5.86,0.34,0.29,0.44,0.0,0.02,1.07,0.83,5.41,0.41,0.34,0.45,0.0,0.04,1.46,1.01,4.61,0.43,0.4,0.47,0.0,0.08,1.74,1.22,4.16,0.47,0.42,0.51,0.0,0.16,2.98,1.74,3.79,0.5,0.5,0.58,0.0,0.41,3.36,2.35,3.53
219.0,4.04,0.2,0.17,0.38,0.0,0.0,0.64,0.5,5.38,0.29,0.27,0.43,0.0,0.01,0.9,0.72,5.87,0.34,0.29,0.44,0.0,0.02,1.07,0.83,5.42,0.41,0.34,0.45,0.0,0.04,1.47,1.02,4.63,0.43,0.4,0.47,0.0,0.08,1.75,1.24,4.22,0.47,0.42,0.51,0.0,0.16,2.99,1.75,3.81,0.5,0.5,0.58,0.0,0.41,3.4,2.45,3.54
220.0,4.11,0.2,0.17,0.38,0.0,0.0,0.64,0.5,5.4,0.29,0.27,0.43,0.0,0.01,0.91,0.73,5.9,0.35,0.29,0.44,0.0,0.02,1.07,0.83,5.47,0.41,0.35,0.45,0.0,0.04,1.48,1.02,4.66,0.43,0.4,0.47,0.0,0.08,1.79,1.24,4.23,0.47,0.42,0.51,0.0,0.16,3.02,1.75,3.83,0.5,0.5,0.58,0.0,0.41,3.41,2.46,3.55
221.0,4.14,0.2,0.17,0.38,0.0,0.0,0.64,0.5,5.45,0.29,0.27,0.43,0.0,0.01,0.91,0.73,5.9,0.35,0.29,0.44,0.0,0.02,1.07,0.84,5.52,0.41,0.35,0.45,0.0,0.04,1.49,1.02,4.71,0.43,0.4,0.47,0.0,0.08,1.82,1.25,4.26,0.47,0.42,0.51,0.0,0.16,3.05,1.76,3.84,0.51,0.51,0.58,0.0,0.41,3.43,2.5,3.6
222.0,4.17,0.2,0.18,0.38,0.0,0.0,0.64,0.51,5.48,0.29,0.27,0.43,0.0,0.01,0.92,0.74,5.97,0.35,0.29,0.44,0.0,0.02,1.08,0.84,5.52,0.42,0.35,0.45,0.0,0.04,1.49,1.02,4.71,0.43,0.4,0.47,0.0,0.08,1.84,1.25,4.27,0.48,0.42,0.51,0.0,0.16,3.06,1.77,3.84,0.51,0.51,0.58,0.0,0.41,3.46,2.51,3.61
223.0,4.19,0.2,0.18,0.39,0.0,0.0,0.65,0.51,5.52,0.3,0.27,0.43,0.0,0.01,0.92,0.74,6.02,0.35,0.29,0.45,0.0,0.02,1.08,0.85,5.6,0.42,0.35,0.46,0.0,0.04,1.5,1.03,4.83,0.43,0.41,0.47,0.0,0.08,1.84,1.27,4.28,0.48,0.43,0.51,0.0,0.16,3.06,1.77,3.9,0.51,0.51,0.58,0.0,0.41,3.46,2.52,3.62
224.0,4.19,0.21,0.18,0.39,0.0,0.0,0.65,0.51,5.55,0.3,0.27,0.43,0.0,0.01,0.92,0.75,6.03,0.35,0.3,0.45,0.0,0.02,1.08,0.85,5.77,0.42,0.35,0.46,0.0,0.04,1.5,1.03,4.84,0.43,0.41,0.47,0.0,0.08,1.85,1.28,4.3,0.48,0.43,0.51,0.0,0.16,3.07,1.77,3.99,0.51,0.51,0.58,0.0,0.41,3.46,2.53,3.64
225.0,4.32,0.21,0.18,0.39,0.0,0.0,0.65,0.51,5.55,0.3,0.28,0.43,0.0,0.01,0.92,0.75,6.04,0.35,0.3,0.45,0.0,0.02,1.08,0.86,5.8,0.42,0.35,0.46,0.0,0.04,1.5,1.04,4.85,0.43,0.41,0.47,0.0,0.08,1.87,1.3,4.31,0.48,0.43,0.52,0.0,0.16,3.11,1.78,4.01,0.51,0.51,0.59,0.0,0.41,3.48,2.56,3.67
226.0,4.34,0.21,0.19,0.39,0.0,0.0,0.65,0.52,5.58,0.3,0.28,0.44,0.0,0.01,0.93,0.75,6.07,0.35,0.31,0.45,0.0,0.02,1.09,0.87,5.85,0.42,0.35,0.46,0.0,0.04,1.53,1.04,4.86,0.44,0.41,0.47,0.0,0.08,1.88,1.31,4.34,0.48,0.43,0.52,0.0,0.16,3.14,1.78,4.03,0.51,0.51,0.59,0.0,0.41,3.48,2.57,3.67
227.0,4.38,0.21,0.19,0.39,0.0,0.0,0.65,0.52,5.7,0.3,0.28,0.44,0.0,0.01,0.94,0.76,6.12,0.35,0.31,0.45,0.0,0.02,1.09,0.87,5.86,0.42,0.35,0.46,0.0,0.04,1.53,1.05,4.86,0.44,0.41,0.48,0.0,0.08,1.88,1.31,4.38,0.48,0.43,0.52,0.0,0.16,3.15,1.8,4.03,0.51,0.51,0.59,0.0,0.41,3.55,2.6,3.67
228.0,4.4,0.21,0.19,0.39,0.0,0.0,0.66,0.53,5.76,0.3,0.28,0.44,0.0,0.01,0.94,0.76,6.15,0.35,0.31,0.45,0.0,0.02,1.1,0.87,5.87,0.42,0.35,0.46,0.0,0.04,1.54,1.06,4.88,0.44,0.41,0.48,0.0,0.08,1.9,1.31,4.39,0.48,0.43,0.52,0.0,0.16,3.16,1.81,4.04,0.52,0.52,0.59,0.0,0.41,3.56,2.61,3.69
229.0,4.47,0.21,0.19,0.39,0.0,0.0,0.67,0.53,5.78,0.3,0.28,0.44,0.0,0.01,0.95,0.77,6.16,0.35,0.32,0.45,0.0,0.02,1.1,0.89,5.89,0.42,0.36,0.46,0.0,0.04,1.54,1.06,4.88,0.44,0.42,0.48,0.0,0.08,1.91,1.33,4.41,0.48,0.43,0.52,0.0,0.16,3.17,1.81,4.05,0.52,0.52,0.59,0.0,0.41,3.62,2.61,3.69
230.0,4.57,0.21,0.19,0.39,0.0,0.0,0.67,0.53,5.78,0.3,0.29,0.44,0.0,0.01,0.95,0.78,6.22,0.35,0.32,0.46,0.0,0.02,1.11,0.89,5.91,0.42,0.36,0.46,0.0,0.04,1.54,1.06,4.91,0.44,0.42,0.48,0.0,0.08,1.96,1.33,4.47,0.48,0.43,0.52,0.0,0.16,3.17,1.83,4.1,0.52,0.52,0.59,0.0,0.41,3.63,2.64,3.72
231.0,4.62,0.22,0.2,0.39,0.0,0.0,0.68,0.54,5.79,0.31,0.29,0.44,0.0,0.01,0.96,0.79,6.38,0.36,0.32,0.46,0.0,0.02,1.11,0.89,5.95,0.43,0.36,0.46,0.0,0.04,1.56,1.06,5.01,0.44,0.42,0.48,0.0,0.08,1.97,1.33,4.5,0.49,0.43,0.52,0.0,0.16,3.18,1.85,4.13,0.52,0.52,0.59,0.0,0.41,3.64,2.66,3.77
232.0,4.65,0.22,0.2,0.39,0.0,0.0,0.68,0.55,5.81,0.32,0.29,0.44,0.0,0.01,0.96,0.79,6.46,0.36,0.32,0.46,0.0,0.02,1.11,0.9,5.96,0.43,0.36,0.46,0.0,0.04,1.56,1.07,5.04,0.44,0.42,0.48,0.0,0.08,2.0,1.33,4.57,0.49,0.44,0.52,0.0,0.16,3.18,1.85,4.14,0.53,0.53,0.59,0.0,0.41,3.65,2.67,3.81
233.0,4.66,0.22,0.2,0.39,0.0,0.0,0.7,0.55,5.83,0.32,0.29,0.44,0.0,0.01,0.97,0.79,6.46,0.36,0.32,0.46,0.0,0.02,1.12,0.9,6.05,0.43,0.37,0.46,0.0,0.04,1.56,1.07,5.1,0.44,0.42,0.48,0.0,0.08,2.0,1.35,4.59,0.49,0.44,0.52,0.0,0.16,3.19,1.86,4.23,0.53,0.53,0.59,0.0,0.41,3.65,2.7,3.83
234.0,4.66,0.22,0.21,0.4,0.0,0.0,0.71,0.55,5.91,0.32,0.29,0.45,0.0,0.01,0.97,0.8,6.95,0.36,0.32,0.46,0.0,0.02,1.12,0.9,6.19,0.43,0.37,0.47,0.0,0.04,1.57,1.07,5.11,0.45,0.43,0.48,0.0,0.08,2.01,1.35,4.59,0.49,0.44,0.52,0.0,0.16,3.21,1.86,4.24,0.53,0.53,0.6,0.0,0.41,3.65,2.75,3.83
235.0,4.69,0.22,0.21,0.4,0.0,0.0,0.71,0.55,5.92,0.32,0.29,0.45,0.0,0.01,0.98,0.8,6.95,0.37,0.32,0.46,0.0,0.02,1.13,0.91,6.19,0.43,0.37,0.47,0.0,0.04,1.57,1.08,5.11,0.45,0.43,0.48,0.0,0.08,2.01,1.35,4.59,0.49,0.44,0.52,0.0,0.16,3.23,1.86,4.25,0.53,0.53,0.6,0.0,0.41,3.68,2.8,3.87
236.0,4.71,0.22,0.21,0.4,0.0,0.0,0.71,0.55,5.97,0.32,0.3,0.45,0.0,0.01,0.98,0.8,6.97,0.37,0.32,0.46,0.0,0.02,1.13,0.91,6.45,0.43,0.37,0.47,0.0,0.04,1.57,1.09,5.13,0.45,0.43,0.48,0.0,0.08,2.01,1.36,4.62,0.49,0.44,0.52,0.0,0.16,3.26,1.89,4.29,0.53,0.53,0.6,0.0,0.41,3.69,2.81,3.88
237.0,4.73,0.23,0.21,0.4,0.0,0.0,0.71,0.56,6.01,0.32,0.3,0.45,0.0,0.01,0.98,0.81,7.0,0.37,0.33,0.46,0.0,0.02,1.13,0.91,6.46,0.43,0.37,0.47,0.0,0.04,1.58,1.09,5.13,0.45,0.44,0.49,0.0,0.08,2.01,1.38,4.62,0.49,0.44,0.52,0.0,0.16,3.3,1.9,4.3,0.53,0.53,0.6,0.0,0.41,3.71,2.84,3.92
238.0,4.77,0.23,0.22,0.4,0.0,0.0,0.71,0.57,6.05,0.33,0.3,0.46,0.0,0.01,1.0,0.82,7.08,0.37,0.33,0.46,0.0,0.02,1.14,0.91,6.51,0.44,0.37,0.47,0.0,0.04,1.58,1.11,5.15,0.45,0.44,0.49,0.0,0.08,2.05,1.4,4.62,0.49,0.44,0.52,0.0,0.16,3.32,1.91,4.32,0.54,0.54,0.6,0.0,0.41,3.73,2.85,3.94
239.0,4.79,0.23,0.22,0.4,0.0,0.0,0.72,0.58,6.11,0.33,0.3,0.46,0.0,0.01,1.0,0.83,7.09,0.38,0.33,0.46,0.0,0.02,1.15,0.91,6.53,0.44,0.37,0.47,0.0,0.04,1.59,1.12,5.21,0.45,0.44,0.49,0.0,0.08,2.07,1.4,4.69,0.49,0.44,0.53,0.0,0.16,3.32,1.92,4.35,0.54,0.54,0.6,0.0,0.41,3.73,2.86,3.94
240.0,4.82,0.23,0.22,0.41,0.0,0.0,0.73,0.58,6.12,0.33,0.3,0.46,0.0,0.01,1.01,0.83,7.19,0.38,0.33,0.47,0.0,0.02,1.16,0.92,6.57,0.44,0.38,0.47,0.0,0.04,1.61,1.12,5.22,0.46,0.44,0.49,0.0,0.08,2.08,1.42,4.73,0.49,0.45,0.53,0.0,0.16,3.33,1.94,4.35,0.54,0.54,0.6,0.0,0.41,3.74,2.87,3.97
241.0,4.83,0.23,0.22,0.41,0.0,0.0,0.73,0.58,6.15,0.33,0.3,0.46,0.0,0.01,1.01,0.83,7.24,0.38,0.33,0.47,0.0,0.02,1.16,0.94,6.62,0.44,0.38,0.47,0.0,0.04,1.62,1.13,5.23,0.46,0.44,0.49,0.0,0.08,2.09,1.42,4.76,0.49,0.45,0.53,0.0,0.16,3.34,1.94,4.35,0.54,0.54,0.6,0.0,0.41,3.76,2.89,3.97
242.0,4.84,0.24,0.22,0.41,0.0,0.0,0.73,0.58,6.41,0.33,0.3,0.46,0.0,0.01,1.01,0.84,7.29,0.38,0.33,0.47,0.0,0.02,1.16,0.94,6.66,0.44,0.38,0.48,0.0,0.04,1.62,1.14,5.32,0.46,0.44,0.49,0.0,0.08,2.1,1.43,4.77,0.49,0.45,0.53,0.0,0.16,3.35,1.94,4.42,0.54,0.54,0.6,0.0,0.41,3.77,2.99,3.98
243.0,4.93,0.24,0.22,0.41,0.0,0.0,0.74,0.59,6.47,0.33,0.3,0.46,0.0,0.01,1.01,0.84,7.43,0.38,0.33,0.47,0.0,0.02,1.17,0.94,6.69,0.44,0.38,0.48,0.0,0.04,1.63,1.14,5.46,0.46,0.44,0.49,0.0,0.08,2.1,1.43,4.77,0.49,0.45,0.53,0.0,0.16,3.35,1.96,4.44,0.54,0.54,0.6,0.0,0.41,3.81,3.01,4.02
244.0,5.0,0.24,0.23,0.41,0.0,0.0,0.74,0.59,6.63,0.34,0.31,0.46,0.0,0.01,1.02,0.84,7.48,0.38,0.34,0.47,0.0,0.02,1.17,0.95,6.77,0.45,0.39,0.48,0.0,0.04,1.63,1.14,5.52,0.46,0.44,0.49,0.0,0.08,2.11,1.48,4.83,0.49,0.45,0.53,0.0,0.16,3.35,1.98,4.46,0.54,0.54,0.6,0.0,0.41,3.81,3.05,4.02
245.0,5.04,0.24,0.23,0.41,0.0,0.0,0.74,0.6,6.64,0.34,0.31,0.46,0.0,0.01,1.02,0.85,7.58,0.39,0.34,0.47,0.0,0.02,1.18,0.95,6.84,0.45,0.39,0.48,0.0,0.04,1.64,1.15,5.52,0.47,0.44,0.49,0.0,0.08,2.12,1.49,4.88,0.5,0.45,0.53,0.0,0.16,3.36,1.98,4.47,0.55,0.55,0.6,0.0,0.41,3.84,3.09,4.03
246.0,5.05,0.24,0.23,0.41,0.0,0.0,0.75,0.6,6.73,0.34,0.31,0.47,0.0,0.01,1.02,0.85,7.6,0.39,0.34,0.48,0.0,0.02,1.18,0.95,6.87,0.45,0.39,0.48,0.0,0.04,1.64,1.17,5.6,0.47,0.44,0.49,0.0,0.08,2.2,1.49,4.89,0.5,0.46,0.53,0.0,0.16,3.36,1.99,4.53,0.55,0.55,0.61,0.0,0.41,3.85,3.1,4.05
247.0,5.13,0.24,0.23,0.41,0.0,0.0,0.75,0.6,6.85,0.34,0.31,0.47,0.0,0.01,1.03,0.86,7.6,0.39,0.34,0.48,0.0,0.02,1.18,0.96,6.96,0.45,0.39,0.48,0.0,0.04,1.65,1.17,5.61,0.47,0.45,0.49,0.0,0.08,2.24,1.5,4.91,0.5,0.46,0.53,0.0,0.16,3.38,2.02,4.56,0.55,0.55,0.61,0.0,0.41,3.86,3.11,4.06
248.0,5.15,0.24,0.23,0.42,0.0,0.0,0.75,0.6,6.87,0.34,0.32,0.47,0.0,0.01,1.04,0.86,7.6,0.39,0.34,0.48,0.0,0.02,1.19,0.97,6.96,0.45,0.39,0.48,0.0,0.04,1.66,1.17,5.71,0.47,0.45,0.5,0.0,0.08,2.24,1.5,4.92,0.5,0.46,0.54,0.0,0.16,3.41,2.02,4.57,0.55,0.55,0.61,0.0,0.41,3.93,3.12,4.06
249.0,5.16,0.24,0.23,0.42,0.0,0.0,0.75,0.61,6.92,0.35,0.32,0.47,0.0,0.01,1.04,0.86,7.6,0.4,0.35,0.48,0.0,0.02,1.2,0.98,6.98,0.45,0.39,0.48,0.0,0.04,1.67,1.17,5.74,0.47,0.45,0.5,0.0,0.08,2.25,1.5,4.93,0.5,0.46,0.54,0.0,0.16,3.43,2.03,4.67,0.55,0.55,0.61,0.0,0.41,3.95,3.13,4.08
250.0,5.28,0.24,0.23,0.42,0.0,0.0,0.75,0.61,6.94,0.35,0.32,0.47,0.0,0.01,1.05,0.86,7.63,0.4,0.35,0.48,0.0,0.02,1.21,1.0,6.98,0.45,0.39,0.48,0.0,0.04,1.69,1.19,5.75,0.47,0.45,0.5,0.0,0.08,2.25,1.5,5.05,0.51,0.46,0.54,0.0,0.16,3.45,2.06,4.69,0.55,0.55,0.61,0.0,0.41,3.95,3.15,4.09
251.0,5.36,0.24,0.24,0.43,0.0,0.0,0.76,0.62,6.98,0.35,0.32,0.47,0.0,0.01,1.05,0.87,7.73,0.4,0.35,0.48,0.0,0.02,1.23,1.01,6.99,0.45,0.4,0.49,0.0,0.04,1.74,1.2,5.76,0.47,0.45,0.5,0.0,0.08,2.28,1.52,5.08,0.51,0.46,0.54,0.0,0.16,3.46,2.07,4.7,0.55,0.55,0.61,0.0,0.41,3.97,3.17,4.11
252.0,5.45,0.24,0.24,0.43,0.0,0.0,0.76,0.62,7.08,0.35,0.32,0.47,0.0,0.01,1.05,0.88,8.02,0.4,0.35,0.48,0.0,0.02,1.23,1.01,7.0,0.45,0.4,0.49,0.0,0.04,1.74,1.2,5.77,0.47,0.45,0.5,0.0,0.08,2.29,1.54,5.09,0.51,0.46,0.54,0.0,0.16,3.48,2.07,4.72,0.55,0.55,0.61,0.0,0.41,3.98,3.18,4.19
253.0,5.46,0.24,0.24,0.43,0.0,0.0,0.76,0.62,7.16,0.35,0.32,0.47,0.0,0.01,1.06,0.88,8.28,0.4,0.35,0.48,0.0,0.02,1.23,1.01,7.02,0.45,0.4,0.49,0.0,0.04,1.75,1.21,5.81,0.47,0.45,0.5,0.0,0.08,2.29,1.55,5.11,0.52,0.46,0.54,0.0,0.16,3.5,2.07,4.76,0.55,0.55,0.61,0.0,0.41,4.0,3.2,4.21
254.0,5.47,0.25,0.24,0.44,0.0,0.0,0.76,0.62,7.18,0.35,0.32,0.48,0.0,0.01,1.06,0.88,8.4,0.4,0.35,0.49,0.0,0.02,1.23,1.01,7.03,0.46,0.4,0.49,0.0,0.04,1.75,1.22,5.85,0.47,0.45,0.5,0.0,0.08,2.29,1.58,5.18,0.52,0.47,0.54,0.0,0.16,3.51,2.08,4.78,0.56,0.56,0.61,0.0,0.41,4.03,3.24,4.22
255.0,5.55,0.25,0.24,0.44,0.0,0.0,0.76,0.62,7.18,0.35,0.32,0.48,0.0,0.01,1.06,0.89,8.43,0.4,0.35,0.49,0.0,0.02,1.24,1.03,7.05,0.46,0.4,0.49,0.0,0.04,1.75,1.24,5.86,0.47,0.45,0.5,0.0,0.08,2.29,1.58,5.21,0.52,0.47,0.55,0.0,0.16,3.52,2.12,4.84,0.56,0.56,0.61,0.0,0.41,4.06,3.25,4.28
256.0,5.56,0.25,0.25,0.44,0.0,0.0,0.76,0.62,7.35,0.36,0.32,0.48,0.0,0.01,1.06,0.89,8.47,0.41,0.35,0.49,0.0,0.02,1.25,1.03,7.07,0.46,0.41,0.49,0.0,0.04,1.78,1.25,5.9,0.48,0.45,0.5,0.0,0.08,2.33,1.63,5.26,0.53,0.47,0.55,0.0,0.16,3.52,2.16,4.89,0.56,0.56,0.62,0.0,0.41,4.07,3.32,4.28
257.0,5.59,0.25,0.25,0.44,0.0,0.0,0.77,0.62,7.38,0.36,0.33,0.48,0.0,0.01,1.06,0.9,8.51,0.41,0.36,0.49,0.0,0.02,1.26,1.04,7.09,0.46,0.41,0.49,0.0,0.04,1.79,1.25,5.91,0.48,0.45,0.5,0.0,0.08,2.33,1.64,5.26,0.53,0.47,0.55,0.0,0.16,3.54,2.17,4.9,0.57,0.57,0.62,0.0,0.41,4.07,3.34,4.38
258.0,5.61,0.26,0.25,0.44,0.0,0.0,0.78,0.62,7.43,0.36,0.34,0.48,0.0,0.01,1.07,0.9,8.51,0.41,0.36,0.49,0.0,0.02,1.27,1.06,7.22,0.46,0.42,0.49,0.0,0.04,1.82,1.27,5.98,0.48,0.45,0.51,0.0,0.08,2.35,1.65,5.49,0.53,0.47,0.55,0.0,0.16,3.56,2.17,4.95,0.57,0.57,0.62,0.0,0.41,4.09,3.35,4.43
259.0,5.62,0.26,0.25,0.44,0.0,0.0,0.78,0.62,7.44,0.36,0.34,0.48,0.0,0.01,1.07,0.9,8.58,0.42,0.36,0.49,0.0,0.02,1.27,1.06,7.24,0.47,0.42,0.49,0.0,0.04,1.83,1.29,6.02,0.48,0.46,0.51,0.0,0.08,2.35,1.65,5.52,0.53,0.47,0.55,0.0,0.16,3.58,2.2,5.07,0.57,0.57,0.62,0.0,0.41,4.21,3.35,4.43
260.0,5.66,0.27,0.26,0.45,0.0,0.0,0.78,0.63,7.57,0.36,0.34,0.48,0.0,0.01,1.09,0.91,8.62,0.42,0.36,0.5,0.0,0.02,1.28,1.06,7.26,0.47,0.42,0.5,0.0,0.04,1.85,1.29,6.09,0.48,0.46,0.51,0.0,0.08,2.37,1.66,5.52,0.54,0.47,0.55,0.0,0.16,3.59,2.2,5.08,0.57,0.57,0.62,0.0,0.41,4.23,3.36,4.48
261.0,5.72,0.27,0.26,0.45,0.0,0.0,0.78,0.63,7.61,0.36,0.34,0.48,0.0,0.01,1.09,0.91,8.75,0.42,0.36,0.5,0.0,0.02,1.28,1.06,7.26,0.47,0.42,0.5,0.0,0.04,1.85,1.3,6.14,0.48,0.46,0.52,0.0,0.08,2.39,1.67,5.54,0.54,0.48,0.55,0.0,0.16,3.63,2.21,5.09,0.57,0.57,0.63,0.0,0.41,4.23,3.36,4.52
262.0,5.83,0.27,0.26,0.45,0.0,0.0,0.78,0.63,7.75,0.37,0.35,0.48,0.0,0.01,1.09,0.91,8.81,0.42,0.37,0.5,0.0,0.02,1.28,1.06,7.27,0.47,0.42,0.5,0.0,0.04,1.86,1.3,6.16,0.48,0.46,0.52,0.0,0.08,2.4,1.68,5.56,0.54,0.48,0.55,0.0,0.16,3.65,2.26,5.1,0.57,0.57,0.63,0.0,0.41,4.25,3.49,4.54
263.0,5.96,0.27,0.26,0.45,0.0,0.0,0.78,0.64,7.76,0.37,0.35,0.48,0.0,0.01,1.1,0.91,9.08,0.42,0.37,0.5,0.0,0.02,1.3,1.08,7.28,0.47,0.43,0.5,0.0,0.04,1.86,1.3,6.24,0.48,0.46,0.52,0.0,0.08,2.44,1.69,5.63,0.54,0.48,0.56,0.0,0.16,3.69,2.28,5.12,0.58,0.58,0.63,0.0,0.41,4.25,3.49,4.58
264.0,6.07,0.27,0.26,0.45,0.0,0.0,0.78,0.64,7.98,0.37,0.35,0.49,0.0,0.01,1.13,0.92,9.22,0.42,0.37,0.5,0.0,0.02,1.3,1.09,7.41,0.47,0.43,0.5,0.0,0.04,1.89,1.33,6.27,0.48,0.47,0.52,0.0,0.08,2.45,1.7,5.65,0.54,0.48,0.56,0.0,0.16,3.7,2.28,5.21,0.58,0.58,0.63,0.0,0.41,4.27,3.51,4.69
265.0,6.12,0.27,0.26,0.45,0.0,0.0,0.79,0.65,8.01,0.37,0.36,0.49,0.0,0.01,1.13,0.92,9.54,0.42,0.37,0.5,0.0,0.02,1.31,1.09,7.44,0.48,0.43,0.5,0.0,0.04,1.93,1.35,6.28,0.48,0.47,0.52,0.0,0.08,2.47,1.72,5.72,0.54,0.48,0.56,0.0,0.16,3.71,2.33,5.26,0.58,0.58,0.63,0.0,0.41,4.29,3.51,4.75
266.0,6.17,0.28,0.27,0.45,0.0,0.0,0.79,0.65,8.03,0.37,0.36,0.49,0.0,0.01,1.14,0.94,9.55,0.42,0.38,0.5,0.0,0.02,1.32,1.1,7.48,0.49,0.43,0.5,0.0,0.04,1.94,1.35,6.3,0.49,0.47,0.52,0.0,0.08,2.47,1.72,5.73,0.54,0.48,0.56,0.0,0.16,3.71,2.35,5.26,0.58,0.58,0.63,0.0,0.41,4.34,3.58,4.83
267.0,6.2,0.28,0.27,0.45,0.0,0.0,0.79,0.65,8.2,0.38,0.37,0.49,0.0,0.01,1.17,0.94,9.59,0.43,0.38,0.5,0.0,0.02,1.33,1.11,7.54,0.49,0.43,0.51,0.0,0.04,1.96,1.35,6.31,0.49,0.47,0.52,0.0,0.08,2.58,1.75,5.85,0.54,0.48,0.56,0.0,0.16,3.72,2.38,5.34,0.58,0.58,0.64,0.0,0.41,4.36,3.62,4.85
268.0,6.27,0.28,0.27,0.45,0.0,0.0,0.8,0.66,8.26,0.38,0.37,0.49,0.0,0.01,1.17,0.94,10.08,0.43,0.38,0.5,0.0,0.02,1.33,1.12,7.57,0.49,0.44,0.51,0.0,0.04,1.98,1.35,6.38,0.49,0.47,0.52,0.0,0.08,2.59,1.75,5.88,0.54,0.49,0.56,0.0,0.16,3.74,2.39,5.38,0.58,0.58,0.64,0.0,0.41,4.37,3.64,4.86
269.0,6.3,0.28,0.27,0.45,0.0,0.0,0.8,0.66,8.53,0.38,0.37,0.49,0.0,0.01,1.18,0.95,10.1,0.43,0.39,0.5,0.0,0.02,1.33,1.13,7.58,0.49,0.44,0.51,0.0,0.04,2.01,1.35,6.44,0.49,0.47,0.53,0.0,0.08,2.6,1.75,5.92,0.54,0.49,0.56,0.0,0.16,3.8,2.39,5.41,0.59,0.59,0.64,0.0,0.41,4.38,3.74,4.89
270.0,6.53,0.28,0.27,0.45,0.0,0.0,0.81,0.66,8.67,0.38,0.37,0.5,0.0,0.01,1.19,0.95,10.73,0.43,0.39,0.51,0.0,0.02,1.34,1.13,7.6,0.49,0.44,0.51,0.0,0.04,2.01,1.36,6.44,0.49,0.48,0.53,0.0,0.08,2.61,1.76,5.96,0.54,0.49,0.56,0.0,0.16,3.81,2.4,5.44,0.59,0.59,0.64,0.0,0.41,4.45,3.78,4.94
271.0,6.53,0.28,0.27,0.45,0.0,0.0,0.83,0.67,8.88,0.38,0.38,0.5,0.0,0.01,1.19,0.96,10.77,0.43,0.39,0.51,0.0,0.02,1.35,1.13,7.64,0.49,0.44,0.51,0.0,0.04,2.02,1.36,6.5,0.49,0.48,0.53,0.0,0.08,2.65,1.76,5.97,0.55,0.49,0.56,0.0,0.16,3.83,2.45,5.44,0.59,0.59,0.64,0.0,0.41,4.46,3.8,4.99
272.0,6.64,0.29,0.27,0.45,0.0,0.0,0.84,0.67,8.97,0.38,0.38,0.5,0.0,0.01,1.19,0.96,10.97,0.43,0.39,0.51,0.0,0.02,1.35,1.13,7.66,0.49,0.44,0.51,0.0,0.04,2.04,1.37,6.53,0.49,0.48,0.53,0.0,0.08,2.68,1.79,6.03,0.55,0.49,0.56,0.0,0.16,3.86,2.45,5.45,0.59,0.59,0.64,0.0,0.41,4.49,3.81,5.0
273.0,6.74,0.29,0.27,0.45,0.0,0.0,0.84,0.67,8.99,0.38,0.39,0.51,0.0,0.01,1.2,0.97,11.09,0.43,0.39,0.51,0.0,0.02,1.35,1.14,7.74,0.5,0.44,0.51,0.0,0.04,2.09,1.37,6.57,0.49,0.49,0.53,0.0,0.08,2.69,1.8,6.04,0.55,0.49,0.56,0.0,0.16,3.87,2.46,5.45,0.59,0.59,0.65,0.0,0.41,4.54,3.85,5.09
274.0,6.78,0.29,0.27,0.46,0.0,0.0,0.84,0.67,9.34,0.39,0.39,0.51,0.0,0.01,1.2,0.97,11.1,0.44,0.4,0.51,0.0,0.02,1.35,1.15,7.75,0.5,0.44,0.51,0.0,0.04,2.1,1.37,6.71,0.49,0.49,0.53,0.0,0.08,2.74,1.8,6.2,0.56,0.49,0.56,0.0,0.16,3.89,2.47,5.45,0.59,0.59,0.65,0.0,0.41,4.57,3.9,5.12
275.0,6.79,0.29,0.28,0.46,0.0,0.0,0.85,0.68,9.41,0.39,0.4,0.51,0.0,0.01,1.2,0.97,11.11,0.44,0.4,0.51,0.0,0.02,1.36,1.16,7.96,0.5,0.45,0.51,0.0,0.04,2.1,1.38,6.71,0.49,0.49,0.53,0.0,0.08,2.76,1.82,6.38,0.56,0.49,0.56,0.0,0.16,3.96,2.49,5.51,0.59,0.59,0.65,0.0,0.41,4.58,3.92,5.13
276.0,6.85,0.29,0.28,0.46,0.0,0.0,0.87,0.69,9.48,0.39,0.4,0.51,0.0,0.01,1.2,0.97,11.16,0.44,0.4,0.51,0.0,0.02,1.36,1.16,8.24,0.5,0.45,0.52,0.0,0.04,2.12,1.39,6.75,0.5,0.49,0.53,0.0,0.08,2.77,1.83,6.81,0.56,0.49,0.57,0.0,0.16,3.96,2.55,5.52,0.59,0.59,0.65,0.0,0.41,4.61,3.92,5.15
277.0,6.88,0.3,0.29,0.46,0.0,0.0,0.88,0.69,9.52,0.39,0.41,0.51,0.0,0.01,1.22,0.98,11.33,0.44,0.4,0.52,0.0,0.02,1.36,1.17,8.29,0.5,0.45,0.52,0.0,0.04,2.12,1.41,6.8,0.5,0.49,0.53,0.0,0.08,2.81,1.85,6.84,0.56,0.49,0.57,0.0,0.16,3.97,2.6,5.56,0.59,0.59,0.65,0.0,0.41,4.61,3.95,5.17
278.0,7.03,0.3,0.29,0.46,0.0,0.0,0.88,0.69,9.59,0.39,0.41,0.52,0.0,0.01,1.22,0.98,11.38,0.45,0.4,0.52,0.0,0.02,1.37,1.17,8.34,0.5,0.45,0.52,0.0,0.04,2.14,1.41,6.81,0.5,0.49,0.53,0.0,0.08,2.85,1.85,6.84,0.56,0.5,0.57,0.0,0.16,4.03,2.6,5.56,0.59,0.59,0.65,0.0,0.41,4.64,3.96,5.28
279.0,7.08,0.3,0.29,0.46,0.0,0.0,0.89,0.7,9.67,0.4,0.41,0.52,0.0,0.01,1.23,0.99,11.39,0.45,0.4,0.52,0.0,0.02,1.38,1.17,8.39,0.51,0.45,0.52,0.0,0.04,2.14,1.42,6.85,0.5,0.49,0.53,0.0,0.08,2.85,1.85,6.92,0.56,0.5,0.57,0.0,0.16,4.03,2.65,5.58,0.6,0.6,0.65,0.0,0.41,4.68,3.97,5.42
280.0,7.22,0.3,0.3,0.46,0.0,0.0,0.89,0.7,9.93,0.4,0.42,0.52,0.0,0.01,1.24,1.0,11.6,0.45,0.41,0.52,0.0,0.02,1.39,1.18,8.43,0.51,0.45,0.52,0.0,0.04,2.16,1.42,6.93,0.5,0.49,0.53,0.0,0.08,2.85,1.85,7.06,0.56,0.5,0.57,0.0,0.16,4.08,2.67,5.63,0.6,0.6,0.66,0.0,0.41,4.7,3.97,5.45
281.0,7.25,0.3,0.3,0.46,0.0,0.0,0.89,0.71,9.97,0.4,0.42,0.52,0.0,0.01,1.24,1.0,11.64,0.45,0.41,0.52,0.0,0.02,1.39,1.19,8.47,0.51,0.46,0.52,0.0,0.04,2.17,1.44,6.93,0.5,0.5,0.53,0.0,0.08,2.85,1.86,7.09,0.56,0.5,0.57,0.0,0.16,4.08,2.69,5.73,0.6,0.6,0.66,0.0,0.41,4.72,3.97,5.47
282.0,7.26,0.3,0.3,0.47,0.0,0.0,0.9,0.71,10.12,0.4,0.42,0.52,0.0,0.01,1.24,1.01,11.87,0.46,0.41,0.52,0.0,0.02,1.4,1.19,8.56,0.51,0.46,0.52,0.0,0.04,2.24,1.46,7.06,0.5,0.5,0.53,0.0,0.08,2.89,1.88,7.1,0.56,0.51,0.57,0.0,0.16,4.08,2.69,5.82,0.6,0.6,0.66,0.0,0.41,4.73,4.08,5.54
283.0,7.29,0.3,0.3,0.47,0.0,0.0,0.9,0.71,10.13,0.41,0.42,0.52,0.0,0.01,1.25,1.01,11.94,0.46,0.42,0.53,0.0,0.02,1.41,1.2,8.62,0.51,0.46,0.52,0.0,0.04,2.24,1.47,7.07,0.51,0.5,0.54,0.0,0.08,2.9,1.9,7.18,0.57,0.51,0.57,0.0,0.16,4.12,2.7,5.85,0.6,0.6,0.66,0.0,0.41,4.76,4.09,5.57
284.0,7.44,0.3,0.3,0.47,0.0,0.0,0.91,0.72,10.18,0.41,0.42,0.53,0.0,0.01,1.25,1.01,12.05,0.46,0.42,0.53,0.0,0.02,1.41,1.21,8.7,0.52,0.46,0.53,0.0,0.04,2.25,1.47,7.22,0.51,0.5,0.54,0.0,0.08,2.97,1.92,7.19,0.57,0.51,0.57,0.0,0.16,4.15,2.72,5.86,0.6,0.6,0.67,0.0,0.41,4.76,4.09,5.57
285.0,7.48,0.3,0.3,0.47,0.0,0.0,0.91,0.72,10.24,0.41,0.42,0.53,0.0,0.01,1.27,1.02,12.28,0.46,0.42,0.53,0.0,0.02,1.41,1.21,8.79,0.52,0.46,0.53,0.0,0.04,2.25,1.49,7.23,0.52,0.5,0.54,0.0,0.08,2.97,1.92,7.19,0.57,0.51,0.57,0.0,0.16,4.16,2.74,5.88,0.6,0.6,0.67,0.0,0.41,4.8,4.11,5.6
286.0,7.55,0.32,0.31,0.47,0.0,0.0,0.91,0.72,10.43,0.41,0.42,0.53,0.0,0.01,1.27,1.04,12.33,0.46,0.42,0.53,0.0,0.02,1.41,1.21,9.06,0.53,0.46,0.53,0.0,0.04,2.27,1.49,7.24,0.52,0.5,0.54,0.0,0.08,3.03,1.94,7.22,0.58,0.51,0.57,0.0,0.16,4.18,2.74,6.02,0.6,0.6,0.67,0.0,0.41,4.81,4.12,5.64
287.0,7.59,0.32,0.31,0.48,0.0,0.0,0.92,0.72,10.5,0.41,0.42,0.53,0.0,0.01,1.28,1.04,12.4,0.46,0.43,0.53,0.0,0.02,1.43,1.22,9.08,0.53,0.47,0.53,0.0,0.04,2.28,1.49,7.27,0.52,0.5,0.54,0.0,0.08,3.04,1.95,7.24,0.58,0.51,0.58,0.0,0.16,4.22,2.74,6.04,0.6,0.6,0.68,0.0,0.41,4.89,4.12,5.71
288.0,7.63,0.32,0.31,0.48,0.0,0.0,0.92,0.72,10.51,0.41,0.43,0.53,0.0,0.01,1.31,1.04,12.46,0.46,0.43,0.53,0.0,0.02,1.44,1.23,9.17,0.53,0.47,0.53,0.0,0.04,2.3,1.5,7.31,0.52,0.5,0.54,0.0,0.08,3.06,1.98,7.29,0.58,0.51,0.58,0.0,0.16,4.27,2.75,6.08,0.6,0.6,0.68,0.0,0.41,4.97,4.14,5.72
289.0,7.68,0.32,0.31,0.48,0.0,0.0,0.92,0.73,10.56,0.42,0.43,0.53,0.0,0.01,1.32,1.05,12.78,0.46,0.44,0.54,0.0,0.02,1.45,1.27,9.17,0.54,0.47,0.54,0.0,0.04,2.32,1.51,7.38,0.52,0.51,0.54,0.0,0.08,3.11,1.98,7.31,0.58,0.52,0.58,0.0,0.16,4.29,2.75,6.24,0.6,0.6,0.68,0.0,0.41,4.97,4.15,5.78
290.0,7.84,0.32,0.32,0.48,0.0,0.0,0.92,0.73,10.57,0.42,0.43,0.53,0.0,0.01,1.32,1.05,13.05,0.46,0.44,0.54,0.0,0.02,1.45,1.27,9.19,0.54,0.48,0.54,0.0,0.04,2.35,1.52,7.54,0.53,0.51,0.55,0.0,0.08,3.13,2.0,7.32,0.58,0.53,0.59,0.0,0.16,4.3,2.77,6.4,0.6,0.6,0.68,0.0,0.41,5.01,4.19,5.8
291.0,7.97,0.33,0.32,0.49,0.0,0.0,0.92,0.74,10.67,0.42,0.44,0.53,0.0,0.01,1.32,1.06,13.2,0.47,0.44,0.54,0.0,0.02,1.46,1.31,9.33,0.55,0.48,0.54,0.0,0.04,2.35,1.54,8.15,0.53,0.51,0.55,0.0,0.08,3.14,2.0,7.43,0.59,0.53,0.59,0.0,0.16,4.31,2.77,6.7,0.6,0.6,0.69,0.0,0.41,5.01,4.22,5.85
292.0,7.99,0.33,0.33,0.49,0.0,0.0,0.92,0.74,10.79,0.43,0.44,0.54,0.0,0.01,1.33,1.06,13.39,0.47,0.45,0.54,0.0,0.02,1.46,1.32,9.39,0.55,0.48,0.54,0.0,0.04,2.36,1.54,8.23,0.53,0.51,0.55,0.0,0.08,3.15,2.02,7.48,0.59,0.54,0.59,0.0,0.16,4.31,2.77,6.81,0.6,0.6,0.69,0.0,0.41,5.03,4.24,5.89
293.0,8.03,0.33,0.33,0.49,0.0,0.0,0.92,0.74,10.82,0.43,0.44,0.54,0.0,0.01,1.33,1.07,13.44,0.47,0.45,0.54,0.0,0.02,1.46,1.33,9.44,0.55,0.48,0.54,0.0,0.04,2.37,1.54,8.24,0.53,0.51,0.55,0.0,0.08,3.15,2.07,7.66,0.59,0.54,0.59,0.0,0.16,4.34,2.79,6.81,0.61,0.61,0.7,0.0,0.41,5.06,4.36,5.92
294.0,8.13,0.33,0.33,0.49,0.0,0.0,0.93,0.74,10.9,0.43,0.44,0.55,0.0,0.01,1.33,1.07,13.53,0.47,0.45,0.54,0.0,0.02,1.46,1.34,9.48,0.55,0.48,0.55,0.0,0.04,2.37,1.54,8.43,0.53,0.52,0.55,0.0,0.08,3.16,2.08,7.71,0.59,0.54,0.6,0.0,0.16,4.36,2.8,6.94,0.61,0.61,0.7,0.0,0.41,5.08,4.48,6.02
295.0,8.47,0.33,0.33,0.49,0.0,0.0,0.93,0.74,10.93,0.43,0.45,0.55,0.0,0.01,1.34,1.08,13.63,0.47,0.46,0.54,0.0,0.02,1.49,1.34,9.49,0.55,0.48,0.55,0.0,0.04,2.38,1.55,8.54,0.54,0.52,0.55,0.0,0.08,3.2,2.1,7.73,0.59,0.54,0.6,0.0,0.16,4.39,2.84,7.02,0.61,0.61,0.7,0.0,0.41,5.09,4.57,6.02
296.0,8.62,0.34,0.33,0.49,0.0,0.0,0.93,0.75,10.96,0.43,0.45,0.55,0.0,0.01,1.34,1.08,13.78,0.47,0.46,0.55,0.0,0.02,1.5,1.34,9.67,0.55,0.48,0.55,0.0,0.04,2.5,1.57,8.56,0.54,0.52,0.55,0.0,0.08,3.24,2.12,7.88,0.59,0.54,0.6,0.0,0.16,4.42,2.85,7.08,0.61,0.61,0.7,0.0,0.41,5.12,4.58,6.09
297.0,8.63,0.34,0.33,0.49,0.0,0.0,0.93,0.75,11.01,0.43,0.45,0.55,0.0,0.01,1.36,1.08,14.03,0.47,0.47,0.55,0.0,0.02,1.5,1.35,9.91,0.55,0.48,0.55,0.0,0.04,2.55,1.57,8.68,0.54,0.52,0.55,0.0,0.08,3.24,2.13,7.93,0.59,0.54,0.6,0.0,0.16,4.43,2.92,7.1,0.61,0.61,0.7,0.0,0.41,5.13,4.64,6.1
298.0,8.63,0.34,0.33,0.49,0.0,0.0,0.93,0.75,11.12,0.43,0.45,0.55,0.0,0.01,1.36,1.09,14.22,0.48,0.47,0.55,0.0,0.02,1.53,1.35,9.95,0.56,0.48,0.55,0.0,0.04,2.56,1.58,9.03,0.54,0.52,0.56,0.0,0.08,3.26,2.14,8.1,0.59,0.55,0.6,0.0,0.16,4.48,2.94,7.14,0.61,0.61,0.7,0.0,0.41,5.17,4.64,6.17
299.0,8.69,0.34,0.34,0.5,0.0,0.0,0.94,0.75,11.53,0.43,0.45,0.55,0.0,0.01,1.37,1.09,14.9,0.48,0.47,0.55,0.0,0.02,1.53,1.35,9.95,0.56,0.48,0.55,0.0,0.04,2.57,1.59,9.19,0.54,0.52,0.56,0.0,0.08,3.3,2.15,8.22,0.59,0.55,0.6,0.0,0.16,4.48,2.96,7.24,0.61,0.61,0.71,0.0,0.41,5.22,4.69,6.19
300.0,8.77,0.35,0.34,0.5,0.0,0.0,0.94,0.76,11.55,0.43,0.46,0.56,0.0,0.01,1.37,1.09,15.31,0.48,0.47,0.55,0.0,0.02,1.54,1.36,10.0,0.56,0.48,0.56,0.0,0.04,2.57,1.63,9.31,0.54,0.52,0.56,0.0,0.08,3.34,2.15,8.36,0.6,0.55,0.6,0.0,0.16,4.58,2.97,7.38,0.62,0.62,0.71,0.0,0.41,5.23,4.7,6.22
301.0,8.78,0.35,0.35,0.5,0.0,0.0,0.94,0.76,11.58,0.44,0.46,0.56,0.0,0.01,1.37,1.11,15.34,0.48,0.47,0.56,0.0,0.02,1.57,1.37,10.03,0.56,0.49,0.56,0.0,0.04,2.62,1.63,9.37,0.54,0.53,0.57,0.0,0.08,3.34,2.17,8.41,0.6,0.55,0.61,0.0,0.16,4.62,3.02,7.48,0.62,0.62,0.71,0.0,0.41,5.32,4.7,6.27
302.0,8.86,0.35,0.35,0.5,0.0,0.0,0.95,0.76,11.7,0.44,0.46,0.56,0.0,0.01,1.38,1.12,15.49,0.49,0.48,0.56,0.0,0.02,1.59,1.39,10.08,0.56,0.49,0.56,0.0,0.04,2.64,1.64,9.37,0.54,0.53,0.57,0.0,0.08,3.36,2.18,9.1,0.6,0.55,0.61,0.0,0.16,4.63,3.08,7.5,0.62,0.62,0.71,0.0,0.41,5.35,4.72,6.42
303.0,8.94,0.36,0.35,0.51,0.0,0.0,0.96,0.77,11.75,0.44,0.46,0.57,0.0,0.01,1.38,1.13,16.29,0.49,0.48,0.56,0.0,0.02,1.59,1.42,10.21,0.57,0.49,0.56,0.0,0.04,2.65,1.65,9.38,0.54,0.53,0.57,0.0,0.08,3.37,2.2,9.25,0.61,0.55,0.61,0.0,0.16,4.67,3.09,7.65,0.62,0.62,0.72,0.0,0.41,5.35,4.76,6.43
304.0,8.97,0.36,0.35,0.51,0.0,0.0,0.96,0.77,12.11,0.45,0.46,0.57,0.0,0.01,1.38,1.15,16.33,0.49,0.48,0.56,0.0,0.02,1.6,1.42,10.37,0.57,0.49,0.56,0.0,0.04,2.68,1.65,9.39,0.54,0.53,0.57,0.0,0.08,3.42,2.21,9.27,0.61,0.55,0.61,0.0,0.16,4.72,3.15,7.68,0.62,0.62,0.72,0.0,0.41,5.4,4.76,6.45
305.0,9.16,0.36,0.35,0.51,0.0,0.0,0.96,0.78,12.25,0.45,0.46,0.57,0.0,0.01,1.39,1.17,16.34,0.5,0.48,0.56,0.0,0.02,1.61,1.44,10.38,0.57,0.5,0.56,0.0,0.04,2.71,1.69,9.44,0.55,0.54,0.58,0.0,0.08,3.46,2.22,9.36,0.61,0.56,0.61,0.0,0.16,4.77,3.16,7.74,0.63,0.63,0.72,0.0,0.41,5.44,4.78,6.53
306.0,9.45,0.37,0.36,0.51,0.0,0.0,0.96,0.78,12.79,0.45,0.47,0.57,0.0,0.01,1.39,1.18,16.39,0.5,0.48,0.56,0.0,0.02,1.63,1.45,10.51,0.57,0.5,0.56,0.0,0.04,2.74,1.69,9.57,0.55,0.54,0.58,0.0,0.08,3.53,2.24,9.37,0.61,0.56,0.62,0.0,0.16,4.81,3.24,7.75,0.63,0.63,0.72,0.0,0.41,5.44,4.8,6.67
307.0,9.65,0.37,0.36,0.51,0.0,0.0,0.97,0.78,13.04,0.45,0.47,0.58,0.0,0.01,1.4,1.19,16.41,0.51,0.48,0.56,0.0,0.02,1.66,1.45,10.53,0.57,0.5,0.56,0.0,0.04,2.74,1.72,9.63,0.56,0.54,0.58,0.0,0.08,3.54,2.26,9.42,0.61,0.56,0.62,0.0,0.16,4.82,3.24,7.96,0.63,0.63,0.72,0.0,0.41,5.5,4.81,6.78
308.0,10.12,0.37,0.36,0.51,0.0,0.0,0.98,0.78,13.18,0.45,0.47,0.58,0.0,0.01,1.41,1.22,16.54,0.51,0.48,0.56,0.0,0.02,1.67,1.46,10.7,0.57,0.5,0.57,0.0,0.04,2.76,1.74,9.87,0.56,0.54,0.58,0.0,0.08,3.63,2.29,9.44,0.61,0.56,0.62,0.0,0.16,4.86,3.25,8.17,0.63,0.63,0.72,0.0,0.41,5.54,4.83,6.78
309.0,10.19,0.37,0.36,0.51,0.0,0.0,0.99,0.79,13.23,0.46,0.47,0.58,0.0,0.01,1.41,1.22,16.57,0.52,0.48,0.57,0.0,0.02,1.71,1.48,10.77,0.58,0.5,0.57,0.0,0.04,2.77,1.75,9.87,0.56,0.54,0.58,0.0,0.08,3.64,2.36,9.46,0.61,0.56,0.62,0.0,0.16,4.91,3.25,8.35,0.64,0.64,0.73,0.0,0.41,5.78,4.89,7.01
310.0,10.52,0.37,0.37,0.51,0.0,0.0,0.99,0.79,13.63,0.46,0.47,0.58,0.0,0.01,1.41,1.24,16.73,0.52,0.49,0.58,0.0,0.02,1.75,1.49,11.03,0.58,0.5,0.57,0.0,0.04,2.81,1.77,9.91,0.56,0.54,0.58,0.0,0.08,3.74,2.39,9.57,0.61,0.56,0.62,0.0,0.16,4.95,3.29,8.38,0.64,0.64,0.73,0.0,0.41,5.82,4.9,7.03
311.0,10.64,0.38,0.37,0.52,0.0,0.0,1.0,0.79,14.3,0.46,0.47,0.58,0.0,0.01,1.43,1.24,16.89,0.52,0.49,0.58,0.0,0.02,1.78,1.49,11.11,0.59,0.5,0.57,0.0,0.04,2.81,1.8,10.7,0.57,0.55,0.58,0.0,0.08,3.79,2.41,9.76,0.61,0.56,0.62,0.0,0.16,5.01,3.3,8.45,0.64,0.64,0.73,0.0,0.41,5.85,4.92,7.07
312.0,10.84,0.38,0.38,0.52,0.0,0.0,1.01,0.79,14.51,0.46,0.47,0.59,0.0,0.01,1.43,1.25,17.02,0.52,0.49,0.58,0.0,0.02,1.8,1.5,11.38,0.59,0.5,0.58,0.0,0.04,2.81,1.8,10.95,0.57,0.55,0.58,0.0,0.08,3.8,2.41,9.88,0.61,0.56,0.62,0.0,0.16,5.02,3.32,8.67,0.64,0.64,0.73,0.0,0.41,5.86,4.96,7.18
313.0,10.96,0.38,0.38,0.52,0.0,0.0,1.02,0.79,14.65,0.46,0.48,0.59,0.0,0.01,1.46,1.26,17.47,0.53,0.49,0.58,0.0,0.02,1.82,1.51,11.52,0.59,0.5,0.58,0.0,0.04,2.85,1.82,11.04,0.57,0.55,0.59,0.0,0.08,3.82,2.42,9.97,0.62,0.56,0.62,0.0,0.16,5.05,3.39,8.73,0.65,0.65,0.73,0.0,0.41,5.89,4.96,7.22
314.0,11.16,0.38,0.39,0.52,0.0,0.0,1.02,0.79,14.7,0.47,0.48,0.59,0.0,0.01,1.46,1.26,17.6,0.53,0.49,0.58,0.0,0.02,1.83,1.51,11.71,0.6,0.5,0.58,0.0,0.04,2.85,1.82,11.11,0.57,0.55,0.59,0.0,0.08,3.83,2.44,9.99,0.62,0.56,0.63,0.0,0.16,5.06,3.39,8.81,0.65,0.65,0.74,0.0,0.41,5.98,5.03,7.23
315.0,11.24,0.38,0.39,0.52,0.0,0.0,1.03,0.8,14.77,0.47,0.49,0.59,0.0,0.01,1.47,1.27,17.64,0.54,0.5,0.58,0.0,0.02,1.83,1.51,12.0,0.6,0.5,0.59,0.0,0.04,2.85,1.88,11.52,0.58,0.56,0.59,0.0,0.08,3.85,2.45,10.41,0.62,0.57,0.63,0.0,0.16,5.08,3.47,8.98,0.65,0.65,0.74,0.0,0.41,6.02,5.04,7.24
316.0,11.27,0.39,0.4,0.52,0.0,0.0,1.05,0.8,14.99,0.47,0.49,0.59,0.0,0.01,1.49,1.28,17.77,0.54,0.5,0.59,0.0,0.02,1.84,1.52,12.19,0.6,0.5,0.59,0.0,0.04,2.86,1.9,11.75,0.58,0.56,0.59,0.0,0.08,3.93,2.46,10.42,0.62,0.57,0.63,0.0,0.16,5.08,3.52,9.04,0.65,0.65,0.75,0.0,0.41,6.05,5.24,7.33
317.0,11.32,0.39,0.4,0.52,0.0,0.0,1.06,0.8,15.13,0.48,0.49,0.59,0.0,0.01,1.5,1.29,18.83,0.54,0.5,0.59,0.0,0.02,1.85,1.52,12.41,0.6,0.5,0.59,0.0,0.04,2.88,1.92,11.77,0.58,0.56,0.59,0.0,0.08,3.96,2.47,10.59,0.62,0.57,0.64,0.0,0.16,5.09,3.54,9.17,0.65,0.65,0.75,0.0,0.41,6.05,5.24,7.36
318.0,11.5,0.39,0.4,0.52,0.0,0.0,1.06,0.8,15.34,0.48,0.49,0.6,0.0,0.01,1.5,1.3,19.06,0.54,0.5,0.59,0.0,0.02,1.85,1.53,12.69,0.6,0.51,0.59,0.0,0.04,2.88,1.97,11.91,0.58,0.56,0.59,0.0,0.08,3.99,2.49,10.76,0.63,0.57,0.64,0.0,0.16,5.1,3.58,9.25,0.65,0.65,0.75,0.0,0.41,6.1,5.29,7.38
319.0,11.64,0.39,0.4,0.52,0.0,0.0,1.07,0.81,16.39,0.48,0.49,0.6,0.0,0.01,1.52,1.32,19.15,0.55,0.5,0.59,0.0,0.02,1.87,1.6,13.21,0.61,0.52,0.59,0.0,0.04,2.93,1.97,12.17,0.58,0.57,0.59,0.0,0.08,4.01,2.52,10.82,0.63,0.57,0.64,0.0,0.16,5.15,3.59,9.25,0.65,0.65,0.75,0.0,0.41,6.22,5.31,7.93
320.0,12.35,0.39,0.4,0.52,0.0,0.0,1.07,0.84,16.98,0.49,0.49,0.6,0.0,0.01,1.53,1.33,19.75,0.55,0.5,0.59,0.0,0.02,1.89,1.61,13.41,0.61,0.52,0.6,0.0,0.04,2.93,1.97,12.53,0.58,0.57,0.59,0.0,0.08,4.04,2.56,10.91,0.64,0.57,0.64,0.0,0.16,5.22,3.66,9.28,0.65,0.65,0.75,0.0,0.41,6.31,5.37,8.18
321.0,12.36,0.4,0.41,0.53,0.0,0.0,1.07,0.84,17.11,0.49,0.5,0.6,0.0,0.01,1.55,1.36,20.44,0.56,0.5,0.6,0.0,0.02,1.91,1.61,13.48,0.61,0.52,0.6,0.0,0.04,2.96,1.97,13.08,0.58,0.57,0.59,0.0,0.08,4.09,2.59,10.95,0.64,0.57,0.64,0.0,0.16,5.25,3.77,9.4,0.65,0.65,0.75,0.0,0.41,6.31,5.43,8.18
322.0,12.82,0.4,0.41,0.53,0.0,0.0,1.07,0.86,18.1,0.5,0.5,0.6,0.0,0.01,1.59,1.37,21.53,0.56,0.51,0.6,0.0,0.02,1.93,1.63,14.03,0.61,0.52,0.6,0.0,0.04,3.01,2.0,13.26,0.58,0.57,0.59,0.0,0.08,4.18,2.6,11.03,0.64,0.58,0.65,0.0,0.16,5.49,3.78,9.52,0.66,0.66,0.75,0.0,0.41,6.32,5.46,8.23
323.0,12.9,0.4,0.42,0.53,0.0,0.0,1.07,0.86,18.16,0.5,0.5,0.6,0.0,0.01,1.59,1.39,21.74,0.57,0.51,0.6,0.0,0.02,1.93,1.66,14.06,0.61,0.52,0.6,0.0,0.04,3.04,2.0,13.27,0.58,0.58,0.6,0.0,0.08,4.19,2.61,11.16,0.65,0.59,0.65,0.0,0.16,5.5,3.82,9.71,0.66,0.66,0.75,0.0,0.41,6.33,5.48,8.47
324.0,13.62,0.4,0.42,0.53,0.0,0.0,1.1,0.86,20.51,0.51,0.5,0.61,0.0,0.01,1.61,1.39,23.33,0.57,0.51,0.61,0.0,0.02,1.94,1.67,14.38,0.62,0.52,0.61,0.0,0.04,3.05,2.02,13.42,0.59,0.58,0.6,0.0,0.08,4.19,2.62,11.24,0.65,0.59,0.65,0.0,0.16,5.54,3.84,9.97,0.66,0.66,0.76,0.0,0.41,6.46,5.49,8.64
325.0,13.81,0.41,0.42,0.53,0.0,0.0,1.1,0.88,21.13,0.51,0.5,0.61,0.0,0.01,1.62,1.39,23.43,0.57,0.51,0.61,0.0,0.02,1.96,1.68,15.2,0.63,0.53,0.61,0.0,0.04,3.06,2.06,13.42,0.59,0.58,0.6,0.0,0.08,4.19,2.65,11.24,0.65,0.59,0.66,0.0,0.16,5.56,3.84,10.09,0.66,0.66,0.76,0.0,0.41,6.47,5.51,8.7
326.0,14.42,0.42,0.42,0.53,0.0,0.0,1.12,0.89,21.44,0.51,0.5,0.61,0.0,0.01,1.65,1.4,23.44,0.57,0.52,0.61,0.0,0.02,1.97,1.69,15.46,0.63,0.53,0.61,0.0,0.04,3.13,2.07,13.77,0.59,0.58,0.6,0.0,0.08,4.25,2.67,11.4,0.66,0.59,0.66,0.0,0.16,5.63,3.85,10.18,0.67,0.67,0.76,0.0,0.41,6.53,5.54,8.85
327.0,14.68,0.42,0.42,0.53,0.0,0.0,1.12,0.89,21.57,0.51,0.5,0.61,0.0,0.01,1.66,1.41,24.01,0.57,0.52,0.61,0.0,0.02,2.03,1.7,15.75,0.63,0.53,0.61,0.0,0.04,3.15,2.15,13.82,0.59,0.58,0.61,0.0,0.08,4.26,2.72,11.44,0.66,0.59,0.66,0.0,0.16,5.65,3.93,10.3,0.67,0.67,0.76,0.0,0.41,6.63,5.58,9.06
328.0,15.12,0.42,0.42,0.53,0.0,0.0,1.13,0.9,22.85,0.52,0.51,0.61,0.0,0.01,1.69,1.42,24.96,0.58,0.52,0.61,0.0,0.02,2.04,1.73,16.16,0.64,0.53,0.61,0.0,0.04,3.16,2.15,13.96,0.59,0.59,0.61,0.0,0.08,4.29,2.72,11.57,0.66,0.59,0.66,0.0,0.16,5.72,3.94,10.42,0.67,0.67,0.77,0.0,0.41,6.7,5.58,9.1
329.0,15.45,0.42,0.43,0.54,0.0,0.0,1.13,0.91,22.91,0.52,0.51,0.61,0.0,0.01,1.69,1.43,25.68,0.58,0.52,0.61,0.0,0.02,2.07,1.75,16.51,0.64,0.53,0.62,0.0,0.04,3.21,2.18,14.0,0.59,0.59,0.61,0.0,0.08,4.3,2.75,11.7,0.66,0.6,0.66,0.0,0.16,5.76,3.96,10.82,0.68,0.68,0.77,0.0,0.41,6.73,5.59,9.11
330.0,15.74,0.42,0.43,0.54,0.0,0.0,1.14,0.93,23.43,0.53,0.51,0.61,0.0,0.01,1.71,1.46,25.8,0.58,0.52,0.61,0.0,0.02,2.1,1.76,16.73,0.64,0.54,0.62,0.0,0.04,3.35,2.18,14.12,0.6,0.6,0.61,0.0,0.08,4.39,2.78,11.7,0.66,0.6,0.66,0.0,0.16,5.82,3.97,11.2,0.68,0.68,0.77,0.0,0.41,6.8,5.61,9.17
331.0,16.09,0.42,0.44,0.54,0.0,0.0,1.14,0.93,23.49,0.54,0.51,0.62,0.0,0.01,1.74,1.47,26.16,0.58,0.53,0.61,0.0,0.02,2.1,1.77,16.82,0.64,0.54,0.62,0.0,0.04,3.38,2.19,14.18,0.6,0.6,0.61,0.0,0.08,4.4,2.8,11.77,0.66,0.6,0.66,0.0,0.16,5.86,3.97,11.24,0.68,0.68,0.77,0.0,0.41,6.82,5.69,9.19
332.0,16.54,0.42,0.44,0.54,0.0,0.0,1.15,0.93,24.17,0.54,0.51,0.62,0.0,0.01,1.77,1.52,26.85,0.59,0.53,0.61,0.0,0.02,2.12,1.77,17.26,0.65,0.54,0.62,0.0,0.04,3.42,2.2,14.52,0.61,0.6,0.61,0.0,0.08,4.47,2.82,11.81,0.67,0.6,0.67,0.0,0.16,5.88,3.99,11.33,0.69,0.69,0.77,0.0,0.41,6.9,5.72,9.23
333.0,16.72,0.43,0.44,0.55,0.0,0.0,1.16,0.94,24.31,0.54,0.51,0.62,0.0,0.01,1.79,1.52,28.32,0.59,0.53,0.61,0.0,0.02,2.16,1.78,17.88,0.65,0.54,0.62,0.0,0.04,3.44,2.23,14.65,0.61,0.6,0.63,0.0,0.08,4.48,2.88,12.38,0.67,0.6,0.67,0.0,0.16,5.95,4.01,11.33,0.69,0.69,0.77,0.0,0.41,6.99,5.74,9.24
334.0,17.11,0.43,0.44,0.55,0.0,0.0,1.17,0.94,24.33,0.54,0.52,0.62,0.0,0.01,1.82,1.54,29.64,0.6,0.54,0.61,0.0,0.02,2.18,1.82,18.69,0.65,0.54,0.62,0.0,0.04,3.57,2.24,14.66,0.61,0.61,0.63,0.0,0.08,4.49,2.91,12.71,0.67,0.6,0.67,0.0,0.16,5.97,4.06,11.4,0.69,0.69,0.77,0.0,0.41,7.21,5.81,9.45
335.0,17.11,0.43,0.44,0.55,0.0,0.0,1.17,0.94,24.47,0.54,0.52,0.62,0.0,0.01,1.82,1.54,29.81,0.6,0.54,0.61,0.0,0.02,2.19,1.83,19.33,0.65,0.55,0.63,0.0,0.04,3.58,2.24,15.11,0.61,0.61,0.63,0.0,0.08,4.5,2.96,12.84,0.67,0.61,0.67,0.0,0.16,5.98,4.08,11.48,0.69,0.69,0.78,0.0,0.41,7.25,5.99,9.68
336.0,17.35,0.43,0.45,0.56,0.0,0.0,1.17,0.95,24.51,0.55,0.53,0.62,0.0,0.01,1.86,1.56,30.09,0.6,0.54,0.61,0.0,0.02,2.21,1.83,19.84,0.66,0.55,0.63,0.0,0.04,3.64,2.26,15.34,0.61,0.61,0.63,0.0,0.08,4.57,2.96,13.07,0.67,0.61,0.67,0.0,0.16,6.01,4.2,11.53,0.7,0.7,0.78,0.0,0.41,7.29,6.02,10.34
337.0,17.43,0.43,0.45,0.56,0.0,0.0,1.17,0.95,24.73,0.55,0.54,0.63,0.0,0.01,1.86,1.56,30.2,0.6,0.54,0.62,0.0,0.02,2.26,1.84,20.99,0.66,0.55,0.63,0.0,0.04,3.72,2.35,15.37,0.62,0.61,0.63,0.0,0.08,4.57,2.96,13.08,0.68,0.61,0.68,0.0,0.16,6.07,4.22,11.7,0.7,0.7,0.78,0.0,0.41,7.32,6.03,10.35
338.0,17.54,0.44,0.45,0.56,0.0,0.0,1.18,0.96,26.03,0.55,0.55,0.63,0.0,0.01,1.87,1.58,30.74,0.61,0.55,0.62,0.0,0.02,2.31,1.86,21.23,0.66,0.55,0.63,0.0,0.04,3.79,2.41,15.4,0.62,0.62,0.63,0.0,0.08,4.62,3.02,13.26,0.68,0.62,0.68,0.0,0.16,6.15,4.56,11.7,0.7,0.7,0.78,0.0,0.41,7.33,6.17,10.46
339.0,17.93,0.45,0.45,0.57,0.0,0.0,1.18,0.97,26.33,0.55,0.55,0.63,0.0,0.01,1.88,1.6,31.13,0.61,0.55,0.62,0.0,0.02,2.32,1.9,21.34,0.66,0.55,0.63,0.0,0.04,3.82,2.42,15.75,0.62,0.62,0.64,0.0,0.08,4.65,3.03,13.27,0.69,0.62,0.68,0.0,0.16,6.2,4.61,11.92,0.7,0.7,0.78,0.0,0.41,7.35,6.19,10.52
340.0,18.61,0.45,0.45,0.58,0.0,0.0,1.19,0.97,26.55,0.55,0.55,0.64,0.0,0.01,1.9,1.61,31.29,0.61,0.55,0.62,0.0,0.02,2.34,1.91,21.52,0.66,0.56,0.63,0.0,0.04,3.93,2.44,15.79,0.62,0.62,0.64,0.0,0.08,4.66,3.06,13.33,0.69,0.62,0.68,0.0,0.16,6.21,4.62,12.69,0.7,0.7,0.79,0.0,0.41,7.37,6.2,10.68
341.0,18.96,0.45,0.45,0.58,0.0,0.0,1.19,0.98,29.19,0.56,0.56,0.64,0.0,0.01,1.91,1.62,32.0,0.61,0.55,0.62,0.0,0.02,2.37,1.91,21.91,0.66,0.56,0.63,0.0,0.04,3.99,2.46,16.05,0.62,0.62,0.64,0.0,0.08,4.7,3.09,13.38,0.69,0.62,0.68,0.0,0.16,6.22,4.63,12.72,0.7,0.7,0.79,0.0,0.41,7.38,6.28,10.92
342.0,19.44,0.46,0.45,0.58,0.0,0.0,1.21,1.0,29.72,0.56,0.57,0.64,0.0,0.01,1.93,1.62,32.35,0.62,0.56,0.62,0.0,0.02,2.38,1.91,22.57,0.67,0.56,0.63,0.0,0.04,4.07,2.47,16.15,0.63,0.62,0.64,0.0,0.08,4.72,3.1,13.42,0.7,0.63,0.68,0.0,0.16,6.23,4.64,13.38,0.7,0.7,0.8,0.0,0.41,7.4,6.32,11.07
343.0,20.25,0.46,0.47,0.58,0.0,0.0,1.21,1.0,30.2,0.56,0.57,0.64,0.0,0.01,2.02,1.63,32.42,0.63,0.56,0.62,0.0,0.02,2.5,1.92,23.4,0.67,0.56,0.64,0.0,0.04,4.13,2.47,16.16,0.63,0.63,0.64,0.0,0.08,4.78,3.14,13.42,0.7,0.63,0.69,0.0,0.16,6.27,4.65,13.39,0.7,0.7,0.8,0.0,0.41,7.41,6.4,11.33
344.0,20.29,0.46,0.47,0.59,0.0,0.0,1.22,1.01,30.66,0.56,0.57,0.64,0.0,0.01,2.05,1.64,35.2,0.64,0.56,0.62,0.0,0.02,2.51,1.92,23.43,0.68,0.57,0.64,0.0,0.04,4.15,2.5,16.27,0.64,0.64,0.65,0.0,0.08,4.82,3.22,13.53,0.7,0.63,0.69,0.0,0.16,6.48,4.66,13.7,0.71,0.71,0.8,0.0,0.41,7.44,6.45,11.53
345.0,22.1,0.46,0.47,0.59,0.0,0.0,1.23,1.01,30.87,0.56,0.57,0.64,0.0,0.01,2.05,1.67,35.39,0.64,0.57,0.62,0.0,0.02,2.55,1.94,24.32,0.68,0.57,0.64,0.0,0.04,4.19,2.5,16.6,0.64,0.64,0.65,0.0,0.08,4.89,3.24,13.77,0.7,0.63,0.7,0.0,0.16,6.62,4.68,14.56,0.71,0.71,0.8,0.0,0.41,7.52,6.46,11.63
346.0,22.45,0.46,0.48,0.59,0.0,0.0,1.24,1.02,30.96,0.57,0.57,0.64,0.0,0.01,2.08,1.68,35.6,0.64,0.57,0.62,0.0,0.02,2.68,1.96,24.37,0.68,0.57,0.64,0.0,0.04,4.2,2.5,17.87,0.64,0.64,0.65,0.0,0.08,4.9,3.27,14.16,0.71,0.64,0.7,0.0,0.16,6.64,4.7,15.4,0.71,0.71,0.8,0.0,0.41,7.54,6.49,11.76
347.0,22.66,0.47,0.48,0.59,0.0,0.0,1.25,1.02,31.69,0.58,0.58,0.64,0.0,0.01,2.09,1.69,35.85,0.65,0.57,0.62,0.0,0.02,2.72,1.96,25.01,0.68,0.57,0.64,0.0,0.04,4.22,2.54,19.19,0.65,0.65,0.65,0.0,0.08,4.91,3.27,14.16,0.71,0.64,0.7,0.0,0.16,6.73,4.76,15.58,0.72,0.72,0.8,0.0,0.41,7.59,6.65,11.77
348.0,23.27,0.47,0.48,0.6,0.0,0.0,1.27,1.02,33.07,0.58,0.58,0.64,0.0,0.01,2.13,1.7,35.87,0.65,0.57,0.62,0.0,0.02,2.73,1.97,26.04,0.69,0.57,0.65,0.0,0.04,4.24,2.56,19.28,0.65,0.65,0.66,0.0,0.08,4.95,3.29,14.19,0.71,0.64,0.71,0.0,0.16,6.81,4.84,16.01,0.72,0.72,0.8,0.0,0.41,7.63,6.7,11.8
349.0,23.84,0.48,0.49,0.6,0.0,0.0,1.28,1.03,33.65,0.58,0.58,0.64,0.0,0.01,2.17,1.74,36.6,0.65,0.58,0.63,0.0,0.02,2.73,1.98,27.12,0.69,0.57,0.65,0.0,0.04,4.25,2.57,20.37,0.65,0.65,0.66,0.0,0.08,4.96,3.32,14.2,0.72,0.64,0.71,0.0,0.16,6.89,4.89,16.31,0.72,0.72,0.8,0.0,0.41,7.65,6.93,12.22
350.0,23.93,0.49,0.49,0.6,0.0,0.0,1.28,1.04,33.66,0.58,0.58,0.64,0.0,0.01,2.19,1.77,38.26,0.65,0.59,0.63,0.0,0.02,2.73,2.0,27.74,0.7,0.58,0.65,0.0,0.04,4.29,2.59,20.77,0.65,0.65,0.67,0.0,0.08,5.04,3.52,14.59,0.72,0.64,0.71,0.0,0.16,6.99,4.97,16.52,0.72,0.72,0.81,0.0,0.41,7.81,6.94,12.48
351.0,24.08,0.5,0.49,0.6,0.0,0.0,1.29,1.05,34.03,0.58,0.58,0.65,0.0,0.01,2.2,1.81,38.29,0.66,0.59,0.63,0.0,0.02,2.74,2.01,28.61,0.7,0.58,0.65,0.0,0.04,4.36,2.61,21.36,0.65,0.66,0.67,0.0,0.08,5.05,3.67,14.76,0.73,0.64,0.71,0.0,0.16,7.04,5.01,16.71,0.72,0.72,0.81,0.0,0.41,7.86,6.99,13.2
352.0,24.31,0.5,0.5,0.6,0.0,0.0,1.33,1.05,34.08,0.59,0.58,0.65,0.0,0.01,2.29,1.82,38.56,0.67,0.6,0.63,0.0,0.02,2.74,2.06,28.84,0.71,0.58,0.65,0.0,0.04,4.36,2.65,22.27,0.66,0.67,0.68,0.0,0.08,5.05,3.75,15.37,0.73,0.64,0.71,0.0,0.16,7.06,5.06,16.77,0.72,0.72,0.81,0.0,0.41,7.93,7.0,13.55
353.0,24.39,0.5,0.5,0.6,0.0,0.0,1.34,1.06,34.98,0.6,0.59,0.66,0.0,0.01,2.32,1.82,38.76,0.67,0.6,0.63,0.0,0.02,2.76,2.09,28.92,0.71,0.58,0.65,0.0,0.04,4.42,2.73,22.97,0.66,0.67,0.68,0.0,0.08,5.07,3.78,15.57,0.73,0.64,0.71,0.0,0.16,7.08,5.28,16.81,0.73,0.73,0.82,0.0,0.41,8.0,7.27,13.84
354.0,25.36,0.5,0.5,0.61,0.0,0.0,1.34,1.08,37.15,0.61,0.59,0.66,0.0,0.01,2.33,1.84,38.86,0.67,0.61,0.63,0.0,0.02,2.84,2.15,30.57,0.73,0.58,0.65,0.0,0.04,4.43,2.8,23.77,0.66,0.67,0.69,0.0,0.08,5.08,3.84,15.57,0.73,0.65,0.72,0.0,0.16,7.1,5.28,17.17,0.73,0.73,0.82,0.0,0.41,8.08,7.29,14.06
355.0,25.67,0.5,0.51,0.61,0.0,0.0,1.36,1.08,38.55,0.61,0.59,0.66,0.0,0.01,2.36,1.85,38.9,0.68,0.61,0.64,0.0,0.02,2.85,2.19,30.76,0.73,0.59,0.65,0.0,0.04,4.57,2.82,25.05,0.67,0.67,0.69,0.0,0.08,5.14,3.85,15.69,0.74,0.65,0.72,0.0,0.16,7.11,5.33,17.5,0.73,0.73,0.82,0.0,0.41,8.23,7.44,15.27
356.0,26.3,0.51,0.51,0.61,0.0,0.0,1.38,1.09,38.71,0.61,0.59,0.66,0.0,0.01,2.46,1.88,39.52,0.68,0.61,0.64,0.0,0.02,2.93,2.2,32.25,0.74,0.59,0.65,0.0,0.04,4.6,2.86,25.7,0.67,0.68,0.69,0.0,0.08,5.15,3.86,16.31,0.74,0.65,0.72,0.0,0.16,7.12,5.5,17.53,0.73,0.73,0.82,0.0,0.41,8.29,7.62,15.37
357.0,26.35,0.51,0.51,0.62,0.0,0.0,1.4,1.1,39.4,0.61,0.59,0.66,0.0,0.01,2.47,1.93,41.64,0.68,0.61,0.64,0.0,0.02,2.94,2.33,33.0,0.74,0.59,0.66,0.0,0.04,4.6,2.97,26.0,0.67,0.68,0.7,0.0,0.08,5.28,3.88,16.52,0.74,0.66,0.72,0.0,0.16,7.19,5.54,17.61,0.73,0.73,0.83,0.0,0.41,8.35,7.62,15.66
358.0,28.97,0.51,0.52,0.62,0.0,0.0,1.41,1.1,39.44,0.62,0.59,0.66,0.0,0.01,2.54,1.96,42.58,0.69,0.62,0.64,0.0,0.02,2.98,2.45,33.51,0.74,0.6,0.66,0.0,0.04,4.62,2.97,26.1,0.67,0.68,0.7,0.0,0.08,5.45,3.9,16.66,0.74,0.66,0.72,0.0,0.16,7.4,5.61,17.62,0.74,0.74,0.83,0.0,0.41,8.39,7.65,15.9
359.0,29.01,0.51,0.52,0.62,0.0,0.0,1.43,1.1,39.62,0.62,0.59,0.66,0.0,0.01,2.62,1.98,43.27,0.69,0.63,0.64,0.0,0.02,3.0,2.47,34.14,0.74,0.6,0.66,0.0,0.04,4.62,2.99,26.43,0.68,0.69,0.7,0.0,0.08,5.45,4.27,16.71,0.74,0.66,0.73,0.0,0.16,7.43,5.66,17.65,0.74,0.74,0.83,0.0,0.41,8.8,7.77,16.24
360.0,29.65,0.52,0.52,0.63,0.0,0.0,1.46,1.11,40.41,0.62,0.59,0.66,0.0,0.01,2.66,2.06,43.92,0.7,0.63,0.64,0.0,0.02,3.09,2.47,34.22,0.75,0.6,0.67,0.0,0.04,4.78,3.06,26.7,0.68,0.7,0.71,0.0,0.08,5.46,4.3,16.93,0.74,0.66,0.73,0.0,0.16,7.44,5.88,17.96,0.74,0.74,0.83,0.0,0.41,8.83,7.8,16.31
361.0,30.08,0.52,0.52,0.63,0.0,0.0,1.47,1.12,40.62,0.62,0.59,0.66,0.0,0.01,2.7,2.06,43.98,0.7,0.63,0.64,0.0,0.02,3.1,2.54,34.47,0.76,0.6,0.67,0.0,0.04,4.87,3.06,27.46,0.68,0.7,0.71,0.0,0.08,5.48,4.34,16.98,0.75,0.66,0.73,0.0,0.17,7.54,5.88,18.78,0.75,0.75,0.83,0.0,0.41,8.87,7.83,16.39
362.0,30.12,0.52,0.53,0.63,0.0,0.0,1.47,1.16,41.34,0.62,0.59,0.67,0.0,0.01,2.71,2.07,44.5,0.71,0.63,0.64,0.0,0.02,3.11,2.55,34.91,0.77,0.61,0.67,0.0,0.04,4.91,3.09,27.82,0.68,0.7,0.71,0.0,0.08,5.52,4.52,17.02,0.75,0.66,0.73,0.0,0.17,7.56,6.17,19.17,0.76,0.76,0.84,0.0,0.41,9.2,8.04,16.64
363.0,30.28,0.52,0.53,0.63,0.0,0.0,1.5,1.16,41.65,0.63,0.59,0.67,0.0,0.01,2.71,2.08,44.5,0.71,0.63,0.64,0.0,0.02,3.12,2.61,36.31,0.78,0.61,0.67,0.0,0.04,5.09,3.11,28.84,0.69,0.71,0.71,0.0,0.08,5.53,4.54,17.62,0.75,0.66,0.74,0.0,0.17,7.64,6.24,19.25,0.76,0.76,0.84,0.0,0.41,9.23,8.1,17.63
364.0,32.28,0.52,0.53,0.63,0.0,0.0,1.55,1.16,41.7,0.66,0.6,0.67,0.0,0.01,2.75,2.08,45.15,0.72,0.64,0.64,0.0,0.02,3.15,2.64,36.59,0.78,0.61,0.68,0.0,0.04,5.11,3.32,28.85,0.7,0.71,0.72,0.0,0.08,5.59,4.56,18.32,0.75,0.67,0.74,0.0,0.17,7.65,6.42,20.26,0.76,0.76,0.84,0.0,0.41,9.27,8.19,18.05
365.0,32.9,0.53,0.53,0.64,0.0,0.0,1.56,1.17,41.88,0.66,0.6,0.67,0.0,0.01,2.8,2.11,45.24,0.72,0.64,0.64,0.0,0.02,3.23,2.65,36.94,0.78,0.61,0.68,0.0,0.04,5.12,3.33,28.92,0.7,0.71,0.72,0.0,0.08,5.74,4.57,19.09,0.76,0.67,0.74,0.0,0.17,7.88,6.67,20.38,0.76,0.76,0.84,0.0,0.41,9.3,8.24,18.5
366.0,33.42,0.53,0.54,0.64,0.0,0.0,1.56,1.17,42.93,0.66,0.6,0.68,0.0,0.01,2.84,2.13,45.62,0.73,0.64,0.65,0.0,0.02,3.42,2.65,37.15,0.78,0.61,0.68,0.0,0.04,5.28,3.41,29.67,0.7,0.71,0.73,0.0,0.08,5.88,4.58,19.19,0.76,0.67,0.74,0.0,0.17,7.89,6.71,20.7,0.76,0.76,0.85,0.0,0.41,9.35,8.26,18.5
367.0,33.51,0.54,0.54,0.64,0.0,0.0,1.57,1.17,45.01,0.66,0.6,0.68,0.0,0.01,2.88,2.14,46.11,0.74,0.65,0.65,0.0,0.02,3.47,2.73,37.47,0.79,0.62,0.68,0.0,0.04,5.31,3.71,29.7,0.71,0.71,0.73,0.0,0.08,5.88,4.66,19.37,0.76,0.67,0.74,0.0,0.17,7.97,6.76,20.84,0.76,0.76,0.85,0.0,0.41,9.4,8.27,18.54
368.0,34.62,0.54,0.55,0.64,0.0,0.0,1.6,1.18,46.27,0.66,0.61,0.68,0.0,0.01,2.89,2.15,46.26,0.74,0.65,0.65,0.0,0.02,3.52,2.77,37.97,0.79,0.62,0.68,0.0,0.04,5.44,3.72,30.53,0.71,0.72,0.73,0.0,0.08,6.02,4.75,19.72,0.76,0.67,0.75,0.0,0.17,8.07,6.84,21.17,0.77,0.77,0.86,0.0,0.41,9.43,8.28,18.76
369.0,35.45,0.54,0.56,0.65,0.0,0.0,1.61,1.18,46.59,0.67,0.61,0.68,0.0,0.01,2.9,2.16,46.29,0.74,0.66,0.65,0.0,0.02,3.67,2.82,38.56,0.8,0.62,0.68,0.0,0.04,5.45,3.73,30.61,0.72,0.73,0.73,0.0,0.08,6.36,4.77,20.41,0.77,0.67,0.75,0.0,0.17,8.1,7.02,21.39,0.77,0.77,0.86,0.0,0.41,9.43,8.43,18.81
370.0,35.51,0.55,0.56,0.65,0.0,0.0,1.63,1.19,47.25,0.68,0.62,0.68,0.0,0.01,3.07,2.18,46.99,0.75,0.67,0.65,0.0,0.02,3.69,2.82,38.99,0.81,0.62,0.68,0.0,0.04,5.46,3.76,30.71,0.72,0.73,0.73,0.0,0.08,6.64,4.89,21.13,0.77,0.68,0.75,0.0,0.17,8.13,7.15,21.57,0.77,0.77,0.87,0.0,0.41,9.87,8.45,19.22
371.0,35.68,0.55,0.56,0.65,0.0,0.0,1.65,1.19,47.61,0.7,0.62,0.68,0.0,0.01,3.11,2.26,48.23,0.77,0.67,0.66,0.0,0.02,3.79,2.84,39.4,0.82,0.63,0.68,0.0,0.04,5.48,3.77,30.75,0.73,0.74,0.73,0.0,0.08,6.74,4.97,22.65,0.77,0.69,0.75,0.0,0.17,8.23,7.34,21.64,0.77,0.77,0.88,0.0,0.41,9.95,8.65,19.58
372.0,36.47,0.55,0.56,0.65,0.0,0.0,1.66,1.19,47.69,0.7,0.63,0.68,0.0,0.01,3.14,2.28,48.56,0.78,0.67,0.66,0.0,0.02,3.84,2.86,39.55,0.82,0.64,0.69,0.0,0.04,5.52,3.82,30.77,0.73,0.74,0.73,0.0,0.08,6.76,5.09,22.94,0.78,0.69,0.75,0.0,0.17,8.25,7.5,21.69,0.77,0.77,0.89,0.0,0.41,10.44,8.92,20.07
373.0,36.6,0.56,0.56,0.67,0.0,0.0,1.67,1.2,48.22,0.71,0.63,0.68,0.0,0.01,3.15,2.29,50.53,0.79,0.67,0.67,0.0,0.02,3.96,2.92,39.59,0.83,0.64,0.69,0.0,0.04,5.55,4.02,33.12,0.74,0.74,0.74,0.0,0.08,7.17,5.28,22.97,0.78,0.69,0.75,0.0,0.17,8.58,7.66,22.44,0.77,0.77,0.89,0.0,0.41,10.78,9.32,21.44
374.0,36.81,0.57,0.57,0.67,0.0,0.0,1.69,1.21,48.5,0.71,0.63,0.69,0.0,0.01,3.27,2.35,50.74,0.79,0.67,0.67,0.0,0.02,4.11,2.94,39.71,0.83,0.65,0.69,0.0,0.04,5.65,4.06,33.7,0.74,0.74,0.74,0.0,0.08,7.51,5.28,23.56,0.79,0.69,0.76,0.0,0.17,8.77,7.74,22.94,0.77,0.77,0.9,0.0,0.41,10.84,9.37,21.66
375.0,37.58,0.57,0.57,0.67,0.0,0.0,1.71,1.21,49.29,0.71,0.63,0.7,0.0,0.01,3.36,2.41,50.92,0.79,0.67,0.67,0.0,0.02,4.12,3.07,40.94,0.83,0.66,0.7,0.0,0.04,5.81,4.27,34.53,0.75,0.75,0.74,0.0,0.08,7.56,5.28,24.44,0.8,0.72,0.76,0.0,0.17,8.84,8.06,22.97,0.77,0.77,0.9,0.0,0.41,10.87,9.73,21.81
376.0,38.4,0.57,0.57,0.68,0.0,0.0,1.72,1.22,51.02,0.71,0.63,0.7,0.0,0.01,3.39,2.45,51.29,0.79,0.69,0.67,0.0,0.02,4.14,3.11,42.67,0.83,0.67,0.7,0.0,0.04,5.91,4.34,34.97,0.75,0.76,0.74,0.0,0.08,7.67,5.32,24.65,0.8,0.73,0.76,0.0,0.17,8.88,8.1,23.56,0.78,0.78,0.9,0.0,0.41,10.95,9.86,22.09
377.0,38.6,0.57,0.57,0.68,0.0,0.0,1.72,1.22,51.36,0.73,0.64,0.71,0.0,0.01,3.41,2.48,51.55,0.81,0.7,0.68,0.0,0.02,4.36,3.24,43.79,0.83,0.69,0.7,0.0,0.04,5.97,4.34,36.31,0.75,0.76,0.75,0.0,0.08,7.72,5.5,25.87,0.81,0.73,0.76,0.0,0.17,9.39,8.12,23.99,0.79,0.79,0.91,0.0,0.41,11.17,10.08,22.72
378.0,38.99,0.57,0.57,0.68,0.0,0.0,1.73,1.23,51.77,0.73,0.64,0.71,0.0,0.01,3.42,2.49,52.69,0.82,0.7,0.68,0.0,0.02,4.57,3.27,44.33,0.84,0.69,0.7,0.0,0.04,6.08,4.57,36.4,0.77,0.76,0.75,0.0,0.08,7.78,5.57,26.11,0.81,0.74,0.77,0.0,0.17,9.71,8.3,24.15,0.79,0.79,0.91,0.0,0.41,11.26,10.13,23.95
379.0,39.27,0.58,0.58,0.7,0.0,0.0,1.74,1.23,52.89,0.73,0.64,0.71,0.0,0.01,3.47,2.51,52.96,0.83,0.7,0.68,0.0,0.02,4.6,3.34,45.35,0.84,0.7,0.71,0.0,0.04,6.26,4.73,36.42,0.77,0.77,0.76,0.0,0.08,8.1,5.78,26.73,0.82,0.74,0.77,0.0,0.17,10.1,8.66,24.62,0.8,0.8,0.91,0.0,0.41,11.26,10.14,24.22
380.0,39.37,0.59,0.58,0.71,0.0,0.0,1.75,1.25,53.93,0.74,0.64,0.72,0.0,0.01,3.52,2.53,53.0,0.84,0.71,0.68,0.0,0.02,4.6,3.48,46.11,0.84,0.71,0.71,0.0,0.04,6.33,4.78,37.04,0.77,0.78,0.76,0.0,0.08,8.23,6.0,28.32,0.82,0.75,0.77,0.0,0.17,10.61,8.99,24.72,0.8,0.8,0.92,0.0,0.41,11.92,10.25,24.69
381.0,40.41,0.59,0.58,0.71,0.0,0.0,1.75,1.25,53.98,0.75,0.65,0.72,0.0,0.01,3.6,2.56,54.82,0.84,0.71,0.69,0.0,0.02,4.91,3.87,46.64,0.84,0.71,0.71,0.0,0.04,6.5,4.89,38.19,0.78,0.78,0.76,0.0,0.08,8.41,6.23,28.33,0.82,0.75,0.77,0.0,0.17,10.78,9.12,25.11,0.8,0.8,0.92,0.0,0.41,11.97,10.48,25.86
382.0,41.56,0.59,0.59,0.72,0.0,0.0,1.82,1.27,54.6,0.75,0.65,0.73,0.0,0.01,3.76,2.58,55.05,0.84,0.71,0.69,0.0,0.02,5.1,3.9,47.3,0.85,0.71,0.72,0.0,0.04,6.58,5.04,38.2,0.78,0.78,0.76,0.0,0.08,8.97,6.46,29.18,0.82,0.75,0.79,0.0,0.17,10.97,9.23,25.35,0.8,0.8,0.92,0.0,0.41,12.36,10.68,26.02
383.0,41.62,0.59,0.59,0.72,0.0,0.0,1.83,1.28,57.03,0.76,0.65,0.73,0.0,0.01,3.88,2.6,56.16,0.85,0.71,0.7,0.0,0.02,5.21,3.97,49.94,0.86,0.72,0.72,0.0,0.04,6.64,5.14,38.58,0.78,0.78,0.76,0.0,0.08,9.0,6.71,29.67,0.82,0.75,0.79,0.0,0.17,11.09,9.41,26.16,0.81,0.81,0.92,0.0,0.41,12.66,10.9,26.36
384.0,44.25,0.59,0.6,0.72,0.0,0.0,1.87,1.3,57.31,0.76,0.65,0.73,0.0,0.01,3.94,2.65,57.84,0.85,0.71,0.7,0.0,0.02,5.69,4.14,51.55,0.86,0.72,0.73,0.0,0.04,6.74,5.16,39.55,0.78,0.79,0.76,0.0,0.08,9.02,6.72,30.13,0.83,0.76,0.79,0.0,0.17,11.13,9.45,26.3,0.81,0.81,0.93,0.0,0.41,12.85,11.09,26.49
385.0,44.7,0.6,0.6,0.72,0.0,0.0,1.87,1.31,57.57,0.76,0.65,0.73,0.0,0.01,4.07,2.66,58.65,0.85,0.72,0.7,0.0,0.02,5.91,4.19,52.52,0.86,0.73,0.74,0.0,0.04,6.76,5.28,39.6,0.79,0.79,0.76,0.0,0.08,9.17,6.76,30.22,0.84,0.77,0.8,0.0,0.17,11.15,9.7,26.86,0.81,0.81,0.94,0.0,0.41,13.49,11.4,26.61
386.0,44.87,0.61,0.62,0.73,0.0,0.0,1.87,1.31,57.78,0.76,0.66,0.73,0.0,0.01,4.13,2.68,60.89,0.87,0.72,0.7,0.0,0.02,5.98,4.26,52.86,0.87,0.73,0.75,0.0,0.04,6.87,5.54,39.62,0.79,0.79,0.76,0.0,0.08,9.52,6.84,31.0,0.84,0.78,0.8,0.0,0.17,11.28,9.73,27.8,0.82,0.82,0.95,0.0,0.41,13.72,12.15,27.15
387.0,45.37,0.61,0.62,0.73,0.0,0.0,1.91,1.31,58.75,0.76,0.66,0.74,0.0,0.01,4.13,2.77,68.95,0.87,0.73,0.7,0.0,0.02,6.5,4.27,53.44,0.91,0.73,0.75,0.0,0.04,6.96,5.56,41.19,0.8,0.79,0.77,0.0,0.08,9.65,6.9,31.03,0.84,0.78,0.8,0.0,0.17,11.59,10.11,28.66,0.82,0.82,0.95,0.0,0.41,15.03,12.48,27.18
388.0,46.17,0.61,0.63,0.73,0.0,0.0,1.91,1.33,58.8,0.78,0.66,0.74,0.0,0.01,4.33,2.82,69.54,0.88,0.73,0.71,0.0,0.02,6.58,4.31,56.57,0.92,0.74,0.76,0.0,0.04,7.18,5.78,41.47,0.8,0.8,0.77,0.0,0.08,9.77,7.06,31.07,0.85,0.79,0.81,0.0,0.17,12.01,10.24,28.9,0.82,0.82,0.96,0.0,0.41,15.15,12.75,27.67
389.0,46.43,0.61,0.63,0.73,0.0,0.0,1.96,1.33,59.49,0.78,0.67,0.74,0.0,0.01,4.39,2.83,71.54,0.88,0.73,0.71,0.0,0.02,6.71,4.7,57.4,0.92,0.74,0.76,0.0,0.04,7.7,6.18,41.54,0.81,0.81,0.78,0.0,0.08,10.02,7.07,32.56,0.85,0.79,0.81,0.0,0.17,12.63,10.25,30.14,0.83,0.83,0.97,0.0,0.41,15.3,13.11,29.41
390.0,47.14,0.61,0.64,0.75,0.0,0.0,2.01,1.35,60.49,0.79,0.67,0.75,0.0,0.01,4.62,2.83,73.05,0.88,0.73,0.71,0.0,0.02,6.72,4.92,57.65,0.93,0.75,0.76,0.0,0.04,7.72,6.46,42.31,0.81,0.81,0.78,0.0,0.08,10.77,7.2,33.21,0.85,0.79,0.81,0.0,0.17,12.67,10.29,30.83,0.83,0.83,0.98,0.0,0.41,15.35,13.27,29.62
391.0,48.75,0.61,0.65,0.75,0.0,0.0,2.12,1.41,61.15,0.79,0.68,0.76,0.0,0.01,4.63,2.85,75.29,0.88,0.73,0.71,0.0,0.02,6.76,5.04,58.99,0.93,0.75,0.77,0.0,0.04,8.01,6.72,43.08,0.81,0.81,0.78,0.0,0.08,11.15,7.83,33.78,0.86,0.79,0.81,0.0,0.17,14.35,10.43,31.41,0.83,0.83,0.98,0.0,0.41,15.73,13.3,29.94
392.0,48.8,0.62,0.66,0.75,0.0,0.0,2.18,1.43,63.72,0.8,0.68,0.76,0.0,0.01,4.81,2.87,76.31,0.89,0.73,0.72,0.0,0.02,6.92,5.16,59.23,0.94,0.75,0.77,0.0,0.04,8.05,6.95,43.22,0.82,0.82,0.78,0.0,0.08,11.49,7.86,34.02,0.86,0.8,0.81,0.0,0.17,16.51,10.6,32.62,0.83,0.83,0.99,0.0,0.41,16.04,13.78,30.22
393.0,51.45,0.62,0.66,0.75,0.0,0.0,2.19,1.44,66.34,0.8,0.68,0.77,0.0,0.01,5.01,2.9,76.62,0.9,0.74,0.72,0.0,0.02,6.94,5.53,60.44,0.97,0.76,0.79,0.0,0.04,8.44,7.0,43.79,0.83,0.83,0.79,0.0,0.08,11.59,8.66,34.7,0.87,0.8,0.81,0.0,0.17,16.68,10.78,32.74,0.83,0.83,0.99,0.0,0.41,16.53,14.06,30.51
394.0,52.21,0.62,0.66,0.76,0.0,0.0,2.21,1.44,66.59,0.8,0.69,0.77,0.0,0.01,5.09,2.99,78.75,0.9,0.75,0.72,0.0,0.02,7.72,5.69,61.75,0.99,0.76,0.79,0.0,0.04,8.84,7.06,44.39,0.85,0.83,0.79,0.0,0.08,11.75,9.19,35.13,0.87,0.81,0.81,0.0,0.17,16.83,10.93,33.05,0.83,0.83,1.0,0.0,0.41,16.74,14.82,30.63
395.0,52.55,0.63,0.67,0.77,0.0,0.0,2.21,1.46,66.7,0.82,0.69,0.77,0.0,0.01,5.35,3.07,79.15,0.92,0.76,0.74,0.0,0.02,7.97,5.72,62.3,1.01,0.77,0.79,0.0,0.04,9.0,7.33,45.29,0.86,0.83,0.8,0.0,0.08,11.78,9.23,35.39,0.88,0.81,0.81,0.0,0.17,16.84,11.25,33.51,0.84,0.84,1.0,0.0,0.41,18.02,15.2,31.85
396.0,53.1,0.63,0.68,0.77,0.0,0.0,2.22,1.46,66.93,0.82,0.7,0.78,0.0,0.01,5.4,3.14,80.77,0.92,0.76,0.74,0.0,0.02,8.02,5.93,64.22,1.03,0.77,0.8,0.0,0.04,11.51,7.79,46.43,0.88,0.83,0.8,0.0,0.08,12.64,10.97,37.62,0.88,0.82,0.82,0.0,0.17,16.85,11.51,34.67,0.84,0.84,1.01,0.0,0.41,18.31,17.01,31.96
397.0,54.21,0.63,0.68,0.77,0.0,0.0,2.22,1.47,67.1,0.83,0.71,0.78,0.0,0.01,5.54,3.14,81.4,0.92,0.76,0.75,0.0,0.02,8.3,6.0,65.07,1.04,0.77,0.8,0.0,0.04,11.61,7.96,46.79,0.89,0.84,0.8,0.0,0.08,13.76,11.34,39.6,0.88,0.83,0.82,0.0,0.17,17.29,11.72,34.7,0.84,0.84,1.01,0.0,0.41,18.63,19.17,32.48
398.0,54.5,0.63,0.68,0.78,0.0,0.0,2.27,1.51,72.4,0.83,0.72,0.79,0.0,0.01,5.87,3.34,81.51,0.94,0.76,0.76,0.0,0.02,10.86,6.41,65.31,1.04,0.77,0.8,0.0,0.04,12.58,8.2,49.51,0.9,0.84,0.81,0.0,0.08,15.33,11.71,39.85,0.89,0.84,0.82,0.0,0.17,18.31,11.76,34.89,0.85,0.85,1.02,0.0,0.41,18.72,19.24,33.11
399.0,54.97,0.63,0.68,0.78,0.0,0.0,2.3,1.52,73.07,0.84,0.72,0.79,0.0,0.01,5.95,3.34,83.99,0.95,0.76,0.76,0.0,0.02,11.09,6.61,65.52,1.04,0.78,0.8,0.0,0.04,12.66,8.66,49.91,0.9,0.84,0.81,0.0,0.08,16.21,12.27,40.39,0.9,0.84,0.82,0.0,0.17,19.01,12.21,35.91,0.85,0.85,1.03,0.0,0.41,18.85,19.58,33.46
400.0,55.43,0.64,0.69,0.78,0.0,0.0,2.3,1.56,73.8,0.84,0.74,0.79,0.0,0.01,6.05,3.47,84.0,0.95,0.77,0.76,0.0,0.02,11.4,6.73,66.34,1.04,0.78,0.81,0.0,0.04,12.71,8.77,49.94,0.9,0.86,0.81,0.0,0.08,16.97,12.98,40.42,0.91,0.84,0.82,0.0,0.17,19.88,12.83,36.24,0.85,0.85,1.04,0.0,0.41,18.94,20.11,33.5
401.0,55.97,0.64,0.7,0.79,0.0,0.0,2.33,1.61,74.42,0.86,0.74,0.81,0.0,0.01,6.27,3.71,84.62,0.95,0.77,0.77,0.0,0.02,11.51,6.74,66.53,1.05,0.8,0.82,0.0,0.04,14.06,9.64,50.35,0.91,0.87,0.82,0.0,0.08,17.41,13.42,41.19,0.93,0.84,0.83,0.0,0.17,20.23,13.54,36.34,0.85,0.85,1.05,0.0,0.41,20.11,20.18,33.8
402.0,56.99,0.64,0.7,0.8,0.0,0.0,2.37,1.62,77.12,0.86,0.75,0.81,0.0,0.01,6.52,4.0,86.86,0.96,0.77,0.77,0.0,0.02,12.14,8.14,66.84,1.06,0.8,0.83,0.0,0.04,14.22,10.97,50.69,0.92,0.88,0.82,0.0,0.08,17.59,13.78,41.41,0.93,0.85,0.84,0.0,0.17,20.46,14.82,36.39,0.87,0.87,1.05,0.0,0.41,20.71,20.35,34.51
403.0,57.36,0.64,0.71,0.8,0.0,0.0,2.38,1.63,77.13,0.87,0.76,0.81,0.0,0.01,6.71,4.08,86.96,0.97,0.78,0.77,0.0,0.02,12.84,8.77,66.85,1.06,0.83,0.84,0.0,0.04,14.44,11.44,50.76,0.93,0.89,0.82,0.0,0.08,19.01,13.78,41.54,0.93,0.86,0.85,0.0,0.17,20.74,15.6,37.45,0.89,0.89,1.07,0.0,0.41,20.96,21.12,34.99
404.0,59.06,0.65,0.71,0.82,0.0,0.0,2.46,1.64,81.7,0.89,0.77,0.81,0.0,0.01,7.0,4.41,87.05,0.98,0.79,0.77,0.0,0.02,13.56,9.23,69.07,1.07,0.83,0.84,0.0,0.04,14.57,11.71,51.55,0.93,0.89,0.84,0.0,0.08,19.45,14.06,41.76,0.95,0.86,0.85,0.0,0.17,21.53,15.64,37.62,0.9,0.9,1.09,0.0,0.41,21.69,21.31,35.14
405.0,59.68,0.66,0.72,0.82,0.0,0.0,2.46,1.71,82.35,0.92,0.77,0.81,0.0,0.01,7.12,4.51,88.05,0.98,0.79,0.78,0.0,0.02,14.44,10.4,69.54,1.08,0.83,0.84,0.0,0.04,15.7,12.27,52.35,0.93,0.9,0.85,0.0,0.08,20.07,14.98,42.56,0.95,0.88,0.86,0.0,0.17,22.04,16.03,38.29,0.9,0.9,1.09,0.0,0.41,23.21,21.42,35.41
406.0,61.45,0.67,0.72,0.82,0.0,0.0,2.5,1.72,84.46,0.92,0.78,0.81,0.0,0.01,7.41,4.7,88.16,0.98,0.79,0.78,0.0,0.02,14.98,10.83,69.89,1.08,0.84,0.84,0.0,0.04,16.05,14.78,52.55,0.95,0.91,0.85,0.0,0.08,20.09,15.64,43.62,0.96,0.9,0.86,0.0,0.17,22.83,17.25,39.02,0.91,0.91,1.09,0.0,0.41,23.32,23.14,37.07
407.0,64.12,0.68,0.73,0.82,0.0,0.0,2.51,1.73,84.86,0.93,0.78,0.81,0.0,0.01,7.42,4.84,90.22,1.0,0.8,0.78,0.0,0.02,15.15,11.65,70.16,1.09,0.84,0.85,0.0,0.04,16.27,15.26,53.1,0.95,0.91,0.85,0.0,0.08,20.3,15.68,43.68,0.96,0.9,0.86,0.0,0.17,22.85,17.87,40.11,0.91,0.91,1.12,0.0,0.41,23.39,23.62,37.89
408.0,65.26,0.68,0.73,0.82,0.0,0.0,2.53,1.74,85.6,0.94,0.79,0.82,0.0,0.01,8.02,5.0,90.7,1.01,0.8,0.78,0.0,0.02,15.19,13.44,70.76,1.09,0.85,0.86,0.0,0.04,17.01,16.2,53.18,0.96,0.91,0.86,0.0,0.08,20.53,17.23,44.17,0.99,0.91,0.86,0.0,0.17,23.32,18.83,41.19,0.92,0.92,1.12,0.0,0.41,23.46,24.09,39.16
409.0,65.29,0.68,0.73,0.82,0.0,0.0,2.62,1.74,87.78,0.94,0.79,0.82,0.0,0.01,8.11,5.56,91.1,1.01,0.8,0.78,0.0,0.02,15.32,13.99,70.84,1.1,0.86,0.86,0.0,0.04,17.07,16.89,53.44,0.97,0.91,0.86,0.0,0.08,20.96,19.0,45.72,0.99,0.93,0.87,0.0,0.17,23.61,19.18,41.34,0.93,0.93,1.12,0.0,0.41,24.71,24.96,42.5
410.0,65.51,0.69,0.74,0.83,0.0,0.0,2.69,1.79,88.18,0.95,0.8,0.82,0.0,0.01,8.24,5.78,94.03,1.01,0.8,0.79,0.0,0.02,16.13,14.33,72.03,1.1,0.87,0.86,0.0,0.04,17.45,17.41,57.4,0.98,0.92,0.86,0.0,0.08,21.17,19.18,46.21,1.01,0.94,0.88,0.0,0.17,24.51,21.71,41.81,0.95,0.95,1.13,0.0,0.41,24.77,26.08,42.93
411.0,66.15,0.7,0.75,0.83,0.0,0.0,2.75,1.8,89.72,0.96,0.81,0.83,0.0,0.01,8.3,5.78,94.19,1.02,0.81,0.79,0.0,0.02,16.25,15.44,72.16,1.11,0.87,0.86,0.0,0.04,17.52,18.22,58.42,1.01,0.93,0.86,0.0,0.08,22.28,19.64,48.06,1.01,0.94,0.88,0.0,0.17,24.96,22.57,42.38,0.95,0.95,1.14,0.0,0.41,25.05,26.25,43.0
412.0,66.45,0.7,0.76,0.83,0.0,0.0,2.81,1.84,90.14,0.96,0.81,0.84,0.0,0.01,8.35,5.98,96.08,1.03,0.82,0.79,0.0,0.02,16.35,15.51,73.05,1.11,0.88,0.86,0.0,0.04,17.8,19.32,59.84,1.01,0.93,0.88,0.0,0.08,23.84,20.13,48.4,1.01,0.94,0.88,0.0,0.17,25.33,22.91,42.45,0.95,0.95,1.16,0.0,0.41,25.14,27.74,43.25
413.0,68.21,0.71,0.76,0.83,0.0,0.0,2.84,1.88,92.31,0.97,0.81,0.84,0.0,0.01,8.37,6.42,97.45,1.03,0.82,0.8,0.0,0.02,16.38,15.84,73.95,1.11,0.88,0.86,0.0,0.04,19.13,19.5,60.0,1.02,0.95,0.89,0.0,0.08,23.98,20.39,48.52,1.02,0.94,0.88,0.0,0.17,25.74,23.21,42.93,0.97,0.97,1.16,0.0,0.41,25.2,28.96,44.2
414.0,68.64,0.72,0.77,0.84,0.0,0.0,2.9,1.91,93.91,0.98,0.82,0.86,0.0,0.01,8.68,6.9,97.62,1.04,0.82,0.81,0.0,0.02,16.51,16.0,74.22,1.11,0.89,0.87,0.0,0.04,20.75,20.16,60.42,1.02,0.96,0.89,0.0,0.08,24.06,20.4,49.28,1.03,0.95,0.88,0.0,0.17,27.94,24.16,42.95,0.98,0.98,1.16,0.0,0.41,25.24,29.21,44.73
415.0,69.05,0.72,0.77,0.84,0.0,0.0,2.95,1.91,94.33,0.99,0.82,0.86,0.0,0.01,8.86,7.05,99.64,1.04,0.83,0.81,0.0,0.02,16.68,16.44,74.57,1.12,0.89,0.87,0.0,0.04,22.4,21.51,60.65,1.03,0.98,0.89,0.0,0.08,24.32,21.71,49.47,1.05,0.98,0.88,0.0,0.17,28.2,24.27,42.98,0.98,0.98,1.18,0.0,0.41,25.77,29.36,46.09
416.0,72.07,0.74,0.78,0.85,0.0,0.0,2.97,1.95,95.14,1.02,0.82,0.87,0.0,0.01,8.95,7.18,100.36,1.05,0.83,0.81,0.0,0.02,17.96,16.79,78.63,1.12,0.89,0.87,0.0,0.04,23.6,22.27,61.75,1.03,0.98,0.89,0.0,0.08,24.51,22.18,49.58,1.06,0.99,0.89,0.0,0.17,28.43,24.5,44.17,0.98,0.98,1.18,0.0,0.41,27.93,29.83,46.76
417.0,72.16,0.76,0.79,0.85,0.0,0.0,3.26,1.97,96.04,1.03,0.83,0.87,0.0,0.01,8.96,7.25,100.57,1.05,0.83,0.81,0.0,0.02,18.83,17.59,80.19,1.12,0.9,0.87,0.0,0.04,23.71,22.41,62.22,1.04,0.99,0.9,0.0,0.08,26.23,22.29,49.84,1.08,0.99,0.9,0.0,0.17,28.5,25.98,46.9,0.99,0.99,1.21,0.0,0.41,28.31,31.01,47.13
418.0,72.71,0.76,0.79,0.86,0.0,0.0,3.26,2.09,100.68,1.03,0.83,0.87,0.0,0.01,9.72,7.69,101.02,1.07,0.84,0.81,0.0,0.02,18.94,17.67,84.91,1.13,0.91,0.88,0.0,0.04,23.82,22.59,66.16,1.05,0.99,0.91,0.0,0.08,28.91,22.36,50.33,1.09,1.01,0.91,0.0,0.17,28.82,26.21,47.1,0.99,0.99,1.21,0.0,0.41,28.5,31.14,49.07
419.0,73.18,0.76,0.79,0.86,0.0,0.0,3.28,2.15,101.05,1.05,0.83,0.88,0.0,0.01,9.79,8.01,101.97,1.07,0.86,0.81,0.0,0.02,19.2,18.16,86.04,1.13,0.92,0.88,0.0,0.04,24.25,22.89,66.41,1.06,1.0,0.92,0.0,0.08,29.56,23.9,53.33,1.1,1.03,0.91,0.0,0.17,28.91,27.13,47.53,1.0,1.0,1.21,0.0,0.41,28.71,31.62,49.37
420.0,73.57,0.77,0.8,0.86,0.0,0.0,3.33,2.15,102.53,1.07,0.83,0.89,0.0,0.01,10.54,8.24,105.7,1.08,0.86,0.82,0.0,0.02,19.96,18.28,86.93,1.13,0.92,0.88,0.0,0.04,26.24,24.89,66.89,1.07,1.0,0.92,0.0,0.08,30.34,25.09,53.44,1.11,1.05,0.91,0.0,0.17,28.94,27.59,48.06,1.0,1.0,1.22,0.0,0.41,29.63,32.02,49.56
421.0,73.93,0.78,0.8,0.87,0.0,0.0,3.35,2.24,108.41,1.08,0.84,0.89,0.0,0.01,10.74,9.23,111.98,1.08,0.86,0.82,0.0,0.02,20.08,18.88,87.73,1.14,0.97,0.89,0.0,0.04,26.56,24.96,70.53,1.07,1.02,0.92,0.0,0.08,30.9,25.5,54.58,1.12,1.06,0.92,0.0,0.17,30.18,28.47,49.28,1.0,1.0,1.23,0.0,0.41,30.46,32.16,50.32
422.0,75.52,0.79,0.81,0.88,0.0,0.0,3.36,2.39,111.62,1.09,0.84,0.89,0.0,0.01,10.95,9.46,114.49,1.09,0.86,0.82,0.0,0.02,20.32,19.08,88.53,1.14,0.97,0.9,0.0,0.04,26.73,25.6,71.34,1.07,1.03,0.92,0.0,0.08,31.86,25.61,55.12,1.12,1.06,0.92,0.0,0.17,32.06,29.3,49.67,1.01,1.01,1.25,0.0,0.41,31.11,32.59,50.72
423.0,76.0,0.8,0.82,0.88,0.0,0.0,3.41,2.39,115.98,1.1,0.85,0.91,0.0,0.01,11.01,9.66,116.93,1.1,0.86,0.82,0.0,0.02,20.99,19.1,90.52,1.15,0.98,0.92,0.0,0.04,27.76,26.11,73.93,1.1,1.04,0.93,0.0,0.08,33.94,25.95,55.24,1.13,1.06,0.93,0.0,0.17,32.59,29.6,50.15,1.03,1.03,1.25,0.0,0.41,31.6,33.52,51.21
424.0,76.68,0.8,0.83,0.88,0.0,0.0,3.43,2.41,116.36,1.1,0.86,0.91,0.0,0.01,11.37,10.19,119.86,1.1,0.86,0.83,0.0,0.02,21.29,19.73,90.94,1.16,0.99,0.92,0.0,0.04,27.77,26.25,75.72,1.1,1.04,0.95,0.0,0.08,35.05,26.67,57.19,1.13,1.06,0.95,0.0,0.17,33.27,29.7,51.8,1.04,1.04,1.25,0.0,0.41,32.73,33.76,51.53
425.0,77.5,0.81,0.83,0.88,0.0,0.0,3.52,2.41,117.01,1.1,0.87,0.92,0.0,0.01,11.44,10.67,121.49,1.1,0.88,0.83,0.0,0.02,22.02,20.06,91.51,1.17,0.99,0.93,0.0,0.04,27.98,28.72,76.99,1.11,1.05,0.96,0.0,0.08,35.33,26.77,58.78,1.13,1.07,0.96,0.0,0.17,33.29,29.97,52.47,1.05,1.05,1.29,0.0,0.41,33.51,34.12,53.92
426.0,79.48,0.81,0.84,0.89,0.0,0.0,3.66,2.45,117.41,1.1,0.88,0.92,0.0,0.01,11.55,11.34,122.08,1.1,0.88,0.84,0.0,0.02,22.19,21.35,94.07,1.2,1.0,0.93,0.0,0.04,28.36,29.05,79.38,1.12,1.05,0.96,0.0,0.08,35.74,26.89,59.24,1.14,1.07,0.96,0.0,0.17,33.57,30.49,52.47,1.06,1.06,1.3,0.0,0.41,33.64,34.49,54.03
427.0,80.6,0.81,0.86,0.89,0.0,0.0,3.91,2.48,118.27,1.11,0.89,0.93,0.0,0.01,11.89,11.49,122.43,1.11,0.89,0.84,0.0,0.02,22.81,22.39,94.19,1.2,1.01,0.94,0.0,0.04,28.73,29.4,81.67,1.13,1.05,0.96,0.0,0.08,36.27,28.7,60.38,1.15,1.08,0.98,0.0,0.17,34.37,30.77,55.04,1.07,1.07,1.32,0.0,0.41,34.09,34.74,55.05
428.0,80.89,0.81,0.87,0.91,0.0,0.0,4.03,2.61,132.64,1.11,0.9,0.93,0.0,0.01,14.13,11.67,126.3,1.11,0.89,0.84,0.0,0.02,22.91,23.8,94.55,1.2,1.01,0.95,0.0,0.04,28.86,29.48,84.87,1.13,1.06,0.97,0.0,0.08,37.47,28.9,62.37,1.18,1.08,0.98,0.0,0.17,35.33,30.94,55.05,1.07,1.07,1.32,0.0,0.41,37.17,34.78,55.83
429.0,81.75,0.82,0.87,0.91,0.0,0.0,4.11,2.7,136.54,1.12,0.9,0.94,0.0,0.01,14.32,11.9,129.06,1.12,0.91,0.85,0.0,0.02,23.71,25.4,94.61,1.21,1.01,0.96,0.0,0.04,28.91,29.7,85.14,1.13,1.06,0.97,0.0,0.08,37.65,29.3,63.88,1.18,1.08,0.98,0.0,0.17,36.48,31.83,57.19,1.08,1.08,1.33,0.0,0.41,37.18,35.41,56.1
430.0,83.95,0.82,0.87,0.91,0.0,0.0,4.17,2.78,136.75,1.12,0.91,0.94,0.0,0.01,14.44,12.0,129.7,1.13,0.91,0.85,0.0,0.02,24.32,25.52,94.98,1.22,1.02,0.96,0.0,0.04,29.08,30.37,85.52,1.14,1.06,0.98,0.0,0.08,37.76,29.8,64.87,1.2,1.09,1.0,0.0,0.17,37.13,31.99,59.49,1.08,1.08,1.34,0.0,0.41,38.54,35.64,56.34
431.0,84.3,0.83,0.88,0.92,0.0,0.0,4.18,2.85,140.04,1.13,0.91,0.94,0.0,0.01,14.52,12.19,131.21,1.13,0.92,0.87,0.0,0.02,24.44,25.57,97.06,1.24,1.05,0.96,0.0,0.04,29.09,30.95,88.01,1.14,1.07,0.98,0.0,0.08,39.02,30.08,65.2,1.2,1.09,1.0,0.0,0.17,37.24,32.16,59.76,1.08,1.08,1.36,0.0,0.41,38.6,35.97,58.61
432.0,85.39,0.84,0.88,0.94,0.0,0.0,4.22,2.88,141.26,1.14,0.91,0.95,0.0,0.01,14.96,12.61,148.14,1.14,0.92,0.88,0.0,0.02,24.81,25.58,99.64,1.24,1.06,0.97,0.0,0.04,29.09,31.79,88.37,1.15,1.07,0.99,0.0,0.08,39.32,30.82,65.83,1.21,1.1,1.02,0.0,0.17,37.64,32.34,61.96,1.09,1.09,1.37,0.0,0.41,38.88,36.93,58.83
433.0,86.89,0.84,0.9,0.95,0.0,0.0,4.25,2.93,142.13,1.19,0.92,0.95,0.0,0.01,15.13,13.53,148.27,1.15,0.93,0.9,0.0,0.02,25.73,26.25,100.38,1.24,1.06,0.97,0.0,0.04,31.86,31.86,89.61,1.16,1.08,1.0,0.0,0.08,40.42,30.94,67.6,1.21,1.11,1.02,0.0,0.17,37.65,32.92,62.06,1.11,1.11,1.37,0.0,0.41,42.93,38.39,59.41
434.0,88.92,0.84,0.9,0.97,0.0,0.0,4.25,2.97,143.22,1.21,0.92,0.98,0.0,0.01,15.44,13.88,148.37,1.16,0.96,0.92,0.0,0.02,25.77,26.48,101.92,1.25,1.08,0.98,0.0,0.04,32.88,32.79,90.69,1.17,1.08,1.0,0.0,0.08,40.9,31.2,68.79,1.22,1.11,1.02,0.0,0.17,38.88,33.14,62.32,1.12,1.12,1.39,0.0,0.41,45.31,38.67,59.53
435.0,91.34,0.84,0.9,0.97,0.0,0.0,4.26,2.97,145.21,1.23,0.94,0.99,0.0,0.01,15.5,13.99,153.55,1.17,0.96,0.93,0.0,0.02,26.21,26.81,101.97,1.26,1.09,1.0,0.0,0.04,33.09,32.89,92.71,1.18,1.08,1.02,0.0,0.08,40.91,31.23,71.74,1.22,1.14,1.04,0.0,0.17,39.02,33.71,63.1,1.12,1.12,1.4,0.0,0.41,45.62,38.74,62.52
436.0,93.62,0.84,0.9,0.98,0.0,0.0,4.26,3.05,147.49,1.23,0.95,0.99,0.0,0.01,16.28,14.14,162.94,1.18,0.96,0.94,0.0,0.02,26.88,27.41,105.49,1.27,1.1,1.0,0.0,0.04,33.19,33.71,92.94,1.18,1.09,1.02,0.0,0.08,41.52,31.86,73.27,1.23,1.15,1.04,0.0,0.17,39.32,34.75,63.54,1.12,1.12,1.4,0.0,0.41,46.35,39.19,64.44
437.0,96.32,0.85,0.91,0.98,0.0,0.0,4.39,3.08,147.84,1.23,0.95,1.01,0.0,0.01,17.17,15.1,175.44,1.18,0.96,0.94,0.0,0.02,27.99,28.42,108.34,1.28,1.11,1.01,0.0,0.04,33.79,34.01,96.37,1.19,1.11,1.03,0.0,0.08,42.68,32.34,76.45,1.23,1.15,1.04,0.0,0.17,39.85,36.2,63.89,1.12,1.12,1.42,0.0,0.41,47.42,39.38,65.3
438.0,96.57,0.85,0.93,0.99,0.0,0.0,4.61,3.09,148.54,1.24,0.96,1.01,0.0,0.01,17.24,15.22,176.04,1.2,0.97,0.95,0.0,0.02,28.5,29.09,111.65,1.29,1.11,1.01,0.0,0.04,33.94,34.07,101.16,1.21,1.11,1.04,0.0,0.08,43.04,32.7,78.01,1.25,1.15,1.04,0.0,0.17,39.88,36.74,64.03,1.13,1.13,1.44,0.0,0.41,47.79,39.64,65.76
439.0,100.78,0.85,0.93,1.0,0.0,0.0,4.7,3.18,148.96,1.26,0.99,1.02,0.0,0.01,17.57,15.39,184.2,1.22,0.98,0.95,0.0,0.02,29.72,29.22,111.92,1.29,1.11,1.01,0.0,0.04,36.83,34.58,102.05,1.22,1.11,1.05,0.0,0.08,43.24,33.36,78.03,1.26,1.16,1.04,0.0,0.17,40.62,37.1,64.3,1.14,1.14,1.45,0.0,0.41,47.99,40.21,65.83
440.0,102.69,0.85,0.95,1.01,0.0,0.0,4.86,3.42,150.14,1.28,1.0,1.02,0.0,0.01,17.76,15.72,203.66,1.24,1.01,0.96,0.0,0.02,30.95,29.55,116.39,1.29,1.12,1.02,0.0,0.04,37.6,34.78,102.1,1.23,1.12,1.06,0.0,0.08,43.77,33.71,79.55,1.28,1.17,1.04,0.0,0.17,41.39,37.46,64.93,1.14,1.14,1.45,0.0,0.41,52.35,41.09,65.91
441.0,103.64,0.86,0.95,1.01,0.0,0.0,4.95,3.5,160.13,1.32,1.0,1.03,0.0,0.01,18.32,16.31,204.35,1.24,1.01,1.0,0.0,0.02,31.02,29.66,120.5,1.29,1.13,1.02,0.0,0.04,37.76,34.84,104.92,1.24,1.13,1.06,0.0,0.08,44.0,34.07,83.26,1.3,1.18,1.05,0.0,0.17,41.52,38.51,65.2,1.15,1.15,1.46,0.0,0.41,53.84,41.71,67.05
442.0,108.85,0.87,0.95,1.01,0.0,0.0,4.98,3.5,163.32,1.32,1.0,1.03,0.0,0.01,18.38,16.68,207.12,1.24,1.02,1.01,0.0,0.02,31.76,30.27,129.06,1.31,1.13,1.02,0.0,0.04,37.77,35.47,105.32,1.29,1.13,1.06,0.0,0.08,45.43,35.77,85.04,1.31,1.2,1.05,0.0,0.17,41.98,38.78,65.78,1.15,1.15,1.46,0.0,0.41,54.65,42.01,69.74
443.0,114.54,0.87,0.96,1.02,0.0,0.0,5.1,3.52,173.88,1.32,1.01,1.03,0.0,0.01,19.33,16.79,210.12,1.27,1.02,1.02,0.0,0.02,32.15,30.37,132.13,1.31,1.16,1.04,0.0,0.04,37.98,35.49,106.5,1.29,1.14,1.07,0.0,0.08,45.82,36.0,86.98,1.34,1.2,1.07,0.0,0.17,42.68,40.44,65.89,1.16,1.16,1.47,0.0,0.41,56.03,42.25,70.62
444.0,115.57,0.88,0.96,1.03,0.0,0.0,5.27,3.6,182.11,1.33,1.01,1.04,0.0,0.01,19.68,17.76,210.2,1.28,1.04,1.02,0.0,0.02,33.08,30.5,134.89,1.32,1.18,1.04,0.0,0.04,38.3,35.81,109.86,1.29,1.15,1.08,0.0,0.08,46.2,37.42,87.79,1.35,1.24,1.08,0.0,0.17,43.04,40.72,66.93,1.16,1.16,1.47,0.0,0.41,56.35,42.47,71.44
445.0,116.45,0.88,0.97,1.04,0.0,0.0,5.29,3.61,190.03,1.34,1.01,1.04,0.0,0.01,20.64,17.98,225.49,1.28,1.05,1.02,0.0,0.02,33.31,30.89,141.09,1.33,1.19,1.04,0.0,0.04,39.14,36.84,112.71,1.3,1.17,1.09,0.0,0.08,46.27,37.46,88.04,1.36,1.24,1.08,0.0,0.17,43.26,41.34,71.66,1.22,1.22,1.48,0.0,0.41,57.81,43.23,72.36
446.0,117.97,0.88,0.99,1.04,0.0,0.0,5.31,3.7,193.51,1.34,1.03,1.05,0.0,0.01,20.81,18.31,231.49,1.29,1.05,1.03,0.0,0.02,33.88,31.54,142.88,1.34,1.2,1.04,0.0,0.04,39.71,36.98,115.12,1.31,1.17,1.11,0.0,0.08,46.38,37.96,89.49,1.37,1.25,1.08,0.0,0.17,44.35,41.54,76.61,1.22,1.22,1.48,0.0,0.41,59.63,44.96,73.95
447.0,121.75,0.88,1.02,1.04,0.0,0.0,5.44,3.77,196.98,1.36,1.03,1.06,0.0,0.01,21.44,18.38,240.48,1.32,1.06,1.03,0.0,0.02,34.13,31.79,147.11,1.35,1.21,1.05,0.0,0.04,39.98,37.3,118.97,1.36,1.17,1.13,0.0,0.08,46.92,38.1,91.22,1.37,1.26,1.09,0.0,0.17,44.68,41.75,77.69,1.24,1.24,1.48,0.0,0.41,60.27,46.0,74.06
448.0,122.11,0.88,1.02,1.04,0.0,0.0,5.65,3.9,199.81,1.38,1.05,1.06,0.0,0.01,22.07,18.47,260.7,1.32,1.07,1.04,0.0,0.02,35.31,32.41,147.17,1.36,1.24,1.09,0.0,0.04,40.69,37.96,127.29,1.4,1.18,1.13,0.0,0.08,47.19,39.74,96.23,1.38,1.27,1.1,0.0,0.17,46.94,43.11,78.96,1.24,1.24,1.5,0.0,0.41,60.54,46.76,76.6
449.0,122.68,0.89,1.03,1.07,0.0,0.0,5.87,3.97,201.82,1.38,1.06,1.08,0.0,0.01,22.41,19.33,262.69,1.34,1.07,1.05,0.0,0.02,36.07,32.83,150.22,1.36,1.24,1.09,0.0,0.04,41.38,38.05,130.79,1.45,1.18,1.13,0.0,0.08,48.25,41.06,96.37,1.38,1.27,1.1,0.0,0.17,47.47,45.32,80.1,1.27,1.27,1.5,0.0,0.41,62.55,47.91,77.52
450.0,128.97,0.91,1.04,1.07,0.0,0.0,5.88,4.36,206.81,1.39,1.07,1.09,0.0,0.01,23.27,19.78,286.94,1.35,1.1,1.07,0.0,0.02,36.69,32.92,150.43,1.38,1.24,1.12,0.0,0.04,41.73,39.03,131.45,1.51,1.2,1.14,0.0,0.08,48.59,41.63,102.05,1.4,1.28,1.13,0.0,0.17,49.29,45.44,83.26,1.27,1.27,1.51,0.0,0.41,63.51,48.9,79.31
451.0,135.8,0.91,1.05,1.08,0.0,0.0,6.29,4.37,209.5,1.39,1.07,1.09,0.0,0.01,23.5,20.03,297.27,1.37,1.11,1.07,0.0,0.02,36.91,33.22,162.1,1.39,1.25,1.13,0.0,0.04,41.86,39.58,135.57,1.53,1.2,1.14,0.0,0.08,48.64,41.73,104.34,1.42,1.29,1.15,0.0,0.17,51.33,47.41,84.95,1.3,1.3,1.52,0.0,0.41,64.59,49.03,79.35
452.0,164.45,0.92,1.05,1.08,0.0,0.0,6.3,4.38,210.37,1.41,1.08,1.1,0.0,0.01,23.87,20.7,297.97,1.4,1.13,1.07,0.0,0.02,37.12,35.24,167.49,1.4,1.26,1.14,0.0,0.04,42.2,41.06,137.25,1.54,1.22,1.15,0.0,0.08,49.11,42.34,106.44,1.42,1.34,1.15,0.0,0.17,52.08,48.3,85.98,1.3,1.3,1.53,0.0,0.41,64.64,49.43,79.78
453.0,165.28,0.92,1.09,1.08,0.0,0.0,6.32,4.42,212.53,1.41,1.08,1.11,0.0,0.01,24.37,24.73,310.97,1.43,1.13,1.11,0.0,0.02,37.28,35.33,189.98,1.4,1.26,1.15,0.0,0.04,42.68,41.49,141.09,1.55,1.23,1.17,0.0,0.08,51.0,42.7,109.25,1.43,1.34,1.15,0.0,0.17,52.18,48.43,87.19,1.31,1.31,1.53,0.0,0.41,65.56,51.07,80.48
454.0,167.35,0.94,1.09,1.09,0.0,0.0,6.63,4.75,225.47,1.43,1.08,1.12,0.0,0.01,24.53,24.89,329.95,1.43,1.14,1.11,0.0,0.02,39.98,35.44,203.09,1.41,1.26,1.16,0.0,0.04,42.68,42.21,143.49,1.55,1.26,1.17,0.0,0.08,51.68,43.5,109.93,1.44,1.36,1.17,0.0,0.17,54.01,49.2,87.32,1.34,1.34,1.55,0.0,0.41,65.94,51.92,84.15
455.0,171.18,0.96,1.15,1.09,0.0,0.0,6.64,4.88,238.32,1.43,1.09,1.13,0.0,0.01,24.78,25.06,352.36,1.43,1.14,1.14,0.0,0.02,40.02,35.5,213.65,1.42,1.27,1.18,0.0,0.04,42.78,42.7,147.17,1.6,1.27,1.18,0.0,0.08,52.08,45.07,110.47,1.45,1.36,1.23,0.0,0.17,54.77,49.39,88.02,1.35,1.35,1.56,0.0,0.41,65.97,52.14,89.19
456.0,171.66,0.97,1.21,1.1,0.0,0.0,6.91,4.94,244.1,1.45,1.1,1.13,0.0,0.01,24.96,25.1,355.35,1.44,1.14,1.17,0.0,0.02,40.84,35.68,217.83,1.43,1.28,1.19,0.0,0.04,46.2,42.84,148.96,1.61,1.27,1.19,0.0,0.08,54.01,45.32,117.99,1.45,1.37,1.23,0.0,0.17,57.22,49.44,88.93,1.35,1.35,1.57,0.0,0.41,67.98,52.16,91.72
457.0,180.85,1.01,1.26,1.13,0.0,0.0,6.95,5.1,261.23,1.46,1.12,1.13,0.0,0.01,25.58,25.21,368.11,1.49,1.14,1.19,0.0,0.02,41.51,35.74,220.39,1.46,1.29,1.2,0.0,0.04,46.38,44.43,160.23,1.61,1.28,1.19,0.0,0.08,54.48,45.83,118.97,1.46,1.42,1.25,0.0,0.17,57.43,49.62,92.28,1.36,1.36,1.62,0.0,0.41,68.0,54.06,94.31
458.0,210.48,1.02,1.27,1.15,0.0,0.0,7.09,5.18,269.67,1.52,1.12,1.14,0.0,0.01,25.8,26.63,374.8,1.49,1.16,1.19,0.0,0.02,42.67,35.81,247.16,1.46,1.3,1.28,0.0,0.04,46.64,46.16,164.64,1.66,1.28,1.19,0.0,0.08,54.56,49.2,120.89,1.47,1.52,1.25,0.0,0.17,58.23,51.23,93.96,1.38,1.38,1.63,0.0,0.41,68.72,56.03,94.57
459.0,219.43,1.03,1.28,1.17,0.0,0.0,7.16,5.23,271.42,1.58,1.12,1.15,0.0,0.01,26.26,27.54,391.24,1.49,1.18,1.19,0.0,0.02,42.68,37.32,255.09,1.51,1.31,1.28,0.0,0.04,47.8,48.04,170.19,1.67,1.32,1.24,0.0,0.08,58.56,49.44,124.31,1.51,1.55,1.28,0.0,0.17,60.37,53.3,94.86,1.38,1.38,1.64,0.0,0.41,69.75,57.24,97.64
460.0,220.2,1.1,1.29,1.17,0.0,0.0,7.28,5.26,291.49,1.6,1.14,1.16,0.0,0.01,26.39,27.79,404.58,1.5,1.18,1.24,0.0,0.02,42.78,38.05,258.48,1.53,1.32,1.29,0.0,0.04,47.82,48.28,174.68,1.68,1.36,1.25,0.0,0.08,60.58,50.24,125.37,1.51,1.57,1.29,0.0,0.17,60.97,53.77,95.99,1.38,1.38,1.66,0.0,0.41,69.83,58.08,98.03
461.0,226.33,1.11,1.29,1.19,0.0,0.0,7.48,5.27,314.16,1.6,1.15,1.17,0.0,0.01,26.88,28.95,421.04,1.52,1.19,1.25,0.0,0.02,42.85,38.31,261.37,1.54,1.34,1.32,0.0,0.04,48.59,48.41,177.62,1.71,1.36,1.25,0.0,0.08,62.18,50.34,127.3,1.52,1.57,1.29,0.0,0.17,61.12,54.61,104.34,1.42,1.42,1.67,0.0,0.41,70.26,58.35,100.57
462.0,238.6,1.12,1.33,1.2,0.0,0.0,8.02,5.85,331.13,1.61,1.15,1.17,0.0,0.01,27.14,28.98,585.57,1.52,1.22,1.25,0.0,0.02,43.91,39.1,278.93,1.6,1.34,1.34,0.0,0.04,48.74,48.83,179.61,1.76,1.37,1.25,0.0,0.08,62.51,51.69,130.42,1.52,1.6,1.31,0.0,0.17,62.51,57.31,105.33,1.44,1.44,1.7,0.0,0.41,73.55,58.88,100.6
463.0,239.73,1.12,1.42,1.21,0.0,0.0,8.1,6.15,352.81,1.63,1.15,1.21,0.0,0.01,27.17,29.02,606.12,1.53,1.22,1.28,0.0,0.02,45.12,40.47,297.97,1.61,1.39,1.35,0.0,0.04,49.29,49.2,189.98,1.81,1.37,1.26,0.0,0.08,66.28,51.77,131.64,1.52,1.62,1.35,0.0,0.17,63.56,57.39,108.5,1.45,1.45,1.72,0.0,0.41,75.18,59.95,100.69
464.0,240.55,1.15,1.46,1.22,0.0,0.0,8.19,6.75,375.73,1.64,1.16,1.23,0.0,0.01,27.35,31.31,646.7,1.55,1.23,1.33,0.0,0.02,47.13,41.62,301.26,1.61,1.4,1.42,0.0,0.04,49.69,50.07,214.55,1.82,1.37,1.26,0.0,0.08,66.5,51.84,134.02,1.55,1.64,1.35,0.0,0.17,64.0,59.29,109.25,1.46,1.46,1.73,0.0,0.41,76.62,60.42,100.81
465.0,253.67,1.15,1.46,1.26,0.0,0.0,8.2,7.3,382.84,1.66,1.28,1.24,0.0,0.01,27.84,32.77,677.3,1.57,1.23,1.35,0.0,0.02,48.74,41.84,329.95,1.65,1.42,1.43,0.0,0.04,51.62,50.49,214.78,1.83,1.38,1.32,0.0,0.08,67.45,55.17,136.55,1.55,1.65,1.39,0.0,0.17,64.99,60.9,109.68,1.47,1.47,1.75,0.0,0.41,80.93,60.49,104.21
466.0,257.28,1.16,1.47,1.26,0.0,0.0,8.34,7.44,406.62,1.7,1.31,1.24,0.0,0.01,28.01,32.95,754.54,1.6,1.23,1.37,0.0,0.02,51.42,42.4,367.04,1.67,1.43,1.44,0.0,0.04,52.25,50.84,220.39,1.83,1.4,1.33,0.0,0.08,68.63,55.27,137.36,1.58,1.68,1.4,0.0,0.17,65.29,61.03,111.78,1.48,1.48,1.77,0.0,0.41,81.52,61.66,106.57
467.0,274.76,1.17,1.49,1.28,0.0,0.0,8.71,7.46,436.35,1.71,1.33,1.25,0.0,0.01,28.32,33.08,757.75,1.6,1.26,1.39,0.0,0.02,52.66,42.7,392.08,1.68,1.48,1.44,0.0,0.04,52.37,57.34,234.48,1.89,1.4,1.36,0.0,0.08,69.03,55.62,139.3,1.59,1.73,1.41,0.0,0.17,67.45,61.97,118.73,1.5,1.5,1.77,0.0,0.41,83.83,64.17,107.61
468.0,309.17,1.17,1.53,1.31,0.0,0.0,8.73,7.92,459.84,1.75,1.35,1.27,0.0,0.01,32.18,35.94,809.12,1.69,1.27,1.4,0.0,0.02,52.78,43.6,407.92,1.68,1.49,1.46,0.0,0.04,53.0,58.56,240.12,1.89,1.43,1.36,0.0,0.08,74.58,56.24,141.21,1.59,1.79,1.42,0.0,0.17,73.61,63.62,119.55,1.5,1.5,1.77,0.0,0.41,84.03,64.35,108.32
469.0,344.56,1.19,1.57,1.31,0.0,0.0,9.05,8.14,461.42,1.78,1.35,1.29,0.0,0.01,32.37,36.05,1031.59,1.73,1.29,1.44,0.0,0.02,55.12,43.88,437.49,1.7,1.49,1.48,0.0,0.04,53.54,58.82,247.16,1.9,1.47,1.36,0.0,0.08,76.82,57.83,141.58,1.69,1.8,1.49,0.0,0.17,77.7,63.98,120.4,1.5,1.5,1.79,0.0,0.41,87.44,65.62,110.37
470.0,347.68,1.2,1.62,1.33,0.0,0.0,9.3,8.32,510.56,1.8,1.36,1.32,0.0,0.01,33.65,37.1,1182.32,1.73,1.3,1.44,0.0,0.02,56.23,44.09,447.73,1.74,1.53,1.53,0.0,0.04,55.99,59.01,261.89,1.92,1.49,1.38,0.0,0.08,77.04,58.07,145.65,1.7,1.81,1.5,0.0,0.17,79.46,66.23,122.99,1.5,1.5,1.81,0.0,0.41,92.96,66.09,117.31
471.0,407.84,1.2,1.64,1.4,0.0,0.0,9.86,8.52,539.31,1.81,1.36,1.32,0.0,0.01,34.58,37.42,1390.13,1.79,1.3,1.47,0.0,0.02,56.36,44.43,450.29,1.75,1.53,1.53,0.0,0.04,56.23,59.05,266.17,1.95,1.51,1.39,0.0,0.08,77.34,58.85,153.08,1.73,1.85,1.53,0.0,0.17,81.89,66.48,133.56,1.51,1.51,1.84,0.0,0.41,94.12,66.48,119.53
472.0,422.93,1.23,1.73,1.41,0.0,0.0,10.37,8.79,568.01,1.88,1.36,1.41,0.0,0.01,34.83,39.88,1418.39,1.8,1.3,1.47,0.0,0.02,56.75,49.2,472.42,1.77,1.55,1.54,0.0,0.04,58.51,60.58,304.29,1.96,1.57,1.43,0.0,0.08,77.7,60.58,160.23,1.79,1.9,1.57,0.0,0.17,82.09,69.91,145.65,1.57,1.57,1.87,0.0,0.41,100.35,68.82,122.69
473.0,482.85,1.23,1.73,1.43,0.0,0.0,10.71,9.23,640.36,2.04,1.38,1.42,0.0,0.01,35.98,40.45,1507.05,1.8,1.31,1.48,0.0,0.02,58.08,50.07,484.39,1.79,1.57,1.58,0.0,0.04,59.9,62.19,305.44,1.96,1.6,1.47,0.0,0.08,77.74,60.62,161.4,1.85,1.93,1.58,0.0,0.17,82.31,72.86,145.76,1.57,1.57,1.96,0.0,0.41,102.65,70.84,135.2
474.0,535.02,1.24,1.74,1.49,0.0,0.0,11.44,9.34,640.79,2.04,1.4,1.45,0.0,0.01,39.39,41.34,1529.73,1.81,1.32,1.52,0.0,0.02,58.32,50.68,486.52,1.8,1.57,1.6,0.0,0.04,61.78,65.8,312.26,1.98,1.64,1.55,0.0,0.08,79.01,61.14,162.27,1.88,1.96,1.58,0.0,0.17,84.03,73.82,148.93,1.6,1.6,1.97,0.0,0.41,105.79,82.94,144.83
475.0,573.87,1.27,1.76,1.51,0.0,0.0,12.26,9.76,660.9,2.04,1.45,1.53,0.0,0.01,40.02,41.35,1573.95,1.81,1.37,1.56,0.0,0.02,58.81,50.85,596.66,1.85,1.57,1.61,0.0,0.04,63.57,67.44,368.69,2.14,1.69,1.55,0.0,0.08,80.95,62.45,166.04,1.88,1.96,1.61,0.0,0.17,87.42,76.83,156.09,1.6,1.6,1.97,0.0,0.41,109.91,86.16,148.65
476.0,596.34,1.28,1.84,1.55,0.0,0.0,12.89,9.91,740.71,2.04,1.45,1.55,0.0,0.01,40.42,42.4,1871.29,1.82,1.37,1.57,0.0,0.02,61.22,52.24,616.02,1.91,1.58,1.63,0.0,0.04,65.26,70.35,377.61,2.19,1.69,1.59,0.0,0.08,83.73,63.62,173.24,1.89,1.98,1.63,0.0,0.17,90.42,79.99,161.37,1.62,1.62,2.0,0.0,0.41,111.39,92.65,155.26
477.0,599.26,1.34,2.03,1.61,0.0,0.0,13.82,10.98,861.86,2.08,1.49,1.56,0.0,0.01,40.81,42.73,2203.36,1.84,1.4,1.59,0.0,0.02,61.29,52.58,650.62,1.98,1.61,1.66,0.0,0.04,66.94,74.49,471.27,2.19,1.7,1.59,0.0,0.08,86.38,63.98,174.72,1.9,2.03,1.67,0.0,0.17,95.96,80.43,161.4,1.65,1.65,2.04,0.0,0.41,113.21,98.26,157.53
478.0,736.64,1.37,2.06,1.62,0.0,0.0,14.74,11.12,980.65,2.1,1.51,1.62,0.0,0.01,40.84,43.52,2564.14,1.87,1.4,1.6,0.0,0.02,61.64,54.25,663.31,1.98,1.62,1.72,0.0,0.04,71.8,76.6,521.47,2.24,1.74,1.61,0.0,0.08,90.42,64.56,176.77,1.9,2.07,1.72,0.0,0.17,96.18,85.87,173.42,1.67,1.67,2.15,0.0,0.41,115.24,99.1,164.94
479.0,740.43,1.44,2.32,1.67,0.0,0.0,14.98,12.22,1061.58,2.19,1.52,1.65,0.0,0.01,40.91,44.09,2662.35,1.88,1.47,1.62,0.0,0.02,61.78,54.88,728.98,2.0,1.67,1.73,0.0,0.04,82.01,76.94,547.32,2.36,1.76,1.63,0.0,0.08,96.18,67.42,188.59,1.94,2.08,1.76,0.0,0.17,99.15,86.8,176.77,1.7,1.7,2.17,0.0,0.41,117.08,100.37,168.4
480.0,748.35,1.48,2.46,1.7,0.0,0.0,15.41,12.8,1127.39,2.22,1.56,1.67,0.0,0.01,41.79,44.43,3111.76,1.93,1.51,1.66,0.0,0.02,62.27,57.62,937.7,2.05,1.68,1.77,0.0,0.04,83.73,80.07,567.77,2.4,1.77,1.64,0.0,0.08,98.07,68.6,189.98,1.96,2.11,1.76,0.0,0.17,106.36,90.68,194.94,1.71,1.71,2.21,0.0,0.41,122.34,102.37,183.92
481.0,909.27,1.48,2.62,1.72,0.0,0.0,15.44,13.37,1134.66,2.23,1.57,1.68,0.0,0.01,41.89,46.7,3600.0,2.04,1.55,1.66,0.0,0.02,62.89,59.92,1098.2,2.12,1.69,1.77,0.0,0.04,84.62,80.97,596.66,2.4,1.78,1.65,0.0,0.08,102.73,71.92,203.88,1.96,2.16,1.79,0.0,0.17,112.47,96.44,203.06,1.71,1.71,2.24,0.0,0.41,125.45,109.43,187.66
482.0,1216.85,1.49,2.78,1.75,0.0,0.0,15.82,14.15,2198.94,2.24,1.59,1.7,0.0,0.01,41.91,47.72,3600.0,2.07,1.56,1.69,0.0,0.02,65.33,60.12,1207.47,2.24,1.78,1.78,0.0,0.04,90.82,83.92,654.34,2.41,1.82,1.65,0.0,0.08,108.88,75.03,213.91,2.01,2.18,1.81,0.0,0.17,115.24,99.24,213.91,1.73,1.73,2.26,0.0,0.41,125.65,110.27,192.83
483.0,1221.21,1.49,3600.0,1.83,0.0,0.0,16.78,15.07,3600.0,2.31,1.6,1.71,0.0,0.01,45.74,47.86,3600.0,2.17,1.57,1.69,0.0,0.02,65.85,63.62,1659.48,2.4,1.81,1.82,0.0,0.04,92.2,84.46,672.43,2.55,1.92,1.67,0.0,0.08,118.44,76.6,221.33,2.02,2.2,1.82,0.0,0.17,120.56,117.09,214.58,1.74,1.74,2.32,0.0,0.41,126.6,111.04,241.26
484.0,1316.4,1.51,3600.0,1.9,0.0,0.0,17.54,15.44,3600.0,2.37,1.61,1.74,0.0,0.01,49.53,49.31,3600.0,2.19,1.63,1.73,0.0,0.02,66.38,64.11,1733.83,2.42,1.81,1.83,0.0,0.04,96.93,89.03,767.27,2.75,2.0,1.69,0.0,0.08,122.81,85.87,222.26,2.03,2.21,1.84,0.0,0.17,125.6,123.14,235.08,1.8,1.8,2.36,0.0,0.41,138.45,112.48,257.52
485.0,1525.88,1.55,3600.0,1.91,0.0,0.0,18.62,16.74,3600.0,2.37,1.64,1.77,0.0,0.01,49.94,49.57,3600.0,2.19,1.64,1.79,0.0,0.02,70.98,65.96,2086.67,2.44,1.82,1.87,0.0,0.04,104.22,94.59,834.0,2.79,2.03,1.73,0.0,0.08,123.68,90.63,245.5,2.05,2.23,1.95,0.0,0.17,129.58,137.19,243.76,1.85,1.85,2.37,0.0,0.41,144.43,116.96,278.55
486.0,1984.6,1.56,3600.0,1.97,0.0,0.0,19.63,16.8,3600.0,2.42,1.66,1.82,0.0,0.01,54.98,50.57,3600.0,2.38,1.67,1.79,0.0,0.02,71.8,68.33,3600.0,2.52,1.87,1.91,0.0,0.04,106.43,96.8,1019.64,2.91,2.05,1.73,0.0,0.08,125.6,105.78,304.29,2.1,2.33,1.96,0.0,0.17,135.64,144.15,253.09,1.89,1.89,2.65,0.0,0.41,160.43,124.89,302.53
487.0,3094.19,1.56,3600.0,1.97,0.0,0.0,20.17,17.28,3600.0,2.55,1.67,1.83,0.0,0.01,56.36,54.88,3600.0,2.44,1.69,1.84,0.0,0.02,72.39,70.31,3600.0,2.58,1.88,1.91,0.0,0.04,109.46,104.73,1048.52,2.94,2.15,1.74,0.0,0.08,126.53,111.7,305.44,2.14,2.34,1.98,0.0,0.17,139.01,146.66,257.96,1.94,1.94,2.73,0.0,0.41,185.73,130.5,343.23
488.0,3600.0,1.6,3600.0,2.02,0.0,0.0,27.33,21.52,3600.0,2.56,1.68,1.86,0.0,0.01,57.66,57.64,3600.0,2.52,1.74,1.91,0.0,0.02,72.8,72.05,3600.0,2.88,1.91,1.92,0.0,0.04,119.31,104.89,1131.48,3.08,2.22,1.75,0.0,0.08,150.53,116.87,312.26,2.2,2.39,2.03,0.0,0.17,146.33,147.03,264.75,2.06,2.06,2.85,0.0,0.41,194.35,133.68,515.59
489.0,3600.0,1.73,3600.0,2.03,0.0,0.0,27.74,21.66,3600.0,2.68,1.68,1.9,0.0,0.01,59.74,60.16,3600.0,2.68,1.77,1.92,0.0,0.02,99.74,73.0,3600.0,3.04,1.98,1.93,0.0,0.04,138.01,109.25,1146.59,3.39,2.32,1.78,0.0,0.08,153.5,121.1,319.15,2.23,2.51,2.1,0.0,0.17,150.9,151.47,302.3,2.32,2.32,2.98,0.0,0.41,194.84,137.09,526.56
490.0,3600.0,1.8,3600.0,2.05,0.0,0.0,31.07,22.34,3600.0,2.75,1.69,1.92,0.0,0.01,61.05,61.37,3600.0,2.89,1.82,2.03,0.0,0.02,111.29,74.49,3600.0,3.19,2.12,1.96,0.0,0.04,148.36,127.49,1257.91,3.41,2.46,1.8,0.0,0.08,156.41,122.52,413.78,2.4,2.56,2.11,0.0,0.17,159.54,155.3,305.44,2.37,2.37,3.01,0.0,0.41,196.83,143.07,819.02
491.0,3600.0,1.84,3600.0,2.1,0.0,0.0,32.92,23.82,3600.0,2.82,1.74,2.13,0.0,0.01,62.02,62.31,3600.0,2.92,1.86,2.16,0.0,0.02,115.95,85.67,3600.0,3.76,2.45,2.06,0.0,0.04,150.53,130.49,1277.28,3.76,2.5,1.86,0.0,0.08,159.54,122.93,460.1,2.47,2.74,2.15,0.0,0.17,187.9,163.72,646.81,2.44,2.44,3.21,0.0,0.41,200.88,146.11,949.01
492.0,3600.0,1.85,3600.0,2.16,0.0,0.0,36.23,27.75,3600.0,3.14,1.77,2.14,0.0,0.01,64.05,68.33,3600.0,3.01,1.92,2.2,0.0,0.02,118.12,95.39,3600.0,3.89,2.58,2.19,0.0,0.04,156.41,132.15,1869.82,3.88,2.68,1.87,0.0,0.08,160.64,132.15,567.77,2.72,2.85,2.16,0.0,0.17,189.7,171.22,767.11,2.7,2.7,3.42,0.0,0.41,204.48,147.94,1504.81
493.0,3600.0,1.86,3600.0,2.16,0.0,0.0,39.19,34.13,3600.0,3.37,1.89,2.24,0.0,0.01,64.98,75.68,3600.0,3.41,1.97,2.22,0.0,0.02,120.1,101.61,3600.0,3.94,2.61,2.21,0.0,0.04,158.35,134.86,2338.78,3.89,2.77,2.15,0.0,0.08,169.14,155.3,771.23,2.75,3.01,2.17,0.0,0.17,213.04,205.7,1144.55,2.8,2.8,3.47,0.0,0.41,215.07,166.97,2004.12
494.0,3600.0,1.93,3600.0,2.16,0.0,0.0,42.84,35.96,3600.0,3.78,1.89,2.58,0.0,0.01,66.42,76.68,3600.0,3.84,2.07,2.34,0.0,0.02,136.76,105.1,3600.0,4.1,2.65,2.64,0.0,0.04,161.65,142.47,3600.0,4.06,2.81,2.17,0.0,0.08,202.41,193.59,813.58,3.2,3.03,2.24,0.0,0.17,236.46,211.64,2118.22,2.88,2.88,3.49,0.0,0.41,241.76,174.62,3600.0
495.0,3600.0,2.0,3600.0,2.21,0.0,0.0,43.18,36.54,3600.0,4.08,2.13,2.61,0.0,0.01,73.81,95.62,3600.0,4.02,2.08,2.47,0.0,0.02,178.76,127.43,3600.0,4.28,2.8,2.69,0.0,0.04,163.81,156.82,3600.0,4.5,3.09,2.55,0.0,0.08,213.5,196.29,989.52,3.39,3.25,2.79,0.0,0.17,270.7,249.24,3026.8,2.9,2.9,3.74,0.0,0.41,290.75,175.43,3600.0
496.0,3600.0,2.04,3600.0,2.41,0.0,0.0,50.57,55.37,3600.0,4.29,2.27,2.65,0.0,0.01,99.74,98.88,3600.0,4.08,2.21,2.69,0.0,0.02,178.78,150.93,3600.0,4.51,3.03,2.72,0.0,0.04,178.78,164.31,3600.0,4.51,3.78,2.7,0.0,0.08,289.93,205.7,1211.51,3.65,3.34,2.92,0.0,0.17,339.89,257.21,3065.67,3.18,3.18,3.77,0.0,0.41,371.33,179.76,3600.0
497.0,3600.0,2.48,3600.0,3.17,0.0,0.0,92.08,62.45,3600.0,4.46,2.58,2.72,0.0,0.01,102.01,103.81,3600.0,4.28,2.24,3.09,0.0,0.02,204.52,159.96,3600.0,6.47,3.15,3.08,0.0,0.04,240.99,203.12,3600.0,4.91,3.8,2.71,0.0,0.08,450.21,468.07,3600.0,4.13,3.52,3.16,0.0,0.17,478.6,452.39,3600.0,3.24,3.24,10.56,0.0,0.41,375.84,240.15,3600.0
498.0,3600.0,2.61,3600.0,3.66,0.0,0.0,96.18,91.51,3600.0,5.64,3600.0,2.81,0.0,0.01,156.62,171.95,3600.0,4.29,2.48,3.32,0.0,0.02,394.71,213.86,3600.0,6.49,3.27,3.49,0.0,0.04,396.34,261.23,3600.0,6.42,4.37,2.8,0.0,0.08,541.42,504.23,3600.0,5.1,3.58,3.33,0.0,0.17,532.31,454.05,3600.0,3.56,3.56,11.88,0.0,0.41,397.81,272.64,3600.0
499.0,3600.0,5.14,3600.0,3.68,0.0,0.0,155.67,95.33,3600.0,6.18,3600.0,3.42,0.0,0.01,178.76,320.69,3600.0,5.27,3.9,3.81,0.0,0.02,735.71,239.56,3600.0,7.77,3.3,4.13,0.0,0.04,1645.87,296.48,3600.0,8.98,8.12,3.13,0.0,0.08,735.8,962.27,3600.0,6.42,3.65,4.6,0.0,0.17,3600.0,468.07,3600.0,12.71,12.71,13.39,0.0,0.41,1110.43,410.91,3600.0


==> times_small.tex <==
count,BEN,ANG-BA50,ANG-K500
0,0.59,0.05,0.35
1,0.82,0.05,0.35
2,0.89,0.05,0.35
3,0.92,0.06,0.35
4,0.96,0.07,0.36
5,0.99,0.07,0.36
6,0.99,0.07,0.36
7,1,0.07,0.36
8,1.01,0.07,0.37
9,1.02,0.07,0.37
10,1.06,0.07,0.38
11,1.07,0.08,0.38
12,1.09,0.08,0.38
13,1.1,0.08,0.38
14,1.1,0.08,0.38
15,1.11,0.08,0.38
16,1.15,0.08,0.38
17,1.16,0.08,0.39
18,1.2,0.08,0.39
19,1.2,0.09,0.39
20,1.2,0.09,0.39
21,1.22,0.09,0.39
22,1.24,0.09,0.39
23,1.24,0.09,0.4
24,1.25,0.09,0.4
25,1.26,0.09,0.4
26,1.27,0.1,0.4
27,1.28,0.1,0.4
28,1.28,0.1,0.4
29,1.28,0.1,0.4
30,1.29,0.1,0.41
31,1.31,0.11,0.41
32,1.35,0.11,0.41
33,1.36,0.11,0.41
34,1.36,0.11,0.41
35,1.36,0.11,0.41
36,1.38,0.11,0.41
37,1.38,0.11,0.41
38,1.4,0.12,0.41
39,1.4,0.12,0.41
40,1.42,0.12,0.42
41,1.42,0.12,0.42
42,1.43,0.13,0.42
43,1.43,0.13,0.42
44,1.43,0.13,0.42
45,1.44,0.13,0.42
46,1.44,0.14,0.42
47,1.46,0.14,0.42
48,1.46,0.14,0.42
49,1.46,0.14,0.43
50,1.47,0.15,0.43
51,1.5,0.15,0.43
52,1.54,0.16,0.43
53,1.56,0.16,0.43
54,1.57,0.16,0.43
55,1.59,0.16,0.43
56,1.59,0.17,0.43
57,1.59,0.17,0.43
58,1.6,0.17,0.43
59,1.63,0.17,0.43
60,1.64,0.18,0.43
61,1.64,0.18,0.43
62,1.64,0.19,0.43
63,1.64,0.19,0.43
64,1.64,0.19,0.43
65,1.67,0.19,0.44
66,1.7,0.19,0.44
67,1.71,0.2,0.44
68,1.71,0.2,0.44
69,1.71,0.2,0.44
70,1.72,0.2,0.44
71,1.73,0.2,0.44
72,1.74,0.2,0.44
73,1.77,0.21,0.45
74,1.8,0.21,0.45
75,1.8,0.21,0.45
76,1.8,0.21,0.45
77,1.8,0.22,0.45
78,1.81,0.22,0.45
79,1.82,0.22,0.45
80,1.82,0.22,0.45
81,1.83,0.23,0.45
82,1.84,0.23,0.45
83,1.85,0.23,0.45
84,1.86,0.23,0.46
85,1.88,0.23,0.46
86,1.88,0.23,0.46
87,1.89,0.24,0.46
88,1.89,0.24,0.46
89,1.9,0.24,0.46
90,1.91,0.24,0.46
91,1.93,0.25,0.46
92,1.95,0.25,0.46
93,2,0.25,0.47
94,2.02,0.25,0.47
95,2.02,0.25,0.47
96,2.05,0.25,0.47
97,2.05,0.25,0.47
98,2.05,0.25,0.47
99,2.06,0.25,0.47
100,2.06,0.26,0.47
101,2.08,0.26,0.47
102,2.08,0.26,0.48
103,2.09,0.26,0.48
104,2.1,0.26,0.48
105,2.1,0.26,0.48
106,2.1,0.27,0.48
107,2.13,0.27,0.48
108,2.15,0.28,0.48
109,2.16,0.28,0.48
110,2.18,0.28,0.48
111,2.18,0.28,0.48
112,2.2,0.28,0.49
113,2.2,0.29,0.49
114,2.21,0.29,0.49
115,2.22,0.29,0.49
116,2.24,0.29,0.49
117,2.25,0.3,0.49
118,2.27,0.3,0.49
119,2.28,0.3,0.49
120,2.36,0.3,0.49
121,2.37,0.3,0.49
122,2.38,0.3,0.5
123,2.4,0.3,0.5
124,2.4,0.3,0.5
125,2.4,0.3,0.5
126,2.42,0.3,0.5
127,2.43,0.3,0.5
128,2.44,0.3,0.5
129,2.45,0.31,0.5
130,2.47,0.31,0.5
131,2.5,0.31,0.5
132,2.51,0.31,0.5
133,2.55,0.31,0.5
134,2.57,0.31,0.5
135,2.6,0.31,0.5
136,2.61,0.31,0.51
137,2.67,0.31,0.51
138,2.67,0.31,0.51
139,2.68,0.31,0.51
140,2.69,0.31,0.51
141,2.7,0.31,0.51
142,2.7,0.31,0.51
143,2.73,0.31,0.51
144,2.73,0.31,0.51
145,2.74,0.32,0.51
146,2.74,0.32,0.51
147,2.76,0.32,0.51
148,2.76,0.32,0.51
149,2.76,0.32,0.52
150,2.77,0.32,0.52
151,2.78,0.32,0.52
152,2.79,0.32,0.52
153,2.79,0.33,0.52
154,2.79,0.33,0.52
155,2.8,0.33,0.52
156,2.81,0.33,0.53
157,2.81,0.33,0.53
158,2.82,0.33,0.53
159,2.84,0.33,0.53
160,2.84,0.33,0.53
161,2.87,0.33,0.53
162,2.88,0.33,0.53
163,2.94,0.34,0.53
164,2.94,0.34,0.53
165,2.98,0.34,0.53
166,2.98,0.34,0.53
167,2.99,0.34,0.53
168,3.03,0.34,0.53
169,3.04,0.34,0.54
170,3.06,0.34,0.54
171,3.07,0.34,0.54
172,3.08,0.34,0.54
173,3.09,0.35,0.54
174,3.09,0.35,0.54
175,3.1,0.35,0.54
176,3.12,0.35,0.54
177,3.13,0.35,0.54
178,3.17,0.35,0.54
179,3.21,0.35,0.54
180,3.21,0.35,0.54
181,3.22,0.35,0.54
182,3.24,0.35,0.54
183,3.27,0.35,0.55
184,3.29,0.36,0.55
185,3.31,0.36,0.55
186,3.35,0.36,0.55
187,3.35,0.36,0.55
188,3.38,0.36,0.55
189,3.38,0.37,0.56
190,3.39,0.37,0.56
191,3.39,0.37,0.56
192,3.45,0.37,0.56
193,3.45,0.37,0.56
194,3.46,0.37,0.56
195,3.46,0.38,0.56
196,3.48,0.38,0.56
197,3.56,0.38,0.56
198,3.57,0.39,0.56
199,3.6,0.39,0.56
200,3.61,0.39,0.56
201,3.63,0.39,0.56
202,3.66,0.39,0.57
203,3.66,0.39,0.57
204,3.74,0.39,0.57
205,3.78,0.39,0.57
206,3.79,0.4,0.57
207,3.8,0.4,0.57
208,3.83,0.4,0.57
209,3.83,0.4,0.57
210,3.86,0.4,0.57
211,3.91,0.4,0.57
212,3.96,0.4,0.57
213,3.97,0.4,0.57
214,3.98,0.4,0.57
215,3.99,0.41,0.57
216,4,0.41,0.58
217,4.02,0.41,0.58
218,4.03,0.41,0.58
219,4.04,0.41,0.58
220,4.11,0.41,0.58
221,4.14,0.41,0.58
222,4.17,0.42,0.58
223,4.19,0.42,0.58
224,4.19,0.42,0.58
225,4.32,0.42,0.59
226,4.34,0.42,0.59
227,4.38,0.42,0.59
228,4.4,0.42,0.59
229,4.47,0.42,0.59
230,4.57,0.42,0.59
231,4.62,0.43,0.59
232,4.65,0.43,0.59
233,4.66,0.43,0.59
234,4.66,0.43,0.6
235,4.69,0.43,0.6
236,4.71,0.43,0.6
237,4.73,0.43,0.6
238,4.77,0.44,0.6
239,4.79,0.44,0.6
240,4.82,0.44,0.6
241,4.83,0.44,0.6
242,4.84,0.44,0.6
243,4.93,0.44,0.6
244,5,0.45,0.6
245,5.04,0.45,0.6
246,5.05,0.45,0.61
247,5.13,0.45,0.61
248,5.15,0.45,0.61
249,5.16,0.45,0.61
250,5.28,0.45,0.61
251,5.36,0.45,0.61
252,5.45,0.45,0.61
253,5.46,0.45,0.61
254,5.47,0.46,0.61
255,5.55,0.46,0.61
256,5.56,0.46,0.62
257,5.59,0.46,0.62
258,5.61,0.46,0.62
259,5.62,0.47,0.62
260,5.66,0.47,0.62
261,5.72,0.47,0.63
262,5.83,0.47,0.63
263,5.96,0.47,0.63
264,6,0.47,0.63
265,6,0.48,0.63
266,6,0.49,0.63
267,6,0.49,0.64
268,6,0.49,0.64
269,6,0.49,0.64
270,6,0.49,0.64
271,6,0.49,0.64
272,6,0.49,0.64
273,6,0.5,0.65
274,6,0.5,0.65
275,6,0.5,0.65
276,6,0.5,0.65
277,6,0.5,0.65
278,6,0.5,0.65
279,6,0.51,0.65
280,6,0.51,0.66
281,6,0.51,0.66
282,6,0.51,0.66
283,6,0.51,0.66
284,6,0.52,0.67
285,6,0.52,0.67
286,6,0.53,0.67
287,6,0.53,0.68
288,6,0.53,0.68
289,6,0.54,0.68
290,6,0.54,0.68
291,6,0.55,0.69
292,6,0.55,0.69
293,6,0.55,0.7
294,6,0.55,0.7
295,6,0.55,0.7
296,6,0.55,0.7
297,6,0.55,0.7
298,6,0.56,0.7
299,6,0.56,0.71
300,6,0.56,0.71
301,6,0.56,0.71
302,6,0.56,0.71
303,6,0.57,0.72
304,6,0.57,0.72
305,6,0.57,0.72
306,6,0.57,0.72
307,6,0.57,0.72
308,6,0.57,0.72
309,6,0.58,0.73
310,6,0.58,0.73
311,6,0.59,0.73
312,6,0.59,0.73
313,6,0.59,0.73
314,6,0.6,0.74
315,6,0.6,0.74
316,6,0.6,0.75
317,6,0.6,0.75
318,6,0.6,0.75
319,6,0.61,0.75
320,6,0.61,0.75
321,6,0.61,0.75
322,6,0.61,0.75
323,6,0.61,0.75
324,6,0.62,0.76
325,6,0.63,0.76
326,6,0.63,0.76
327,6,0.63,0.76
328,6,0.64,0.77
329,6,0.64,0.77
330,6,0.64,0.77
331,6,0.64,0.77
332,6,0.65,0.77
333,6,0.65,0.77
334,6,0.65,0.77
335,6,0.65,0.78
336,6,0.66,0.78
337,6,0.66,0.78
338,6,0.66,0.78
339,6,0.66,0.78
340,6,0.66,0.79
341,6,0.66,0.79
342,6,0.67,0.8
343,6,0.67,0.8
344,6,0.68,0.8
345,6,0.68,0.8
346,6,0.68,0.8
347,6,0.68,0.8
348,6,0.69,0.8
349,6,0.69,0.8
350,6,0.7,0.81
351,6,0.7,0.81
352,6,0.71,0.81
353,6,0.71,0.82
354,6,0.73,0.82
355,6,0.73,0.82
356,6,0.74,0.82
357,6,0.74,0.83
358,6,0.74,0.83
359,6,0.74,0.83
360,6,0.75,0.83
361,6,0.76,0.83
362,6,0.77,0.84
363,6,0.78,0.84
364,6,0.78,0.84
365,6,0.78,0.84
366,6,0.78,0.85
367,6,0.79,0.85
368,6,0.79,0.86
369,6,0.8,0.86
370,6,0.81,0.87
371,6,0.82,0.88
372,6,0.82,0.89
373,6,0.83,0.89
374,6,0.83,0.9
375,6,0.83,0.9
376,6,0.83,0.9
377,6,0.83,0.91
378,6,0.84,0.91
379,6,0.84,0.91
380,6,0.84,0.92
381,6,0.84,0.92
382,6,0.85,0.92
383,6,0.86,0.92
384,6,0.86,0.93
385,6,0.86,0.94
386,6,0.87,0.95
387,6,0.91,0.95
388,6,0.92,0.96
389,6,0.92,0.97
390,6,0.93,0.98
391,6,0.93,0.98
392,6,0.94,0.99
393,6,0.97,0.99
394,6,0.99,1
395,6,1.01,1
396,6,1.03,1.01
397,6,1.04,1.01
398,6,1.04,1.02
399,6,1.04,1.03
400,6,1.04,1.04
401,6,1.05,1.05
402,6,1.06,1.05
403,6,1.06,1.07
404,6,1.07,1.09
405,6,1.08,1.09
406,6,1.08,1.09
407,6,1.09,1.12
408,6,1.09,1.12
409,6,1.1,1.12
410,6,1.1,1.13
411,6,1.11,1.14
412,6,1.11,1.16
413,6,1.11,1.16
414,6,1.11,1.16
415,6,1.12,1.18
416,6,1.12,1.18
417,6,1.12,1.21
418,6,1.13,1.21
419,6,1.13,1.21
420,6,1.13,1.22
421,6,1.14,1.23
422,6,1.14,1.25
423,6,1.15,1.25
424,6,1.16,1.25
425,6,1.17,1.29
426,6,1.2,1.3
427,6,1.2,1.32
428,6,1.2,1.32
429,6,1.21,1.33
430,6,1.22,1.34
431,6,1.24,1.36
432,6,1.24,1.37
433,6,1.24,1.37
434,6,1.25,1.39
435,6,1.26,1.4
436,6,1.27,1.4
437,6,1.28,1.42
438,6,1.29,1.44
439,6,1.29,1.45
440,6,1.29,1.45
441,6,1.29,1.46
442,6,1.31,1.46
443,6,1.31,1.47
444,6,1.32,1.47
445,6,1.33,1.48
446,6,1.34,1.48
447,6,1.35,1.48
448,6,1.36,1.5
449,6,1.36,1.5
450,6,1.38,1.51
451,6,1.39,1.52
452,6,1.4,1.53
453,6,1.4,1.53
454,6,1.41,1.55
455,6,1.42,1.56
456,6,1.43,1.57
457,6,1.46,1.62
458,6,1.46,1.63
459,6,1.51,1.64
460,6,1.53,1.66
461,6,1.54,1.67
462,6,1.6,1.7
463,6,1.61,1.72
464,6,1.61,1.73
465,6,1.65,1.75
466,6,1.67,1.77
467,6,1.68,1.77
468,6,1.68,1.77
469,6,1.7,1.79
470,6,1.74,1.81
471,6,1.75,1.84
472,6,1.77,1.87
473,6,1.79,1.96
474,6,1.8,1.97
475,6,1.85,1.97
476,6,1.91,2
477,6,1.98,2.04
478,6,1.98,2.15
479,6,2,2.17
480,6,2.05,2.21
481,6,2.12,2.24
482,6,2.24,2.26
483,6,2.4,2.32
484,6,2.42,2.36
485,6,2.44,2.37
486,6,2.52,2.65
487,6,2.58,2.73
488,6,2.88,2.85
489,6,3.04,2.98
490,6,3.19,3.01
491,6,3.76,3.21
492,6,3.89,3.42
493,6,3.94,3.47
494,6,4.1,3.49
495,6,4.28,3.74
496,6,4.51,3.77
497,6,6.47,10.56
498,6,6.49,11.88
499,6,7.77,13.39

